Are Graph Neural Networks Optimal Approximation Algorithms?

In this work we design graph neural network architectures that capture optimal approximation algorithms for a large class of combinatorial optimization problems, using powerful algorithmic tools from semidefinite programming (SDP). Concretely, we prove that polynomial-sized message-passing algorithms can represent the most powerful polynomial time algorithms for Max Constraint Satisfaction Problems assuming the Unique Games Conjecture. We leverage this result to construct efficient graph neural network architectures, OptGNN, that obtain high-quality approximate solutions on landmark combinatorial optimization problems such as Max-Cut, Min-Vertex-Cover, and Max-3-SAT. Our approach achieves strong empirical results across a wide range of real-world and synthetic datasets against solvers and neural baselines. Finally, we take advantage of OptGNN's ability to capture convex relaxations to design an algorithm for producing bounds on the optimal solution from the learned embeddings of OptGNN.

==> RB200_RB500.tex <==
\begin{tabular}{lll}
\toprule
Method & RB200 & RB500 \\
\midrule
CMP & 1.031 $^{\pm\text{0.006}}$ & 1.015 $^{\pm\text{0.004}}$ \\
Erd\H{o}sGNN & 1.031 $^{\pm\text{0.004}}$ & 1.021 $^{\pm\text{0.002}}$ \\
Meta-EGN & 1.028 $^{\pm\text{0.005}}$ & 1.016 $^{\pm\text{0.002}}$ \\
RUN-CSP & 1.124 $^{\pm\text{0.001}}$ & 1.062 $^{\pm\text{0.005}}$ \\ \midrule
OptGNN & 1.012 $^{\pm\text{0.006}}$ & 1.013 $^{\pm\text{0.003}}$ \\
\midrule
Greedy MVC    & 1.027 $^{\pm \text{0.007}}$ & 1.014 $^{\pm \text{0.003}}$ \\
%Random CMP    & 1.063 $^{\pm \text{0.027}}$ & 1.031 $^{\pm \text{0.015}}$ \\
%\midrule
%SCIP 8.0.3 (1s) & 1.017 $^{\pm \text{0.104}}$ & 1.025 $^{\pm \text{0.018}}$ \\
%SCIP 8.0.3 (5s) & 1.016 $^{\pm \text{0.007}}$ & 1.011 $^{\pm \text{0.003}}$ \\
%\midrule
Gurobi 10.0 (0.5s) & 1.009 $^{\pm \text{0.006}}$ & 1.013 $^{\pm \text{0.004}}$ \\
Gurobi 10.0 (1s)   & 1.002 $^{\pm \text{0.003}}$ & 1.012 $^{\pm \text{0.003}}$ \\
Gurobi 10.0 (5s)   & 1.000 $^{\pm \text{0.001}}$ & 1.004 $^{\pm \text{0.003}}$ \\
\bottomrule
\end{tabular}

==> VC_ratio_model.tex <==
\begin{tabular}{llllll}
\toprule
         Dataset &             GAT &            GCNN &             GIN &       GatedGCNN &          OptGNN \\
\midrule
 \midrule 
ER\textsuperscript{a} (50,100) & 1.077 $\pm$ 0.029 & 1.182 $\pm$ 0.053 & 1.168 $\pm$ 0.091 & 1.026 $\pm$ 0.018 & \textbf{1.010} $\pm$ 0.015 \\
ER\textsuperscript{a} (100,200) & 1.058 $\pm$ 0.020 & 1.160 $\pm$ 0.028 & 1.143 $\pm$ 0.024 & 1.062 $\pm$ 0.017 & \textbf{1.031} $\pm$ 0.012 \\
ER\textsuperscript{a} (400,500) & 1.069 $\pm$ 0.008 & 1.069 $\pm$ 0.008 & 1.064 $\pm$ 0.007 & 1.061 $\pm$ 0.008 & \textbf{1.013} $\pm$ 0.006 \\
       \midrule 
MUTAG\textsuperscript{b} & 1.021 $\pm$ 0.061 & 1.049 $\pm$ 0.108 & 1.020 $\pm$ 0.039 & 1.017 $\pm$ 0.040 & \textbf{1.009} $\pm$ 0.027 \\
     ENZYMES\textsuperscript{b} & 1.118 $\pm$ 0.135 & 1.310 $\pm$ 0.144 & 1.281 $\pm$ 0.151 & 1.008 $\pm$ 0.020 & \textbf{1.000} $\pm$ 0.000 \\
    PROTEINS\textsuperscript{b} & 1.129 $\pm$ 0.156 & 1.271 $\pm$ 0.125 & 1.262 $\pm$ 0.129 & \textbf{1.006} $\pm$ 0.016 & \textbf{1.010} $\pm$ 0.021 \\
    IMDB-BIN\textsuperscript{b} & 1.051 $\pm$ 0.040 & 1.147 $\pm$ 0.059 & 1.139 $\pm$ 0.070 & \textbf{1.001} $\pm$ 0.010 & 1.002 $\pm$ 0.016 \\
      COLLAB\textsuperscript{b} & 1.015 $\pm$ 0.038 & 1.116 $\pm$ 0.103 & 1.120 $\pm$ 0.120 & 1.102 $\pm$ 0.101 & \textbf{1.001} $\pm$ 0.003 \\
%   \midrule 
%REDDIT-BIN\textsuperscript{c} &                 &                 &                 &                 & \textbf{1.000} $\pm$ 0.002 \\
%REDDIT-M-12K\textsuperscript{c} &                 &                 &                 &                 & \textbf{1.000} $\pm$ 0.001 \\
% REDDIT-M-5K\textsuperscript{c} &                 &                 &                 &                 & \textbf{1.000} $\pm$ 0.001 \\
\bottomrule
\end{tabular}

==> additional.tex <==
Most algorithms can be organized into surprisingly few paradigms such as dynamic programming, convex optimization, divide and conquer, etc.  This observation becomes especially striking when dealing with fundamental NP-hard problems.  It is known, that for a remarkably broad class of problems--max cut, vertex cover, graph coloring, and any max constraint satisfaction problem--improving on the best approximation algorithms would be impossible if the so called unique games conjecture is true.  Perhaps equally remarkably, there is a class of algorithms that is known to be optimal amongst the polynomial time algorithms for max constraint satisfaction problems and it is given by a specific SDP relaxation.  Of course, this algorithm is only "efficient" theoretically, % in quotes, 
and does not preclude better approximation algorithms that could adapt to the data distribution over instances.  In this sense, it is critical that an optimal approximation comes from a learning algorithm that in the worst case still matches the performance of a powerful convex relaxation.  This is the driving question of our work.

\textit{"Is there an approximation algorithm that can learn to adapt to a data distribution over instances yet retain the optimal worst case performance of convex relaxations?"}
\[
\pE_\mu[\textbf{X}]\big|_z = \begin{bmatrix}
    \pE_\mu[1] & \pE_\mu[x_{i_1}] & \cdots & \pE_\mu[X_\phi] & \cdots  \pE_\mu[x_{i_1}x_{i_2}...x_{i_k}]\\
    \pE_\mu[x_{i_1}] & \pE_\mu[x_{i_1}^2] & \cdots &  \pE_\mu[x_{i_1}X_\phi] & \cdots \pE_\mu[x_{i_1}^2x_{i_2}...x_{i_k}]\\
    \vdots & \vdots & \vdots & \ddots & \vdots \\
    \pE_\mu[x_{i_1}x_{i_2}...x_{i_k}] & \pE_\mu[x_{i_1}^2x_{i_2}...x_{i_k}] & \cdots & \pE_\mu[x_{i_1}x_{i_2}...x_{i_k}X_\phi] & \cdots  \pE_\mu[x_{i_1}^2x_{i_2}^2...x_{i_k}^2]
\end{bmatrix}
\]
Even at first glance, if we set $M_{1,t}$ and $M_{2,t}$ to be projection matrices to a subspace of dimension $\hat{r}$ we observe that OptGNN-MC$_r(\textbf{v})$ can simulate projected gradient descent on any $\hat{r}$ less than $r$.  In this sense, OptGNN-MC$_r(\textbf{v})$ can at the very least simulate a dynamic that starts solving the SDP relaxation at $\hat{r} = \sqrt{N}$ and gradually decreases the rank to solve for a fixed point of the greedy dynamic at $\hat{r}=1$ with any schedule of step sizes.  Of course, what it actually learns with backpropagation over a dataset could is a much more diverse set of dynamics that can't be easily described, but can be evaluated as we do in ...          
\NK{Is the discussion around the rank main text worthy? The paragraph on greedy vs SDP relaxations etc is kind of hard to parse. Imo can just assert that this solves the SDP and then elaborate in the supplement}


Unique games curve is given TRUE objective (not relaxed) of value c the best poly time solution.  S(c) is given instances with SDP value c the minimum integral objective.    






\section{Lift and Project}
\[
X = \begin{bmatrix}
    x_{00} & x_{01} & \cdots & x_{0N} \\
    x_{10} & x_{11} & \cdots & x_{1N} \\
    \vdots & \vdots & \vdots & \ddots & \vdots \\
    x_{N0} & x_{N1} & \cdots &  x_{NN}
\end{bmatrix}
\]
We begin our discussion of discrete optimization by focusing on quadratic problems subject to quadratic constraints.  Take for example, the vertex cover problem.  

The integer program for vertex cover is as follows

\begin{align*} 
\text{Minimize:} \quad &  \sum_{i \in [N]} x_i\\
\text{Subject to:} \quad & (1-x_i)(1-x_j) = 0 & \forall (i,j) \in E\\
\quad & x_i \in \{0,1\} & \forall i \in [N]
\end{align*}

The global optimum of the integer program is the min vertex cover.  Unfortunately the loss is discrete and not amenable to the tools of continuous optimization. 
Therefore a common approach is to relax the loss to be within a continuous interval. 

\begin{align*} 
\text{Minimize:} \quad &  \sum_{i \in [N]} x_i\\
\text{Subject to:} \quad & (1-x_i)(1-x_j) = 0 & \forall (i,j) \in E\\
\quad & x_i \in [0,1] & \forall i \in [N]
\end{align*}

For sake of symmetry it's helpful to apply a simple affine transform to $x$ so that it's in the interval $[-1,1]$ as so. 

\begin{align*} 
\text{Minimize:} \quad &  \sum_{i \in [N]} \frac{1+x_i}{2}\\
\text{Subject to:} \quad & (1-x_i)(1-x_j) = 0 & \forall (i,j) \in E\\
\quad & x_i \in [-1,1] & \forall i \in [N]
\end{align*}

Although the objective is linear the constraint is quadratic which is the source of the nonconvexity.  The idea of relaxation is to add variables $x_{ij}$ to replace quadratic variables $x_ix_j$ to form a linear program relaxation. 

\begin{align*} 
\text{Minimize:} \quad &  \sum_{i \in [N]} \frac{1+x_i}{2}\\
\text{Subject to:} \quad & 1-x_i-x_j+x_{ij} = 0 & \forall (i,j) \in E\\
\quad & x_i \in [-1,1] & \forall i \in [N]\\
\quad & x_{ij} \in [-1,1] & \forall i,j \in [N]
\end{align*}

The advantage of the above formulation is its convexity, thus making it a convex relaxation.  A popular tightening of the linear program relaxation is the oft studied semidefinite program (SDP) relaxation.  Let $X$ be a symmetric matrix with entries denoting variables defined as follows.
\[
X = \begin{bmatrix}
    \Tilde{x}_{00} & \Tilde{x}_{01} & \cdots & \Tilde{x}_{0N} \\
    \Tilde{x}_{10} & \Tilde{x}_{11} & \cdots & \Tilde{x}_{1N} \\
    \vdots & \vdots & \vdots & \ddots & \vdots \\
    \Tilde{x}_{N0} & \Tilde{x}_{N1} & \cdots &  \Tilde{x}_{NN}
\end{bmatrix}
\]

Replacing the original variables $x_i$ with $\frac{\Tilde{x}_{i0} + \Tilde{x}_{0i}}{2}$ and $x_{ij}$ with $\frac{\Tilde{x}_{ij} + \Tilde{x}_{ji}}{2}$, and adopting the notation of frobenius inner product $\langle \rangle$ we have for adequately defined matrices $C$ and $A_e$ 

\begin{align*} 
\text{Minimize:} \quad &  \langle C,X\rangle\\
\text{Subject to:} \quad & \langle A_{e},X\rangle = 0 & \forall e \in E\\
\quad & X_{ii} = 1 & \forall i \in [N]\\
\quad & X \succeq 0\\
\end{align*}

Although the SDP formulation is convex, owing to the convexity of the spectrahedral cone of psd matrices, it is notoriously more expensive than linear programming.  However, the infamous 'low rank'  overparameterization of the SDP relaxation by Burer and Monteiro is amenable to fast iterative algorithms such as block coordinate descent (message passing).  Noting that   

\begin{align*} 
\text{Minimize:} \quad &  \langle C,VV^T\rangle\\
\text{Subject to:} \quad & \langle A_{e},VV^T\rangle = 0 & \forall e \in E\\
\quad & v_i \in \R^{r} & \forall i \in [N]\\  
\quad &\|v_i\| = 1 & \forall i \in [N]\\
\quad & V = \begin{bmatrix}
    \cdots & v_1 \cdots \\
    \cdots & v_2 \cdots \\
    & \vdots \\
    \cdots & v_N \cdots
\end{bmatrix}\\
\end{align*}

Next we move the linear constraints to the objective by introducing a penalty term $\rho > 0$ 

\begin{align*} 
\text{Minimize:} \quad &  \langle C,VV^T\rangle + \rho\sum_{e \in E}\langle A_{e},VV^T\rangle^2\\
\text{Subject to:}
\quad & v_i \in \R^{r} & \forall i \in [N]\\  
\quad &\|v_i\| = 1 & \forall i \in [N]\\
\quad & V = \begin{bmatrix}
    \cdots & v_1 \cdots \\
    \cdots & v_2 \cdots \\
    & \vdots \\
    \cdots & v_N \cdots
\end{bmatrix}\\
\end{align*}

Now we can design a simple projected gradient descent scheme as follows 

\begin{align*}
\hat{v_i}^{t+1} \defeq v_i^t - \eta \big( 2\sum_{j \in N(i)}C_{ij} v_j + 4\rho \sum_{j \in N(i)} \langle A_{(i,j)},VV^T\rangle A_{(i,j)} V \big)
\end{align*}

\begin{align*}
v_i^{t+1} = \frac{\hat{v}_i^{t+1}}{ \|\hat{v}_i^{t+1}\|}
\end{align*}

Note that the projected gradient descent is a message passing algorithm where neighbors of a node pass a linear form of their messages followed by a nonlinear update that is normalization.  That is to say it's a graph neural network.  

\subsection{Lift and Project Loss}
We refer to the following as the projected loss.  It corresponds to $r=1$ low rank SDP.  Aside from the fact that $x_i \in [-1,1]$, for $\rho$ sufficiently large it is identical to the discrete optimization problem.    
\begin{align*} 
\text{Minimize:} \quad &  \langle C,xx^T\rangle + \rho \sum_{e \in E} \langle A_e,xx^T\rangle^2\\
\text{Subject to:} 
\quad & x_i \in [-1,1] & \forall i \in [N]\\
\end{align*}

Next we define the lifted loss coresponding to the convex relaxation.  

\begin{align*} 
\text{Minimize:} \quad &  \langle C,VV^T\rangle + \rho\sum_{e \in E}\langle A_{e},VV^T\rangle^2\\
\text{Subject to:}
\quad & v_i \in \R^{r} & \forall i \in [N]\\  
\quad &\|v_i\| = 1 & \forall i \in [N]\\
\quad & V = \begin{bmatrix}
    \cdots & v_1 \cdots \\
    \cdots & v_2 \cdots \\
    & \vdots \\
    \cdots & v_N \cdots
\end{bmatrix}\\
\end{align*}



\section{Neural Certification Scheme}
First we define the primal problem 
\begin{align*}
\text{Minimize:} \quad &  \langle C,X\rangle \\
\text{Subject to:} \quad & \langle A_i, X\rangle = b_i & \forall i \in [k]\\
\quad & X \succeq 0
\end{align*}

Next we introduce lagrange multipliers $\lambda \in \mathbb{R}^k$ and $Q \succeq 0$ to form the lagrangian 
\begin{align*}
\mathcal{L}(\lambda,Q,X) = \langle C,X\rangle + \sum_{i \in [k]} \lambda_i (\langle A_i,X\rangle - b_i) - \langle Q,X\rangle
\end{align*}

where 
\begin{multline*}
OPT(X) = \min_{X \succeq 0}\max_{\lambda \in \R,Q \succeq 0}\mathcal{L}(\lambda,Q,X) \\
\geq \min_{V \in \mathbb{R}^{N \times N}}\max_{\lambda}\langle C,VV^T\rangle + \sum_{i \in [k]} \lambda_i (\langle A_i,VV^T\rangle - b_i)\\
\geq \max_{\lambda}\min_{V \in \mathbb{R}^{N \times N}}\langle C,VV^T\rangle + \sum_{i \in [k]} \lambda_i (\langle A_i,VV^T\rangle - b_i)\\
\geq \min_{V \in \mathbb{R}^{N \times N}}\langle C,VV^T\rangle + \sum_{i \in [k]} \lambda^*_i (\langle A_i,VV^T\rangle - b_i) 
\end{multline*}
Where in the first inequality we replaced $X \succeq 0$ with $VV^T$ which is a lower bound as every psd matrix admits a cholesky decomposition.  In the second inequality we flipped the order of min and max, and in the final inequality we chose a specific set of dual variables $\lambda^* \in \R^k$ which lower bounds the maximization over dual variables.  The key is to find a good setting for $\lambda^*$.  

Let 
\begin{align*}
F_\lambda(X) \defeq  \langle C,X\rangle + \sum_{i \in [k]} \lambda^*_i (\langle A_i,X\rangle - b_i) 
\end{align*}

We have by convexity that 

\begin{align*}
F_\lambda(X) -  F_\lambda(\Tilde{X}) \leq \langle \nabla F_\lambda(X), X - \Tilde{X} \rangle = \langle \nabla F_\lambda(X), X\rangle + \langle - \nabla F_\lambda(X) ,\Tilde{X} \rangle \\
\leq \langle \nabla F_\lambda(X), X\rangle - \lambda_{min}(\nabla F_\lambda(X) )\mathrm{Tr}(\Tilde{X})
\end{align*}
Therefore it suffices to upper bound the two terms above, which except for $\mathrm{Tr}(\Tilde{X})$ is entirely comprised of quantities that can be computed from the output of the lift-network.  Now let 

\begin{align*}
H_\lambda(V) \defeq  \langle C,VV^T\rangle + \sum_{i \in [k]} \lambda^*_i (\langle A_i,VV^T\rangle - b_i) 
\end{align*}

We know 

\begin{align*}
\nabla H_\lambda(V) =  2(C + \sum_{i \in [k]} \lambda^*_i A_i)V = 2 \nabla F_\lambda(X) V
\end{align*}

Let 
\begin{align*}
    R_{\lambda,\rho} (V) \defeq  \langle C,VV^T\rangle + \sum_{i \in [k]} \rho (\langle A_i,VV^T\rangle - b_i)^2 + \sum_{i=1}^N \bar{\lambda}_i(\langle e_ie_i^T, VV^T\rangle - 1)
\end{align*}
denote the penalized lagrangian with quadratic penalties for constraints of the form $\langle A_i,X \rangle = b_i$.  

Taking the gradient we obtain 

\begin{align*}
    \nabla R_{\lambda,\rho} (V) \defeq  2CV + \sum_{i \in [k]} 2\rho (\langle A_i,VV^T\rangle - b_i)A_i V + \sum_{i=1}^N 2\bar{\lambda}_i e_ie_i^TV
\end{align*}

Our rule for setting $\lambda^*_i$ is 
\[\lambda^*_i \defeq  2\rho (\langle A_i,VV^T\rangle - b_i)\] 

our rule for setting 
\[\bar{\lambda}_j \defeq \frac{1}{2}\|e_j^T(C + \sum_{i \in [k]} 2\rho (\langle A_i,VV^T\rangle - b_i)A_i) V \| \]

Writing out everything explicitly we obtain the following matrix for 

\begin{align*}
\nabla F_\lambda(V) =  C + \sum_{i \in [k]}  \rho (\langle A_i,VV^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2}\|e_j^T(C + \sum_{i \in [k]} 2\rho (\langle A_i,VV^T\rangle - b_i)A_i) V \| e_ie_i^T  
\end{align*}

Which is entirely computed in terms of $V$.  It's certainly possible to come up with tighter certification schemes which we leave to future work.    



\textbf{Intuition: } Near global optimality one step of the augmented method of lagrange multipliers ought to closely approximate the dual variables.  After obtaining a guess for the penalized lagrange multipliers we estimate the lagrange multipliers for the norm constraint by approximating $\nabla R_{\lambda}(V) = 0$.  The alternative would have been to solve the linear system for all the lagrange multipliers at once but this runs into numerical issues and degeneracies explained below.    

\textbf{Note:} The reason for splitting the set of dual variables is because the projection operator onto the unit ball is hard coded into the architecture of the lift network. Satisfying the constraint set via projection is different from the soft quadratic penalties on the remaining constraints and require separate handling.

\textbf{Morris Note: } It is important to understand that if we were to have computed $\Tilde{X}$, with all its constraints satisfied we'd have as many lagrange multipliers as $|E| + |V|$ for vertex cover. Indeed $\nabla R_{\lambda,\rho} = 0$ yields $N^2$ linear equalities.  However, many of them can be degenerate and fail to uniquely identify $\lambda$ leading to terrible numerical issues.  For example in vertex cover if only the first coordinate is nonzero then only $N$ linear constraints are active.  This issue is a problem with the bound $\langle A,X\rangle \leq \|A\| \mathrm{Tr}(X)$.  Observe that we may be able to tighten this bound with $\max_{X\succeq 0  \text{s.t} X_{ii} = 1}\langle A,X\rangle $ which computes the max cut relaxation for $A$.  


\subsection{Max Cut Certificate}
\begin{align*}
    \lambda_i = \frac{1}{2}\| \sum_{j \in N(i)} w_{ij}v_j\|    
\end{align*}
\subsection{Vertex Cover Certificate}
\begin{align*}
    \lambda_\phi = \frac{1}{2}\| \frac{1}{2}\sum_{i=1}^N w_iv_i + 2\rho\sum_{(i,j) \in E} (1- \langle v_i + v_j,\phi\rangle + \langle v_i, v_j \rangle)(-v_i - v_j)\|    
\end{align*}

\begin{align*}
    \lambda_i = \frac{1}{2}\| \frac{1}{2}w_j + 2\rho\sum_{j \in N(i)} (1- \langle v_i + v_j,\phi\rangle + \langle v_i, v_j \rangle)(-\phi + v_j)\|    
\end{align*}




 \subsection{Quadratic vs Linear objective for maxclique}

The question remains, does there exist a hypothesis in $\mathcal{H}$ that approximates the distributional loss of the ground truth estimator $h^*$ which belongs to a much bigger (infinite) class of hypotheses $\mathcal{H}^*$.  That is we wish to bound 

We adopt the loss minimization convention.  
\begin{align}
\E_{x \in \mathcal{D}}[\hat{h}(x)] - \E_{x \in \mathcal{D}}[h^*(x)] \leq \text{ ? } 
\end{align}

Convex optimizaqiton on a graph is remarkably stable.  Even large perturbations to the inputs do not effect the output substantially.  For intuition, consider convex optimization on a quadratic.  No matter where I initialize my gradient descent, I will converge to the global optimum after a small number of iterations.  If I parameterize the gradient descent as a neural network with infinite layers, I find that the number of samples required to learn convex optimization is far smaller than the number of parameters in the network (infinite).  This is because I know two facts.  Firstly, there is a much smaller network that can represent a near optimal solution (quantified by some parameter $\epsilon$).  Secondly, this network is agnostic to the initialization of the network, and depends solely on the description of the optimization.  In the case of a quadratic this will be some PSD matrix, and in the case of a graph optimization it will be the adjacency matrix of the graph.  Running this idea through the generalization analysis with a carefully constructed set of hypotheses we obtain a weird result.  We can learn with far fewer samples than the number of parameters in the OptGNN.  We apply this intuition to the case of GNN's.  

The hypothesis class $\mathcal{H}^*$ for a $\Phi$ layer OptGNN (way more general than this) is approximated to error $\epsilon$ by the following construction. For any $h \in \mathcal{H}^*$ comprised of matrices $h = \{M_1,M_2,...,M_{\Phi}\}$ .  Let $\textbf{NET}_{\epsilon'}: \R^{d \times d} \rightarrow \R^{d \times d}$ be a function that takes a $d$-by-$d$ matrix $M$ and maps it to an $\epsilon'$ entrywise fine net of $M$.  
That is to say the $(i,j)$'th entry of $\textbf{NET}_{\epsilon'}(M)$ is defined as 
\[\textbf{NET}_{\epsilon'}(M)_{(i,j)} \defeq 
\floor{M_{ij}/\epsilon'}\epsilon'\]

In particular the range of $\textbf{NET}_{\epsilon'}$ has cardinality $[(1/\epsilon')^{d^2}]$.  

We construct an injective map $\Omega: \mathcal{H}^* \rightarrow \mathcal{H}$ as follows  
\begin{align}
\Omega(h) \defeq \Bigg\{
\textbf{NET}_{\epsilon/d^{2L}}\big(M_{\Phi}\big), \textbf{NET}_{\epsilon/d^{2L}}\big(M_{\Phi - 1}\big), \textbf{NET}_{\epsilon/d^{2L}}\big(M_{\Phi - 2}\big), ..., \textbf{NET}_{\epsilon/d^{2L}}\big(M_{\Phi - L}\big)\Bigg\}
\end{align}
Note that the cardinality of the domain of \[\left|\bigcup_{h \in \mathcal{H}^*}\Omega(h) \right| \leq \Big(\frac{d^{2L}}{\epsilon}\Big)^{L}\]
which is independent of $\Phi$ the number of layers of the network.  Furthermore, we know there exists a hypothesis in $\mathcal{H}$ that $\epsilon$ approximates the optimal distributional loss.

\section{Can Neural Networks Learn Gradient Descent?}
In this section we develop some preliminary theoretical explanations for why deep and narrow neural networks can learn to perform difficult optimizations.  Our focus will be on the setting of networks that are truly deep (possibly infinitely deep) and also narrow which is a notoriously difficult setting as most of the study of overparameterized neural networks takes the large width scaling TODO: cite NTK. These networks are overparameterized as they have more parameters than training data.  We formulate a toy model for why such deep networks can generalize.  In particular, as far as the authors are aware, there does not exist an explanation for why an infinite depth network that is narrow can optimize something as simple as a quadratic!  

We adopt a simple toy model aimed to explain why overparameterized networks can learn to minimize quadratic functions.  

Let $\mathcal{D}$ be a distribution over quadratic functions $f_a(x) = a_2x^2 + a_1 x + a_3$.  Here we restrict the domain of $a_1 \in [0,a_{max}]$ so that we're working with convex functions.  We use the notation $\vec{a} = \{a_1,a_2,a_3\}$ such that we draw a dataset comprised of $N$ datapoints  $\vec{a}_1,\vec{a}_2,...,\vec{a}_N \sim \mathcal{D}$.    
Let $\mathbf{\theta} = \{\theta_1,\theta_2,...,\theta_T\} \in [-1,1]$ be a collection of $T$ parameters in a parameter space $\Theta$.  
Let the $\text{LAYER}_{(\theta,\vec{a})}$ function be defined as
\begin{align}
\text{LAYER}_{(\theta,\vec{a})}(x) \defeq x + \theta f'(x) \\
= x_t + \theta_t (2a_2x_t + a_1)
\end{align}
Then for some fixed initial $x_0 \in \R$ we define the $\text{NN}_{(\mathbf{\theta},x_0)}: \R^3 \rightarrow \R$ to be 
\begin{align}
\text{NN}_{(\theta,x_0)}(\vec{a}) = f_{a} \circ \text{LAYER}_{(\theta_T,\vec{a})} \circ \text{LAYER}_{(\theta_{T-1},\vec{a})} \circ ... \circ \text{LAYER}_{(\theta_0,\vec{a})}(x_0) 
\end{align}
To be clear, $x_0$ is not the data.  The data is a distribution over quadratics.  For convenience of notation we will often drop the dependence on $x_0$ and refer to $\text{NN}_{(\theta,x_0)}$ as $\text{NN}_{\theta}$.  
Clearly if every $\theta_i \in \mathbf{\theta}$ is a small negative constants $\eta \leq 1/2a_{max}$ then $\text{NN}_{\mathbf{\theta}}$ would implement some type of gradient descent.  However, for an $T$ layer network it's not at all clear what algorithm $\text{NN}_{\theta}$ would end up implementing.  For $T$ going to infinity, the standard PAC learning perturbation analysis in \lemref{lem:pac-learn} would suggest that $\text{NN}_{\theta}$ would require $T \log(T/\epsilon)$ samples.  This would imply that the $\text{NN}_{\theta}$ would never learn how to minimize a quadratic on datasets of fixed size.  This is dismal!  

To make the discussion more precise, let the empirical loss minimizer $\hat{\theta}$ be defined as follows.  

\begin{align}
\hat{\theta} \defeq \argmin_{\theta \in \Theta} \frac{1}{N}\sum_{i \in [N]}\text{NN}_{\theta}(\vec{a}_i)
\end{align}

Then we have the following result, that even with an infinite number of layers $T$, the neural network still successfully generalizes with a number of samples that is independent of the number of parameters.  In fact the sample complexity is dependent only on the distribution $\mathcal{D}$, the approximation error $\epsilon$, and the failure probability $\delta$.     

\begin{lemma}
For any number of layers $T > \frac{2a_{max}}{\epsilon}$, for any number of samples $N = poly(\epsilon^{-1},\delta^{-1})$ for any distribution $\mathcal{D}$ over quadratics, the empirical loss minimizer $\hat{\theta}$ satisfies  
\[\Pr\left[\left|\frac{1}{N}\sum_{i \in [N]}\text{NN}_{\hat{\theta}}(\vec{a}_i) 
 - \E_{\vec{a}\sim \mathcal{D}}\left[ \min_{x \in [-B,B]} f_{\vec{a}}(x)\right]\right| \geq \epsilon \right] \leq \delta \]
\end{lemma}
           
\begin{proof}

\end{proof}

In conclusion, deep and narrow networks can generalize despite having more parameters than training data.  



==> iclr_old.tex <==
\section{Introduction}
Combinatorial Optimization is the class of problems that optimize functions subject to constraints over discrete search spaces.  They are often NP-hard to solve and to approximate, owing to their typically exponential search spaces over nonconvex domains.  Nevertheless, their important applications in science and engineering \citep{gardiner2000graph,zaki1997new,smith2004design,du2017multi} has engendered a long history of study rooted in the following simple insight.  In practice, CO instances are endowed with domain-specific structure that can be exploited by specialized algorithms \citep{hespe2020wegotyoucovered, walteros2019maximum, ganesh2020unreasonable}.  In this context, neural networks are natural candidates for learning and then exploiting patterns in the data distribution over CO instances.


% Moreover, algorithms can be designed to provide different kinds of approximation guarantees. 
% Unfortunately designing and utilizing such algorithms requires significant expertise, hence they are only available for certain classes of instances or specific problems. 

% Indeed, there are known cases of data distributions that are hard to tackle with the best known algorithms, e.g., certain cryptographic instances for SAT solvers  \citep{ganesh2020unreasonable}.


The emerging field at the intersection of machine learning (ML) and combinatorial optimization (CO) has led to novel algorithms with promising empirical results for several CO problems. However, similar to classical approaches to CO, ML pipelines have to manage a tradeoff between efficiency and optimality. Indeed, prominent works in this line of research forego optimality and focus on parametrizing heuristics \citep{li2018combinatorial, khalil2017learning, yolcu2019learning, chen2019learning} or by employing specialized models \citep{zhang2023let, nazari2018reinforcement, toenshoff2019run, xu2021reinforcement, min2022can} and task-specific loss functions \citep{amizadeh2018learning, karalias2020erdos, wang2022unsupervised, karalias2022neural, sun2022annealed}. 
 Exact ML solvers that can guarantee optimality often leverage general techniques like branch and bound \citep{gasse2019exact, paulus2022learning} and constraint programming \citep{parjadis2021improving, cappart2019improving}, which offer the additional benefit of providing approximate solutions together with a bound on the distance to the optimal solution. The downside of those methods is their exponential worst-case time complexity. 
 This makes it clear that striking a balance between efficiency and optimality is challenging, which leads us to the central question of this paper:
 
% \emph{Are there \textbf{general and efficient} data-driven algorithms that can provide \textbf{optimal} worst-case approximation guarantees?}


\emph{Are there neural architectures for \textbf{general} combinatorial optimization that can learn to adapt to a data distribution over instances yet capture algorithms with \textbf{optimal} worst-case approximation guarantees?}

%SDP PARAGRAPH MAYBE?
To answer this question, we build on the extensive literature on approximation algorithms and semidefinite programming. Convex relaxations of CO problems via semidefinite programming are the fundamental building block for breakthrough results in the design of efficient algorithms for NP-Hard combinatorial problems, such as the Goemans-Williamson approximation algorithm for Max Cut \citep{goemans1995improved} and the use of the Lov\'{a}sz theta function to find the maximum independent set on perfect graphs \citep{lovasz1979shannon, grotschel1981ellipsoid}.  In fact, it is known that if the Unique Games Conjecture (UGC) is true, then the approximation guarantees obtained through semidefinite programming relaxations are indeed the best that can be achieved \citep{raghavendra2008optimal,barak2014sum}.
We will leverage these results to provide an affirmative answer to our question.  Our contributions can be organized into theory and experiments.  

First, on the theory side we show that a polynomial time message passing algorithm approximates the solution of an SDP with the optimal integrality gap for the class of Maximum Constraint Satisfaction Problems, assuming the UGC. The key theoretical insight is that a message-passing algorithm can be used to compute gradient updates for the augmented Lagrangian of an overparameterized reformulation of the SDP in \citep{raghavendra2008optimal}. This in turn leads to our main contribution, OptGNN, a graph neural network architecture that generalizes our message-passing algorithm and therefore captures its approximation guarantee.

Our second contribution is empirical.  We show that our theoretical construction can be used directly within graph neural network pipelines for CO that are easy to implement and train. By training with the SDP objective as a loss function, OptGNN learns embeddings that can be regarded as feasible fractional solutions of an overparameterized low rank SDP, which are subsequently rounded to feasible integral solutions.  On the primal side, we show OptGNN achieves strong empirical results against classical algorithms across a broad battery of datasets for landmark CO problems such as Max Cut and Vertex Cover.

\begin{figure}[t]
    \centering
    \hspace*{-1.6cm}  
    \includegraphics[width=1.25\linewidth]{figure_1_optgnn.pdf}
    \caption{Schematic representation of OptGNN. During training, OptGNN produces node embeddings $\mathbf{v}$ by calculating gradient updates in its forward pass using message passing on the input graph $G$. These embeddings then used to compute the augmented Lagrangian loss $\mathcal{L}_p(\mathbf{v};G)$. OptGNN is trained by minimizing the average loss over the training set. At inference time, the fractional solutions (embeddings) $\mathbf{v}$ for an input graph $G$ produced by OptGNN are rounded using randomized rounding and a greedy heuristic.}
    \label{fig:OptGNNsummary}
\end{figure}

Finally, to underscore the fact that OptGNN captures powerful convex relaxations, we construct dual certificates of optimality, i.e bounds that are provably correct, from OptGNN embeddings for the Max Cut problem that are virtually tight for small synthetic instances.  See our discussion on general neural certification schemes for extracting dual certificates from OptGNN networks in Appendix \ref{sec:certificate}.

%Our pipeline benefits from the power of semidefinite relaxations whilst avoiding the notoriously poor scalability of SDP solvers.


%  Some methods focus on obtaining exact approximation guarantees 
%  including the augmentation of various solvers with neural networks (citations) 
% CO solvers that rely on machine learning are commonly designed by replacing a known heuristic with one that is learned from the data, usually parametrized by a neural network.
% but not limited to differentiable solver design \citep{vlastelica2019differentiation, agrawal2019differentiable}


%   % For example, methods that rely on learning branch and bound heuristics (cite learning to solve MIPs, learned branch and bound, etc) can guarantee optimality but may suffer from long execution times, while other methods often forego any optimality guarantees in favor of fast execution (citations (learned heuristics, erdos, UL, RL)). This leads us to the central question that will be tackled in this paaper : {Can neural networks be used to design \emph{efficient} algorithms that are \emph{provably optimal?}} 

% % \textcolor{red}{”Is there an approximation algorithm that can learn to adapt to a data distribution over instances
% % yet retain the optimal worst case performance of convex relaxations?”
% % }


% The goal of this work is to make important steps towards answering this question. (TODO: cleanup and a little more granularity)

% (need a paragraph on SDPs and classic approximation results)
% \textcolor{red}{
% }



% First, we will formally investigate the question of optimal neural architecture design for combinatorial optimization. 
% To this end, we will leverage seminal results from the theory of approximation algorithms and semidefinite programming to show that, assuming the unique games conjecture, there exist polynomial size message passing architectures that are optimal for the important class of maximum constraint satisfaction problems. (TODO: more details)
% Drawing upon those insights, we then design efficient neural network architectures based on semidefinite relaxations. The neural networks can be efficiently trained without the need for labeled solutions, which can be computationally expensive to obtain for such problems. We empirically demonstrate that these architectures achieve results that are on par or better than SDP solvers while obtaining significantly better scalability and execution speed. Furthermore, our models perform competitively against neural baselines and state-of-the-art solvers like Gurobi across a variety of different problems and datasets, including real world and hard synthetic instances. 


To summarize, the contribution of this paper is twofold:
\begin{itemize}
    \item We construct a polynomial time message passing algorithm for solving the SDP of \cite{raghavendra2008optimal} for the broad class of maximum constraint satisfaction problems (including Max Cut, max-SAT, etc.), that is optimal barring the possibility of significant breakthroughs in the foundations of algorithms.  
    \item We construct graph neural architectures to capture this message passing algorithm and show that they achieve strong results against solvers and greedy algorithms.
\end{itemize}

% This is achieved by designing a message-passing neural network which leverages the gradients of the semidefinite-programming objective of the problem in its forward pass. Furthermore, we prove that, assuming the Unique Games Conjecture (citation), polynomial-sized message passing architectures are optimal for the class of maximum constraint satisfaction problems. Our method combines the best of both worlds: it enjoys the benefits of powerful convex relaxations obtained by SDPs while also providing improved efficiency and scalability compared to standard SDP solvers.

% \begin{enumerate}
%     \item Par 1: Why are we writing this paper: start by quickly summarizing CO and explaining the motivation for ML+CO.
%   what is missing from the current literature on ml+co. What are the basic questions of the field that have not been conclusively answered.
%   End of first par: transition to what we're going to present in this paper.
%     \item Par 2: What are we doing in this paper. Why is it important and how does it address what is missing from the literature?
%     \item Par 3: How is what we're doing any different from what has been done? What do we gain compared to other approaches?
    
% \end{enumerate}
\section{Related Work}
\paragraph{Optimal approximation algorithms.}
In theoretical computer science, it is typically quite difficult to prove that an algorithm achieves the best approximation guarantee for a given problem, as it is hard to rule out the existence of a more powerful algorithm. The Unique Games Conjecture \citep{khot2002power} is a striking development in the theory of approximation algorithms because it is able to circumvent precisely this obstacle. If true, it implies several approximation hardness results which often match the approximation guarantees of the best-known algorithms \citep{raghavendra2009towards,raghavendra2012reductions}. In fact, it implies something even stronger: there is a \emph{general} algorithm based on semi-definite programming that achieves the best possible approximation guarantees for several important problems \citep{raghavendra2008optimal}. Our theoretical contribution builds on these ideas to construct a neural architecture that is a candidate optimal approximation algorithm. For a complete exposition on the topic of UGC and approximation algorithms we refer the reader to \cite{barak2014sum}.

\paragraph{Semidefinite programming in machine learning.} Semidefinite programming has already found applications in machine learning pipelines. In a similar spirit to our work, \cite{wang2019satnet} propose a differentiable SDP-based SAT solver based on previous works on low-rank SDPs \citep{wang2019low}, while  \cite{krivachy2021high} use neural networks to solve primal-dual SDP pairs for quantum information tasks. The key difference in our case is that our neural network architecture naturally aligns with solving a low-rank SDP and while our GNNs capture the properties of the SDP, in practice they can also improve upon it.

Other applications of semidefinite programming in machine learning include global minimization of functions by obtaining kernel approximations through an SDP \citep{rudi2020finding}, deriving differentiable high-dimensional extensions of discrete functions \citep{karalias2022neural}, and leveraging the connection between SVMs and the Lov\'{a}sz theta function to efficiently find the largest common dense subgraph among a collection of graphs \citep{jethava2013lovasz}.

\paragraph{Neural combinatorial optimization.} Beyond semidefinite programming, prior work in the literature has examined the capabilities of neural networks to obtain solutions to combinatorial problems, including the ability of modern GNNs to achieve approximation guarantees for combinatorial problems \citep{sato2019approximation} and impossibility results for computing combinatorial properties of graphs \citep{loukas2019graph}. It was previously shown that for maxSAT, a neural network can straightforwardly obtain a 1/2-approximation \citep{liu2021can} which is also easily obtainable through a simple randomized algorithm \citep{johnson1973approximation}. SDPs can yield at least 3/4-approximations for max-SAT \citep{goemans1995improved}, so our approach improves significantly over previous results. Finally, a different divide and conquer approach was proposed by \cite{mccarty2021nn}, which uses Baker's paradigm to solve the maximum independent set problem on geometric intersection graphs by partitioning the problem into at most a linear number (on the size of the input) of subproblems of bounded size, which allows them to use a neural network on each subproblem to obtain an approximation guarantee. 

In order to obtain exact solvers that are guaranteed to find the optimal solution, a prominent direction in the field involves combining solvers with neural networks either to provide a \enquote{warm start} \citep{benidis2023solving}, or to learn branching heuristics for branch and bound \citep{gasse2019exact, nair2020solving, gupta2020hybrid, paulus2022learning} and CDCL SAT solvers \citep{selsam2019guiding, kurin2020can, wang2021neurocomb}. Owing to their integration with powerful solvers, those ML pipelines are able to combine some of the strongest elements of classical algorithms and neural networks to obtain compelling results. Other related work in this vein includes constructing differentiable solvers and optimization layers \citep{wang2019satnet, agrawal2019differentiable}, and the paradigm of neural algorithmic reasoning \citep{VELICKOVIC2021100273} which focuses on training neural networks to emulate classical polynomial-time algorithms and using them to solve various combinatorial problems \citep{ibarz2022generalist, georgiev2023neural}. Other prominent neural approaches that have achieved strong empirical results with fast execution times follow different learning paradigms including reinforcement learning \citep{ahn2020learning, bother2022s, tonshoff2022one, barrett2022learning} and unsupervised learning \citep{min2022can, ozolins2022goal, schuetz2022combinatorial, schuetz2022graph}. 

The list of works mentioned here is by no means exhaustive, for a complete overview of the field we refer the reader to the relevant survey papers \citep{cappart2023combinatorial, bengio2021machine}.
 % Gflownets \citep{zhang2023let} and simulated annealing \citep{correia2023neural}.
% For a complete survey on CO with neural networks we refer the reader 
%\begin{itemize}
    % \item \citep{gasse2019exact} l2branch and bound
    % \item \citep{mccarty2021nn} divide and conquer with neural net, break independent set into small instances and solve each with a NN
    % \item \citep{paulus2022learning} learning cutting planes
    % \item \citep{cappart2019improving} learning to improve bounds/decision diagrams with RL
    % \item \citep{parjadis2021improving} improving decision diagrams/constraint programming
    % \item \citep{selsam2019guiding} Unsat certificates with neural guided sat solver

   % \item RL: \citep{khalil2017learning, chen2019learning, yolcu2019learning, ahn2020learning, barrett2020exploratory, barrett2022learning, tonshoff2022one}
   % \item algorithmic reasoning \citep{velivckovic2021neural, georgiev2023neural,xulz20}
    %\item unsupervised maxclique with scattering networks
    %\citep{min2022can}
    %\item gflownets for comb opt\cite{zhang2023let}

    %\item \citep{correia2023neural} neural simulated annealing
     %\item approximate model counting/dnf sat \citep{abboud2020learning}
    
%\end{itemize}


\section{Optimal approximation algorithms with neural networks}
% 
This section is structured as follows. In order to build intuition, we begin the section with the example of finding the maximum cut on a graph. We show that solving the Max Cut problem using a vector (low-rank SDP) relaxation and a simple projected gradient descent scheme amounts to executing a message-passing algorithm on the graph. This sets the stage for our main result for the class of constraint satisfaction problems (CSP) which generalizes this observation. We describe a semidefinite program (\sdpref{alg:sdp-vector}) for maximum constraint satisfaction problems that achieves the optimal integrality gap assuming the UGC. Our theorem \ref{thm:main-theorem} shows that similarly to the Max Cut example, \sdpref{alg:sdp-vector} can be solved with message-passing (\Algref{alg:message-passing}). This leads us to define an overparametrized version of \Algref{alg:message-passing}, dubbed OptGNN. We then show that by solving \sdpref{alg:sdp-vector}, OptGNN can achieve optimal approximation guarantees for maximum constraint satisfaction problems.
% \NK{small warmup paragraph is probably needed here. Should mention:
% - brief informal introduction of the basic notions/pieces that will be needed to construct the argument
% - brief informal summary of the argument itsefl}

\subsection{Solving combinatorial optimization problems with message passing}
To build intuition, we begin with the canonical example for the usage of semidefinite programming in combinatorial optimization: the Maximum Cut (henceforth Max Cut) problem.
Given a graph $G = (V,E)$ with vertices $V$, $|V|=N$ and edge set $E$, in the Max Cut problem we are looking to find a set of nodes in $G$ that maximize the number of edges with exactly one endpoint in that set. Formally, this means solving the following nonconvex quadratic integer program.  
\begin{align}
 \max_{(x_1,x_2,...,x_N)} \quad &  
 \sum_{(i,j) \in E}  \tfrac{1}{2}(1 - x_ix_j)    \\
\text{subject to:}
\quad & x_i^2 = 1 & \forall i \in [N] \nonumber.
\end{align}

The global optimum of the integer program is the Max Cut.  Unfortunately the discrete variables are  not amenable to the tools of continuous optimization.  A standard technique is to 'lift' the problem and solve it with a rank constrained SDP.  Here we introduce a matrix $X \in \R^{N \times N}$ of variables, where we index the $i$'th row and $j$'th column entry as $X_{ij}$.  
\begin{align} \label{alg:rank}
 \max_{X} \quad & 
 \sum\nolimits_{(i,j) \in E}  \tfrac{1}{2}(1 - X_{ij})    \\ \nonumber
\text{subject to:}
\quad & X_{ii} = 1 & \forall i \in [N]\\ \nonumber
\quad & X \succeq 0\\ \nonumber 
\quad & \text{rank}(X) = r
\end{align}
The intuition is that a rank $r=1$ solution to \Algref{alg:rank} is equivalent to solving the integer program.  A common approach is to replace the integer variables $x_i$ with vectors $v_i \in \R^r$ and constrain $v_i$ to lie on the unit sphere. 
\begin{align}
 \min_{v_1,v_2,\dots,v_N}\quad & 
  -\sum\nolimits_{(i,j) \in E}  \tfrac{1}{2}(1 - \langle v_i,v_j\rangle)    \\ \nonumber
\text{subject to:}
\quad & \|v_i\| = 1 & \forall i \in [N]\\ \nonumber
\quad & v_i \in \R^r
\end{align}
% Under general conditions and for sufficiently large $r$, the global optimum of this optimization is equivalent to the standard SDP optimum with no rank constraint (see \cite{boumal2020deterministic} and \cite{o2022burer} for a complete discussion).
\cite{burer03} proposed a fast iterative algorithm for descending this loss.  The landscape of this nonconvex optimization is benign in that all local minima are approximately global minima \citep{GLMspurious16} and variations on stochastic gradient descent converge to its optimum \citep{bhojanapalli2018smoothed,jin2017escape} under a variety of smoothness and compactness assumptions.  Thus, for large enough $r$  (see \cite{boumal2020deterministic} and \cite{o2022burer} for more details), simple algorithms such as block coordinate descent \citep{erdogdu2019convergence} can find an approximate global optimum of the objective. Such optimization problems are covered in the extensive literature on low-rank matrix factorization, for more see \cite{yuelulowrank}.  

% However,  
% % for large $r$, it is unclear how to transform, i.e., round, the vectors $\mathbf{v}$ into a solution to the integral problem. %, an issue known as 'rounding'.  
% Thus we need an approach that generalizes projected gradient descent that performs well for small $r$. 
Projected gradient descent is a natural approach in this context. In iteration $t$ (and for $T$ iterations), it updates vector $v_i$ in $\mathbf{v}$ as
%is of the form: for iteration $t$ in max iterations $T$, and for vector $v_i$ in $\mathbf{v}$, perform the following update.  
\begin{align}
\hat{v_i}^{t+1} = v_i^t - \eta \sum\nolimits_{j \in N(i)} v_j^t \label{eq:gradupdate1}\\
v_i^{t+1} = \frac{\hat{v_i}^{t+1}}{\|\hat{v_i}^{t+1}\|}, \label{eq:gradupdate2}
\end{align}
where $\eta \in \R^{+}$ is an adjustable step size and we let $N(i)$ denote the neighborhood of node $i$.  The gradient updates to the vectors are local, i.e., each vector is updated by aggregating information from its neighboring vectors, so we can interpret the projected gradient descent steps as message-passing iterations. 

\paragraph{Overparametrized message passing.}
Our main contribution in this paper builds on the following observation. We may generalize the dynamics described above by considering an overparametrized version of the gradient descent updates in equations \ref{eq:gradupdate1} and \ref{eq:gradupdate2}. Let $\{M_{1,t}\}_{t \in [T]} \in \R^{r \times r}$ and $\{M_{2,t}\}_{t \in [T]} \in \R^{r \times r}$ each be sets of $T$ learnable matrices corresponding to $T$ layers of a neural network.  Then for layer $t$ in max iterations $T$, for embedding $v_i$ in $\mathbf{v}$, we have  
\begin{align}
\hat{v_i}^{t+1} & \defeq M_{1,t} v_i^t - M_{2,t} \sum\nolimits_{j \in N(i)} v_j^t + b_t\\
v_i^{t+1} & \defeq \frac{\hat{v_i}^{t+1}}{\|\hat{v_i}^{t+1}\|},
\end{align}
where $\{b_t\}_{t \in [T]}$ is a learnable affine shift.  More generally, we can write the dynamics as 
\begin{align}
\hat{v_i}^{t+1} & \defeq \text{UPDATE}(M_{1,t}, v_i^t, b_t, \text{AGGREGATE}(M_{2,t},\{v_j^t\}_{j \in N(i)}))\label{eq:gnnupdate1} \\ 
v_i^{t+1} & \defeq \text{NONLINEAR}(\hat{v_i}^{t+1}), \label{eq:gnnupdate2}
\end{align}
for efficiently computable functions $\text{UPDATE}: \R^{r \times r} \times \R^r \times \R^r \times \R^r \rightarrow \R^r$ and $\text{AGGREGATE}:\R^{r \times r} \times \R^{r|N(i)|} \rightarrow \R^r$ and $\text{NONLINEAR}: \R^{r} \rightarrow \R^r$. It is straightforward to see that these update dynamics can be represented by a Graph Neural Network (GNN), which we call OptGNN. It will become clear that the dynamics in \ref{eq:gradupdate1}, \ref{eq:gradupdate2} can be generalized to a large class of CO problems. Examples include vertex cover, maximum clique, and maximum constraint satisfaction problems (see additional derivation for vertex cover in \ref{sec:vertex-cover}). 

In the rest of this section, we will show that the OptGNN formulation can be used for all {maximum constraint satisfaction problems (max-CSPs). Max-CSPs include Max Cut, max-SAT, etc. Moreover, we will show that OptGNN can implement a message-passing (see \ref{def:message-passing} for definition) algorithm for max-CSPs that can be shown to achieve optimal approximation guarantees, assuming the Unique Games Conjecture. 
                 
\subsection{Message passing for max constraint satisfaction problems}


Given a set of constraints over variables, Max-CSP asks to find a variable assignment that maximizes the number of satisfied constraints.  %This problem is known as Max-CSP.  
 Formally, a Constraint Satisfaction Problem $\Lambda = (\mathcal{V}, \mathcal{P}, q)$ consists of a set of $N$ variables $\mathcal{V} \defeq \{x_i\}_{i \in [N]}$ each taking values in an alphabet $[q]$ and a set of predicates $\mathcal{P} \defeq \{P_z\}_{z \subset \mathcal{V}}$ where each predicate is a payoff function over $k$ variables denoted $X_z = \{x_{i_1}, x_{i_2}, ..., x_{i_k}\}$. Here we refer to $k$ as the arity of the Max-k-CSP.   We adopt the normalization that each predicate $P_z$ returns outputs in $[0,1]$.  We index each predicate $P_z$ by its domain $z$.  The goal of Max-k-CSP is to maximize the payoff of the predicates.  
\begin{equation} \label{eq:csp-obj}
OPT \defeq \max_{(x_1,...,x_N) \in [q]^N} \frac{1}{|\mathcal{P}|}\sum\nolimits_{P_z \in \mathcal{P}} P_z(X_z), 
\end{equation}
where we normalize by the number of constraints so that the total payoff is in $[0,1]$.  Therefore we can unambiguously define an $\epsilon$-approximate assignment as an assignment achieving a payoff of $OPT - \epsilon$. 
Since our result depends on a message-passing algorithm, we will need to define an appropriate graph structure over which messages will be propagated. To that end, we will leverage the constraint graph of the CSP instance. We define the constraint graph associated with a Max-CSP instance $\Lambda$ as follows.  Given a Max-k-CSP instance $\Lambda = (\mathcal{V}, \mathcal{P}, q)$ a constraint graph $G_\Lambda = (V,E)$ is comprised of vertices $V = \{v_{\phi,\zeta}\}$ for every subset of variables $\phi \subseteq z$ for every predicate $P_z \in \mathcal{P}$ and every assignment $\zeta \in [q]^k$ to the variables in $z$.  The edges $E$ are between any pair of vectors $v_{\phi,\zeta}$ and $v_{\phi',\zeta'}$ such that the variables in $\phi$ and $\phi'$ appear in a predicate together.     
%\end{definition}


 
\paragraph{Optimal message passing for Max-CSP.}  In order to construct OptGNN for this problem,  we first establish that message passing can be optimal for Max-CSPs.  To show this, consider the SDP of \cite{raghavendra2008optimal} which is known to possess the optimal integrality gap assuming the UGC. This Unique-Games-optimal program can be equivalently reformulated as we describe in \sdpref{alg:sdp-vector}. Then, for Max-k-CSP we define its approximation ratio to be  
\[ \text{Approximation Ratio} \defeq \min_{\Lambda \in \text{Max-k-CSP}}\frac{OPT(\Lambda)}{SDP(\Lambda)},\]
where the minimization is being taken over all instances $\Lambda$ with arity $k$.  The approximation ratio is always smaller than one.  Similarly the integrality gap is defined to be the inverse of the approximation ratio and is always greater than one.  There is no polynomial time algorithm that can achieve a superior (larger) approximation ratio assuming the truth of the conjecture. Furthermore, there is a polynomial time rounding algorithm \citep{RSanycsp09} that achieves the integrality gap of the SDP  of \citep{raghavendra2008optimal}, and therefore outputs an integral solution with the optimal approximation ratio.  Our main theoretical result is a polynomial time message passing algorithm (detailed in \Algref{alg:message-passing}) that solves the Unique Games optimal SDP.    

\begin{theorem} \label{thm:main} (Informal) Given a Max-k-CSP instance $\Lambda$, there exists a message passing \Algref{alg:message-passing} on constraint graph $G_\Lambda$ with a per iteration update time of $poly(|\mathcal{P}|,q^k)$ that computes in $poly(\epsilon^{-1}, |\mathcal{P}|,q^k,\log(\delta^{-1}))$ iterations an $\epsilon$-approximate solution to \sdpref{alg:sdp-vector} with probability $1-\delta$.  That is to say,  \Algref{alg:message-passing} computes a set of vectors $\mathbf{v}$ satisfying constraints of \sdpref{alg:sdp-vector} to error $\epsilon$ with objective value denoted $OBJ(\mathbf{v})$ satisfying $|OBJ(\mathbf{v}) - SDP(\Lambda)| \leq  \epsilon$.    
\end{theorem}
For the formal theorem and proof see \thmref{thm:main-theorem}.  
Our algorithm is remarkably simple: perform gradient descent on the quadratically penalized objective of \sdpref{alg:sdp-vector}.  We observe that the gradient takes the form of a message-passing algorithm. For each predicate, we associate $q^k$ vectors, one vector for each assignment to each subset of $k$ variables, for a total of $|\mathcal{P}|q^k$ vectors.  The updates on each vector only depend on the vectors appearing in the same predicates.  Therefore, if each variable $x_i$ appears in no more than $C$ predicates, every message update in the algorithm depends no more than $Cq^k$ vectors rather than the total set of  $|\mathcal{P}|q^k$ vectors.  For Max Cut for example this would mean each vector corresponds to a node that is updated as a function of the vectors in adjacent vertices, as described earlier in equations \ref{eq:gradupdate1} and \ref{eq:gradupdate2}. For more complicated CSPs this gradient iteration can be defined analogously by taking gradients of a penalized objective of the reformulated \sdpref{alg:sdp-vector} which is equivalent to the optimal SDP of \cite{raghavendra2008optimal}.   


% For Max Cut, the iteration is simply to adjust the vector corresponding to each node to point in the opposite direction of the neighboring vectors.

% Furthermore, we define message passing algorithms on the constraint graph $G_\Lambda$ as follows.  
\subsection{OptGNN for maximum constraint satisfaction problems}
 By inspection of the gradient iteration of \Algref{alg:message-passing} we see that for a Max-k-CSP instance $\Lambda$, \Algref{alg:message-passing} is a message-passing algorithm (for a precise definition see \ref{def:message-passing}) on the associated constraint graph $G_\Lambda$.  This message-passing form allows us to define OptGNN, a natural GNN generalization that captures this gradient iteration.
\begin{definition} [OptGNN for Max-CSP] \label{def:optgnn-maxcsp}Let $\Lambda$ be a Max-CSP instance on a constraint graph $G_{\Lambda}$ with $N$ nodes.  Let $V$ be an input matrix of dimension $r \times N$ for the $N$ nodes with embedding dimension $r$. Let $\mathcal{L}_\rho$ be the loss defined as in \eqref{eq:obj-penalized} associated with the Max-CSP instance $\Lambda$. Let $M$ be the OptGNN weights which are a set of matrices $M \defeq \{M_{1},M_2,...,M_{T}\} \in \R^{r \times 2r}$. We define the aggregation function $\text{AGG}: \R^{r \times N} \rightarrow \R^{2r \times N}$ as such 
\begin{align}
\text{AGG}(V) \defeq  
\begin{bmatrix}
V \\
\nabla \mathcal{L}_\rho(V)
\end{bmatrix}
\end{align}
Furthermore, let $\text{LAYER}_{M_i}: \R^{r \times N} \rightarrow \R^{r \times N}$ be defined as 
\[\text{LAYER}_{M_i}(V) = M_i (\text{AGG}(V)) \]
Finally, let $\text{OptGNN}_{(G_\Lambda,M)}: \R^{r \times N} \rightarrow \R$ be defined as 
\[\text{OptGNN}_{(G_\Lambda,M)}(V) =  \mathcal{L}_\rho \circ \text{LAYER}_{M_T} \circ .... \circ \text{LAYER}_{M_2} \circ\text{LAYER}_{M_1}(V)\]
Here we feed the output of the final layer $\text{LAYER}_{M_T}$ to the loss function $\mathcal{L}: \R^{r \times N} \rightarrow \R$.
\end{definition}
For the loss $\mathcal{L}_\rho$ defined in \eqref{eq:obj-penalized}
the form of the gradient $\nabla \mathcal{L}_\rho$ is a message passing algorithm over the nodes of the constraint graph $G_\Lambda$.  Therefore, OptGNN is a message passing graph neural network over $G_\Lambda$.  This point is of practical importance as it is what informs out implementation of the OptGNN architecture.  To make the theoretical connection between OptGNN and SDP solving precise,  we must ensure that a small amount of additive stochastic noise $\{b_t\}_{t \in [T]}$ is added at each layer for the sake of theoretical gradient convergence. We then arrive at the following corollary.    
\begin{comment} 
\begin{definition}[OptGNN] Given a Max-k-CSP instance $\Lambda$, an OptGNN$_{(T,r,G_\Lambda)}(\mathbf{v})$ is a $T$ layer, dimension $r$, neural network over constraint graph $G_\Lambda$ with learnable matrices $\{M_{1,t}\}_{t \in [T]}$, $\{M_{2,t}\}_{t \in [T]}$ and stochastic affine shift $\{b_t\}_{t \in [T]}$ that generalizes the gradient iteration \eqref{eq:key-iteration} of \Algref{alg:message-passing} with an embedding $v \in \mathbf{v}$ for every node in $G_{\Lambda}$ with updates of the form   
\[v_w^{t+1} = \text{UPDATE}(M_{1,t},v_w^t, \text{AGGREGATE}(M_{2,t},\{v_j^t\}_{j \in N(w)},v_w^t))\]
\[v_w^{t+1} = \text{NONLINEAR}(v_w^{t+1}) + b_t\]
For arbitrary polynomial time computable functions $\text{UPDATE}:\R^{r \times r} \times \R^r \times \R^r \rightarrow \R^r$, $\text{AGGREGATE}:\R^{r \times r} \times \R^{r|N(w)|} \times \R^r \rightarrow \R^r$,  and $\text{NONLINEAR}:\R^{r} \rightarrow \R^r$.  Here by 'generalize' we mean there exists an instantiation of the learnable parameters $\{M_{1,t}\}_{t \in [T]}$ and $\{M_{2,t}\}_{t \in [T]}$ such that OptGNN is equivalent to \eqref{eq:key-iteration}.      
\end{definition}
\end{comment}

\begin{corollary} \label{cor:optgnn}
Given a Max-k-CSP instance $\Lambda$, there is an OptGNN$_{(T,r,G_\Lambda)}(\mathbf{v})$  with $T = poly(\delta^{-1},\epsilon^{-1},|\mathcal{P}|q^k)$ layers, $r = |\mathcal{P}|q^k$ dimensional embeddings, such that there is an instantiation of learnable parameters $M$ and a random shift $\{b_t\}_{t \in [T]}$ that outputs a set of vectors $\bold{v}$ satisfying the constraints of \sdpref{alg:sdp-vector} and approximating its objective, $OBJ_\text{SDP}(\Lambda)$, to error $\epsilon$ with probability $1-\delta$ over the randomness in $\{b_t\}_{t \in [T]}$.  
\end{corollary}

\begin{comment}
\begin{corollary} \label{cor:optgnn}
Given a Max-k-CSP instance $\Lambda$, there is an OptGNN$_{(T,r,G_\Lambda)}(\mathbf{v})$  with $T = poly(\delta^{-1},\epsilon^{-1},|\mathcal{P}|q^k)$ layers, $r = |\mathcal{P}|q^k$ dimensional embeddings, such that there is an instantiation of learnable parameters $\{M_{1,t}\}_{t \in [T]}$ and $\{M_{2,t}\}_{t \in [T]}$ and a random shift $\{b_t\}_{t \in [T]}$ that outputs a set of vectors $\bold{v}$ satisfying the constraints of \sdpref{alg:sdp-vector} and approximating its objective, $OBJ_\text{SDP}(\Lambda)$, to error $\epsilon$ with probability $1-\delta$ over the randomness in $\{b_t\}_{t \in [T]}$.  
\end{corollary}
\end{comment}
It is also straightforward to conclude that the rounding of \cite{RSanycsp09} achieves the integrality gap of \sdpref{alg:sdp-vector}, and any OptGNN that approximates its solution.  For the sake of completeness, we discuss the implications of the rounding.  Let the integrality gap curve $S_\Lambda(c)$ be defined as \[S_\Lambda(c) \defeq \inf_{\substack{\Lambda \in \text{Max-k-CSP} \\ OBJ_{\text{SDP}}(\Lambda) = c}} OPT(\Lambda),\]  which leads to the following statement about rounding.
\begin{corollary} The OptGNN of \corref{cor:optgnn} , which by construction is equivalent to \Algref{alg:message-passing}, outputs a set of embeddings $\mathbf{v}$ such that the rounding of \cite{RSanycsp09} outputs an integral assignment $\mathcal{V}$ with a Max-k-CSP objective OBJ($\mathcal{V}$) satisfying 
$OBJ(\mathcal{V}) \geq S_{\Lambda}(OBJ_{\text{SDP}}(\Lambda)-\epsilon)-\epsilon$ in time $\text{exp}(\text{exp}(\text{poly}(\frac{kq}{\epsilon})))$ which approximately dominates the Unique Games optimal approximation ratio.    
\end{corollary}
We defer the proofs of the corollaries to \autoref{sec:misc}


\paragraph{Obtaining neural certificates.} The goal of OptGNN is to find high quality solutions to CO problems by capturing powerful classes of convex relaxations. To underscore this point, we construct dual certificates of optimality (a proof) from the embeddings of OptGNN. The certificates provide a bound on the optimal solution of the SDP and can be computed directly from the embeddings produced by OptGNN.  The key idea is to "guess" the dual variables of \sdpref{alg:sdp-vector} from the output embeddings/SDP solution $\mathbf{v}$.  Since we use a quadratic penalty for constraints, the natural dual guess is one step of the augmented method of lagrange multipliers on the SDP solution which can be obtained straightforwardly from the overparameterized primal problem variables $\mathbf{v}$.  Of course, this "guess" need not be dual feasible.  To handle this problem we analytically bound the error in satisfying the KKT conditions of \sdpref{alg:sdp-vector}. See \ref{sec:certificate} for derivations and extended discussion, and \ref{subsec:certificates_experiment} for an experimental demonstration. 


       
%Of course, on instances where the SDP is optimal, we should expect OptGNN to match the SDP performance though this is not a guarantee.  We do not regard OptGNN to be an
%algorithm for learning how to round a fractional solution. Observe that ’rounding’ is inextricably
%intertwined with the solving of low rank SDP formulations as for r = 1 no rounding is even necessary.

\subsection{OptGNN in practice}
OptGNN is a neural network architecture that uses message passing to solve a low-rank semidefinite program (SDP) for a given combinatorial optimization problem. 
% The model learns to produce a feasible low-rank solution to a semidefinite program for the max-CSP. 
This is jointly achieved through the forward and backward pass. The message-passing steps in the forward pass are gradient updates to the node embeddings towards the direction that minimizes the augmented Lagrangian of the SDP. The backward pass aids this process by backpropagating derivatives from the augmented Lagrangian to the parameters of the neural network.  \Figref{fig:OptGNNsummary} summarizes the OptGNN pipeline for solving CO problems. Consider the Max Cut problem as an example. 
Given a distribution over graphs $\mathcal{D}$, for an input graph, OptGNN computes node embeddings 
$v_1,v_2, \dots,v_N \in \mathbb{R}^r$ which are then plugged into the loss function.  The loss in that case would be the Lagrangian which is calculated as $\mathcal{L}(\mathbf{v};G)= -\sum\nolimits_{(i,j) \in E}  \tfrac{1}{2}(1 - \langle v_i,v_j\rangle)$ (see Appendix \ref{sec:vertex-cover} for a minimum vertex cover example).
The network is then trained in a completely unsupervised fashion by minimizing $\mathbb{E}_{G \sim \mathcal{D}}[\mathcal{L}_p(\mathbf{v};G)]$ with a standard automatic differentiation package like Pytorch \citep{paszke2019pytorch}. 

Our theoretical result pertains to capturing the convex relaxation of \cite{raghavendra2008optimal}. As a message-passing algorithm, OptGNN does not deal with the issue of rounding fractional solutions. In practice, when implementing OptGNN, we round its fractional solutions using randomized rounding. Specifically, for each node with embedding vector $v_i$, its discrete assignment $x_i \in \{-1,1\}$ is calculated by $x_i= \text{sign}(v_i^\top y)$, for a random hyperplane vector $y \in \mathbb{R}^r$. We use multiple hyperplanes to obtain multiple solutions and then pick the best one. The solution is then post-processed with a simple heuristic.
 This enables fast inference while also helping ensure feasibility in the case of problems with constraints.

% \textbf{Limitations.} 
% \begin{itemize}
%     \item The applicability of the method requires an SDP relaxation for the problem that is being considered.
%     \item what else
% \end{itemize}

\section{Experiments}

\subsection{Comparisons with classical algorithms}
We report experimental measurements of the performance of the OptGNN approach on two NP-Hard combinatorial optimization problems, \textit{Maximum Cut} and \textit{Minimum Vertex Cover}. We obtain results for several datasets and compare against greedy algorithms, a state-of-the-art MIP solver (Gurobi). For details of the experimental setup see Appendix \ref{app:experimental_setup}.


\begin{table}[h]
\centering
\small
\input{maxcut_baseline_table.tex}
\caption{Performance of OptGNN, Greedy, and Gurobi 0.1s, 1s, and 8s on Maximum Cut. For each approach and dataset, we report the average cut size measured on the test slice. Here, higher score is better. In parentheses, we include the average runtime in \textit{milliseconds} for OptGNN.}
\label{tab:cut_baselines}
\end{table}


\paragraph{Results.}
Overall, we may clearly see that OptGNN can consistently outperform a greedy algorithm and is competitive with Gurobi when execution time is taken into account. 
\autoref{tab:cut_baselines} presents results for the maximum cut problem. Specifically, we report the average integral cut value achieved by OptGNN and classical baselines on a variety of datasets. We note that Greedy achieves poor performance compared to OptGNN and Gurobi on every dataset, indicating that for these datasets, finding Maximum Cut is not trivial. On the worst case, WS (400, 500), OptGNN achieves a cut value within 1.1\% on average of Gurobi with an 8s time limit. On other datasets, OptGNN is typically within a fraction of a percent. Notably, OptGNN is within 0.1\% of Gurobi 8s on all the TU datasets.


\iffalse
\autoref{tab:cut_neural} presents the performance of OptGNN compared to various neural baselines on the GSET instances.
\fi 

\begin{table}[h]
\centering
\small
\input{VC_baseline_table.tex}
\caption{Performance of OptGNN, Greedy, and Gurobi 0.1s, 1s, and 8s on Minimum Vertex Cover. For each approach and dataset, we report the average Vertex Cover size measured on the test slice. Here, lower score is better. In parentheses, we include the average runtime in \textit{milliseconds} for OptGNN.}
\label{tab:VC_baselines}
\end{table}
\autoref{tab:VC_baselines} presents the average size of the Vertex Cover achieved by OptGNN and classical baselines on our datasets. For this problem OptGNN also performs nearly as well as Gurobi 8s, remaining within 1\% on the TU datasets and 3.1\% on the worst case, ER (100, 200). OptGNN in certain cases outperforms Gurobi when considering execution time. Indeed, OptGNN requires only a few milliseconds to execute and is able to frequently outperform Gurobi when the latter is given a comparable time budget (0.1s). However, Gurobi with a 1s time budget is able to solve many of the datasets to optimality. While more computationally expensive than OptGNN, this constitutes only a small increase in total execution time for the entire dataset so Gurobi remains an extremely strong baseline.



\subsection{Experimental demonstration of neural certificates.} \label{subsec:certificates_experiment}
In this section, we provide a simple experimental example of our neural certificate scheme on small synthetic instances. 
Deploying this scheme on Max Cut on random graphs, we find this dual certificate to be remarkably tight. An example can be seen in  \figref{fig:cert50}. For $100$ node graphs with $1000$ edges our certificates deviate from the SDP certificate by about $20$ nodes but are dramatically faster to produce.  The runtime is dominated by the feedforward of OptGNN which is $0.02$ seconds vs. the SDP solve time which is $0.5$ seconds on cvxpy.  See \ref{sec:certificate} for extensive discussion and additional results.   


\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{cert100.png}
    \caption{Experimental comparison of SDP versus Opt-GNN Dual Certificates on random graphs of 100 nodes for the Max Cut problem. Our Opt-GNN certificates track closely with the SDP certificates while taking considerably less time to generate.}
    \label{fig:cert100}
\end{figure}


\iffalse
\begin{table}[!htbp]
\centering
\small
\input{maxcut_neural}
\caption{Comparison on GSET instances for Max Cut against state of the art neural baselines. Numbers reported are the mean deviations from the best known Max Cut values, reported as $f_\text{best}$ in table 2 of \cite{benlic2013breakout}. Lower is better.}
\label{tab:cut_neural}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{llll}
Dataset       & KaMIS          & LwD           & OptGNN (trained on (400, 500)) \\
ER (500, 500) & 459.39 (10.39) & 466.98 (0.23) & 470.52 (0.049) \\
BA (500, 500) & 292.83 (2.07)  & 293.27 (0.23) & 297.67 (0.026) \\
HK (500, 500) & 391.71 (9.68)  & 394.28 (0.27) & 455.82 (0.046) \\
WS (500, 500) & 432.5 (4.57)   & 443.78 (0.27) & 479.11 (0.037)
\end{tabular}
\caption{Comparison against KaMIS and LwD on various randomly generated instances.
Numbers reported are the vertex cover set sizes found by each method.
We report the best test score achieved by any of our models trained on the (400, 500) version of the corresponding dataset.
So the scores we report are not exactly an apples to apples comparison; especially for HK and WS the gap is clear.}
\end{table}
\fi

\subsection{Out Of Distribution generalization}
It is reasonable to examine whether our model learns a general combinatorial optimization algorithm or if it merely learns to fit the data distribution. A potential proxy for this is its out of distribution generalization, i.e., its ability to perform well on data distributions that it was not trained on. We test this using a collection of different datasets.
\begin{table}[h]
\centering
\small
\input{generalizability_table.tex}
\caption{Models for Vertex Cover trained on "dataset" were tested on a selection of the TU datasets ({ENZYMES, PROTEINS, MUTAG, IMDB-BINARY, and COLLAB}). We observe that the performance of the models generalizes well even when they are taken out of their training context.}
\label{tab:generalization}
\end{table}
 Specifically, for each dataset in our collection, we train a model and then test the trained model on a subset of datasets in the collection. The results are shown in \autoref{tab:generalization}. 
It is apparent from the results that the model performance generalizes well to different datasets. Strikingly, we frequently observe that the model reaches its peak performance on a given test dataset even when trained on a different one. This suggests that the model indeed is capturing elements of a more general process instead of just overfitting the training data.




\subsection{Ablation}
In order to better understand the effectiveness of the OptGNN architecture, we compare it against other commonly used GNN architectures from the literature that have been trained using the same loss function. We present the comparison of their performance to OptGNN for maximum cut in \autoref{tab:cut_models}; please see \autoref{sec:VC_ablation} for the analogous table for minimum vertex cover. It is clear that OptGNN consistently outperforms the other architectures on every dataset that we tested. 
Note that while OptGNN was consistently the best model, other models were able to perform relatively well; for instance, GatedGCNN achieves average cut values within a few percent of OptGNN on nearly all the datasets (excluding COLLAB). This points to the overall viability of training using an SDP relaxation for the loss function.
\begin{table}[!htbp]
\small
\input{maxcut_model_table.tex}
\caption{Performance of various model architectures for selected datasets on Maximum Cut. Here, higher is better. GAT is the Graph Attention network \citep{velivckovic2018graph}, GIN is the Graph Isomorphism Network \citep{xu2018how}, GCNN is the Graph Convolutional Neural Network \citep{morris2019weisfeiler}, and GatedGCNN is the gated version \citep{li2015gated}.}
\label{tab:cut_models}
\end{table}


\section{Conclusion}
We have presented OptGNN, a GNN that can capture provably optimal message passing algorithms for a large class of combinatorial optimization problems.
 OptGNN achieves the appealing combination of obtaining approximation guarantees while also being able to adapt to the data to achieve improved results. Empirically, we observed that the OptGNN architecture achieves strong performance on a wide range of datasets and on multiple problems.
 Since the landscape of combinatorial optimization is expansive, there are still important challenges that have to be addressed within the scope of this work such as the extension of our approach to problems with more complex constraints and objectives. OptGNN offers a novel perspective on the connections between general approximation algorithms and neural networks, and opens up new avenues for exploration. These include the design of more powerful and sound (neural) rounding procedures that can secure approximation guarantees, the construction of neural certificates that improve upon the ones we described in Appendix \ref{sec:certificate}, and the design of neural SDP-based branch and bound solvers. 

 \section{Acknowledgment} 

 The authors would like to thank Ankur Moitra, Sirui Li, and Zhongxia Yan for insightful discussions in the preparation of this work.  Nikolaos Karalias is funded by the SNSF, in the context of the project "General neural solvers for combinatorial optimization and algorithmic reasoning" (SNSF grant number: P500PT\_217999). Stefanie Jegelka acknowledges support from NSF award 1900933 and NSF AI Institute TILOS (NSF CCF-2112665).


% Striving for simplicity, we opted for a rudimentary approach to rounding that was able to yield efficient high quality solutions. This can certainly be improved by considering more sophisticated rounding algorithms from the literature or perhaps by adding learnable components to that part of the pipeline.



% We leave the generalization and extension of this technique as an avenue for future work. 


\clearpage
\bibliography{iclr2024_conference}
\bibliographystyle{iclr2024_conference}

\appendix

\section{Vertex Cover and Max Clique}
\label{sec:vertex-cover}
Minimum Vertex Cover can be written as the following integer program 
\begin{align} 
\text{Minimize:} \quad &  \text{VertexCover}(\mathbf{x}) \defeq\sum_{i \in [N]} \frac{1+x_i}{2}\\
\text{Subject to:} \quad & (1-x_i)(1-x_j) = 0 & \forall (i,j) \in E\\
\quad & x_i^2 = 1 & \forall i \in [N]
\end{align}
To deal with the constraint on the edges $(1-x_i)(1-x_j) = 0$, we add a quadratic penalty to the objective with a penalty parameter $\rho > 0$ yielding

\begin{align} 
\text{Minimize:} \quad &  \text{VertexCover}(\mathbf{x}) \defeq\sum_{i \in [N]} \frac{1+x_i}{2} + \rho\sum_{(i,j) \in E} (1 - x_i - x_j + x_ix_j)^2\\
\text{Subject to:} \quad & x_i^2 = 1 \quad \forall i \in [N]
\end{align}
Analogously to Max Cut, we introduce a natural low rank vector formulation $\text{LiftVertexCover}_r(\mathbf{v})$ for vectors $\mathbf{v} = \{v_i\}_{i \in [N]}$ in $r$ dimensions. 
\begin{align} 
\text{Minimize:} \quad &  \text{LiftVertexCover}_r(\mathbf{v}) \defeq\sum_{i \in [N]} \frac{1+\langle v_i,e_1\rangle}{2} + \rho\sum_{(i,j) \in E} (1 - \langle v_i,e_1\rangle - \langle v_j,e_1\rangle + \langle v_i,v_j \rangle)^2\\
\text{Subject to:} \quad & \|v_i\| = 1 \quad v_i \in \R^r \quad \forall i \in [N]
\end{align}

Now we can design a simple projected gradient descent scheme as follows.  For iteration $t $ in max iterations $T$, and for vector $v_i$ in $\mathbf{v}$ we perform the following update.   

\begin{equation}
\hat{v_i}^{t+1} \defeq v_i^t - \eta \big( e_1 + 2\rho \sum_{j \in N(i)}(1 - \langle v_i^t,e_1\rangle - \langle v_j^t,e_1\rangle + \langle v_i^t,v_j^t \rangle)(-e_1 + v_j^t)  \big)
\end{equation}
\begin{equation}
v_i^{t+1} \defeq \frac{\hat{v}_i^{t+1}}{ \|\hat{v}_i^{t+1}\|}
\end{equation}

We can then define a OptGNN-VertexCover$_r(\mathbf{v})$ analogously with learnable matrices $\{M_{1,t}\}_{t \in [T]} \in \R^{r \times r}$ and $\{M_{2,t}\}_{t \in [T]} \in \R^{r \times r}$ which are each sets of $T$ learnable matrices corresponding to $T$ layers of neural network.  Then for layer $t$ in max iterations $T$, for $v_i$ in $\mathbf{v}$, we have   

\begin{equation} \label{eq:vc-pgd}
\hat{v_i}^{t+1} \defeq M_{1,t}v_i^t + M_{2,t}\big( e_1 + 2\rho \sum_{j \in N(i)}(1 - \langle v_i^t,e_1\rangle - \langle v_j^t,e_1\rangle + \langle v_i^t,v_j^t \rangle)(-e_1 + v_j^t)  \big) + b_t
\end{equation}
\begin{equation}
v_i^{t+1} \defeq \frac{\hat{v}_i^{t+1}}{ \|\hat{v}_i^{t+1}\|}
\end{equation}
Here we added an affine shift $\{b_t\}_{t \in [T]}$ for completeness.  Once again we see \eqref{eq:vc-pgd} is captured by the dynamic 
\begin{align}
\hat{v_i}^{t+1} &= \text{UPDATE}(M_{1,t}, v_i^t,  \text{AGGREGATE}(M_{2,t},v_i^t,\{v_j^t\}_{j \in N(i)}) ,b_t)\\
v_i^{t+1} &= \text{NONLINEAR}(\hat{v_i}^{t+1})
\end{align}
For functions $\text{UPDATE}: \R^{r \times r} \times \R^r \times \R^r \times \R^r  \rightarrow \R^r$ and $\text{AGGREGATE}: \R^{r \times r} \times \R^{r|N(i)|} \times \R^r \rightarrow \R^r$ and $\text{NONLINEAR}: \R^{r} \rightarrow \R^r$.  Max Clique is computed by flipping the vertices of a min Vertex Cover on the complement graph.  
\section{Optimality of Message Passing for Max-CSP} \label{sec:message-passing}

Our primary theoretical result is that a polynomial time message passing algorithm  on an appropriately defined constraint graph computes the approximate optimum of \sdpref{alg:sdp-vector} which is notable for being an SDP that achieves the Unique Games optimal integrality gap.  

Our proof roadmap is simple. First, we design an SDP relaxation \sdpref{alg:sdp-vector} for Max-k-CSP that is provably equivalent to the SDP of \cite{raghavendra2008optimal} and therefore inherits its complexity theoretic optimality.  Finally, we design a message passing algorithm to approximately solve \sdpref{alg:sdp-vector} in polynomial time to polynomial precision. Our message passing algorithm has the advantage of being formulated on an appropriately defined constraint graph.  For a Max-k-CSP instance $\Lambda$ with $N$ variables, $|\mathcal{P}|$ predicates, over an alphabet of size $q$, it takes $|\mathcal{P}|q^k$ space to represent the Max-CSP.  Our message passing algorithm achieves an additive $\epsilon$ approximation in time $poly(\epsilon^{-1},N,|\mathcal{P}|q^k)$ which is then polynomial in the size of the CSP and inverse polynomial in the precision.    

Here we briefly reiterate the definition of Max-k-CSP.  A Max-k-CSP instance $\Lambda = (\mathcal{V}, \mathcal{P}, q)$ consists of a set of $N$ variables $\mathcal{V} \defeq \{x_i\}_{i \in [N]}$ each taking values in an alphabet $[q]$ and a set of predicates $\mathcal{P} \defeq \{P_z\}_{z \subset \mathcal{V}}$ where each predicate is a payoff function over $k$ variables denoted $z = \{x_{i_1}, x_{i_2}, ..., x_{i_k}\}$.  Here we refer to $k$ as the arity of the Max-k-CSP, and we adopt the normalization that each predicate $P_z$ returns outputs in $[0,1]$.  We index each predicate $P_z$ by its domain $z$ and we will use the notation $\mathcal{S}(P)$ to denote the domain of a predicate $P$.  The goal of Max-k-CSP is to maximize the payoff of the predicates.   

\begin{equation} \label{eq:csp-obj}
\max_{(x_1,...,x_N) \in [q]^N} \frac{1}{|\mathcal{P}|}\sum_{P_z \in \mathcal{P}} P_z(X_z) 
\end{equation}

Where $X_z$ denotes the assignment of variables $\{x_i\}_{i \in z}$.  

There is an SDP relaxation of \eqref{eq:csp-obj} that is the "qualitatively most powerful assuming the Unique Games conjecture" \cite{raghavendra2008optimal}. More specifically, the integrality gap of the SDP achieves the Unique Games optimal approximation ratio.  Furthermore, there exists a rounding that achieves its integrality gap.

\paragraph{SDP Reformulation: } Next we will introduce the SDP formulation we adopt in this paper.  For the sake of exposition and notational simplicity, we will work with binary Max-k-CSP's where $q = \{0,1\}$.  The extension to general $q$ is straightforward and detailed in the appendix.

We will adopt the standard pseudoexpectation and pseudodistribution formalism in describing our SDP.  
Let $\pE_\mu[\mathbf{x}]$ be a matrix in dimension $\R^{(N+1)^{d/2} \times (N+1)^{d/2}}$ of optimization variables defined as follows

\begin{align}
\pE_\mu[\mathbf{x}] \defeq \pE_\mu[(1,x_1,x_2,...,x_N)^{\otimes d/2} \big((1,x_1,x_2,...,x_N)^{\otimes d/2}\big)^T]
\end{align}
Where we use $\otimes$ to denote tensor product.  It is convenient to think of  $\pE_\mu[\mathbf{x}]$ as a matrix of variables denoting the up to $d$ multilinear moments of a distribution $\mu$ over the variables $\mathcal{V}$.  A multilinear  polynomial is a polynomial of the form $X_\phi \defeq \prod_{i \in \phi} x_i$ for some subset of the variables $\phi \subseteq \mathcal{V}$.  We index the variables of the matrix $\pE_\mu[\mathbf{x}]$ by the multilinear moment that it represents.  Notice that this creates repeat copies as their are multiple entries representing the same monomial.  This is dealt with by constraining the repeated copies to be equal with linear equality constraints.    

Specifically, let $z$ be a subset of the CSP variables $z \subset \{x_i\}_{i \in [N]}$ of size $k$.  Let $X_z$ denote the multilinear moment $X_z \defeq \prod_{i \in z} x_i$.  Then $\pE_\mu[X_z]$ denotes the SDP variable corresponding to the multilinear moment $\E_{\mu}[X_{z}]$.  Of course optimizing over the space of distributions $\mu$ over $\mathcal{V}$ is intractable, and so we opt for optimizing over the space of low degree pseudodistributions and their associated pseudoexpecation functionals.  See \cite{barak2014sum} for references therein.       

In particular, for any subset of variables $X_{z} \defeq \{x_{i_1},...,x_{i_k}\} \in \mathcal{V}$ we let $\pE_\mu[\mathbf{x}]\big|_{z,d}$ denote the matrix of the up to degree up to $d$ multilinear moments of the variables in $z$.

\begin{align}
\pE_\mu[\mathbf{x}]\big|_z \defeq \pE_\mu[(1,x_{i_1},x_{i_2},...,x_{i_k})^{\otimes d/2} \big((1,x_{i_1},x_{i_2},...,x_{i_k})^{\otimes d/2}\big)^T]
\end{align}   
We refer to the above matrix as a degree $d$ pseudoexpectation funcitonal over $X_z$.  Subsequently, we describe a pseudoexpectation formulation of our SDP followed by a vector formulation.
\paragraph{Multilinear Formulation:}A predicate for a boolean Max-k-CSP $P_z(X_z)$ can be written as a multilinear polynomial

\begin{align} \label{eq:defpz}
P_z(X_z) \defeq \sum_{\tau = (\tau_1,...,\tau_k) \in \{-1,1\}^k} w_{z,\tau}\prod_{x_i \in z} \frac{1+\tau_i x_i}{2} \defeq \sum_{s \subseteq z} y_sX_s
\end{align}
For some real valued weights $w_{z,\tau}$ and $y_s$ which are simply the fourier coefficients of the function $P_z$.  Then the pseudoexpectation formulation of our SDP is as follows
\begin{equation} \label{eq:sdp-obj}
\max_{\pE_{\mu}[\mathbf{x}]} \frac{1}{|\mathcal{P}|}\sum_{P_z \in \mathcal{P}} \pE_{\mu}[P_z(X_z)] 
\end{equation}

subject to the following constraints 
\begin{enumerate}
    \item \textbf{Unit: } $\pE_\mu[1] = 1$,  $\pE_\mu[x_i^2] = 1$ for all $x_i \in \mathcal{V}$, and $\pE_\mu[\prod_{i \in s} x_i^2 \prod_{j \in s'} x_j] = \pE_\mu[\prod_{j \in s'} x_j]$ for all $s,s' \subseteq \mathcal{S}(P)$ for every predicate $P \in \mathcal{P}$ such that $2s + s' \leq k$.  In expectation, the squares of all multilinear polynomials are equal to $1$.     
    \item \textbf{Positive Semidefinite: } $\pE_\mu[\mathbf{x}]|_{\mathcal{V},2} \succeq 0$ i.e the degree two pseudoexpectation is positive semidefinite. 
 $\pE_\mu[\mathbf{x}]\big|_{z,2k} \succeq 0$ for all $z = \mathcal{S}(P)$ for all $P \in \mathcal{P}$. The moment matrix for the multilinear polynomials corresponding to every predicate is positive semidefinite.     
\end{enumerate}

Equivalently we can view the SDP in terms of the vectors in the cholesky decomposition of $\pE_\mu[\mathbf{x}]$.  We rewrite the above SDP accordingly.  For this purpose it is useful to introduce the notation $\zeta(A,B) \defeq A \cup B / A \cap B$.  It is also useful to introduce the notation $\mathcal{C}(s)$ for the size of the set $\{g,g' \subseteq s: \zeta(g,g') = s\}$.  
% \makeatletter
% \renewcommand{\ALG@name}{CSP-SDP}
% % \makeatother
% \begin{SDPOPT} 
% \setcounter{algorithm}{0}
% \caption{SDP for Max-k-CSP (Equivalent to UGC-optimal)}
% \label{alg:sdp-vector}
% \begin{algorithmic} 
% \State{SDP Vector Formulation} {$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}. Multilinear formulation of objective.
% \begin{align} 
% \min_{x_1,x_2,\dots,x_N}  & \frac{1}{|\mathcal{P}|}\sum_{P_z \subset \mathcal{P}} \pE_{\mu}[-P_z(X_z)]  \defeq \frac{1}{|\mathcal{P}|}\sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} w_s\frac{1}{|\mathcal{C}(s)|}\sum_{g,g' \subseteq s: \zeta(g,g') = s} \langle v_{g}, v_{g'}\rangle \\
%  \text{subject to:} 
% & \; \|v_{s}\|^2 = 1 \quad \forall s \subseteq \mathcal{S}(P) \text{, } \forall P \in \mathcal{P} \\
% & \; \pE_\mu[X_{\zeta(g,g')}] \defeq \langle v_g,v_{g'} \rangle & \nonumber \\
% & \quad \quad \quad \quad \quad \; \; = \langle v_{h}, v_{h'}\rangle \quad \forall \zeta(g,g') = \zeta(h,h') \; \text{ s.t } \; g \cup g' \subseteq \mathcal{S}(P), \;\forall P \in \mathcal{P} %\\
% \end{align}
% \State{First constraint is the square of multilinear polynomials are unit.\\
% Second constraint are degree $2k$ SoS constraints for products of multilinear polynomials.}
% \end{algorithmic}
% \end{SDPOPT} 

\begin{lemma}
For Max-k-CSP instance $\Lambda$, The SDP of \sdpref{alg:sdp-vector} is at least as tight as the SDP of \cite{raghavendra2008optimal}.  
\end{lemma}
\begin{proof}
The SDP of \cite{raghavendra2008optimal} is a based degree $2$ SoS SDP augmented with $k$-local distributions for every predicate $P \in \mathcal{P}$.  By using the vectors of the cholesky decomposition and constraining them to be unit vectors  we automatically capture degree $2$ SoS.  To capture $k$ local distributions we simply enforce degree $2k$ SoS on the boolean hypercube for the domain of every predicate.  This can be done with the standard vector formulation written in \sdpref{alg:sdp-vector}.  See \cite{barak2014sum} for background and references.       
\end{proof}


% \makeatletter
% \renewcommand{\ALG@name}{Algorithm}
% % \makeatother
% \begin{algorithm} 
% \setcounter{algorithm}{0}
% \caption{Message Passing for Max-CSP}
% \label{alg:message-passing} \setcounter{algorithm}{0}
% \begin{algorithmic}[1]
% \Procedure{Message Passing}{$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}
% \State $n \gets 2^k \log(\delta^{-1})$
% \State $\eta, \psi, \sigma \gets n^{-100}$ \Comment{Initialize step size, noise threshold, and noise variance}
% \State $\mathbf{v}^0 = \{v_s\}_{s \subseteq z: P_z \in \mathcal{P}} \gets Uniform(\mathcal{S}^{n-1})$ \Comment{Initialize vectors to uniform on the unit sphere}
% \For{$t \in [poly(\epsilon^{-1},2^k,\log(\delta^{-1}))]$} 
% \For{$v_w^t \in \mathbf{v}^t$} \Comment{Iterate over vectors}
% \State 
% \begin{align} \label{eq:key-iteration}
% v_w^{t+1} \gets v_w^{t} - \eta \frac{1}{|\mathcal{P}|}\Bigg[\sum_{\substack{P_z \in \mathcal{P}\\\text{s.t } w \subseteq z}} \sum_{\substack{s \subseteq z\\\text{s.t } w \subseteq s}} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{w' \subseteq s\\ \text{s.t }\zeta(w,w') = s}} v_{w'}^t\\ 
% + 2\rho \Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t }w \subseteq z}} \sum_{\substack{w',h,h' \subseteq s\\ \text{s.t } \zeta(w,w') = \zeta(h,h')}} \big(\langle v_w^t,v_{w'}^t\rangle - \langle v_h^t, v_{h'}^t\rangle\big) v_w'^t \\
% +(\| v_w^t\|^2 - 1)v_w^t\Bigg]\Bigg]
% \end{align} \Comment{Update each vector with neighboring vectors in constraint graph}\\
% \If{$\| v_w^{t+1} - v_w^t\| \leq \psi$} 
%     \State $\zeta \gets N(0,\sigma I)$
% \Else 
%     \State $\zeta \gets 0$
% \EndIf
% \State $v_w^{t+1} \gets v_w^{t+1} + \zeta$ \Comment{Add perturbed noise if gradient smaller than threshold}
% \EndFor
% \EndFor
% \State \Return $\mathbf{v}^t$ \Comment{Returns the vectors corresponding to solution to \sdpref{alg:sdp-vector}}
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

\begin{theorem} \label{thm:main-theorem}
\Algref{alg:message-passing} computes in $poly(\epsilon^{-1},|\mathcal{P}|,2^k,\log(\delta^{-1}))$ iterations a set of vectors $\mathbf{v} \defeq\{\hat{v}_s\}$ for all $s \subseteq \mathcal{S}(P)$ for all $P \in \mathcal{P}$ that satisfy the constraints of \sdpref{alg:sdp-vector} to error $\epsilon$ and approximates the optimum of \sdpref{alg:sdp-vector} to error $\epsilon$ with probability $1-\delta$ 
\[\big|\sum_{P_z \in \mathcal{P}} \pE_{\hat{\mu}}[P_z(X_z)] - \text{OPTSDP}(\Lambda)\big| \leq \epsilon\]
where $\text{OPTSDP}(\Lambda)$ is the optimum of \sdpref{alg:sdp-vector}.  
\end{theorem}

\begin{proof}
We begin by writing down the objective penalized by a quadratic on the constraints.    
\begin{multline} \label{eq:obj-penalized}
\mathcal{L}_\rho(\mathbf{v}) \defeq \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \pE_\mu[P_z(X_z)]\\ + \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 +
\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}

For any monomial $X_s = \prod_{i \in s} x_i$ in $P_z(X_z)$ we write     
\begin{align} \label{eq:pseudo-monomial}
\pE_\mu[X_s] \defeq \frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\\text{s.t } \zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle
\end{align}
Where $\mathcal{C}(s)$ is the size of the set $\{g,g' \subseteq s: \zeta(g,g') = s\}$.  In a small abuse of notation, we regard this as the definition of $\pE_\mu[X_s]$ but realize that we're referring to the iterates of the algorithm before they've converged to a pseudoexpectation.  Now recall \eqref{eq:defpz}, we can expand the polynomial $P_z(X_z)$ along its standard monomial basis 
 
\begin{align} \label{eq:coef-basis}
P_z(X_z) = \sum_{s \subseteq z} y_s X_s 
\end{align}

where we have defined coefficients $y_s$ for every monomial in $P_z(X_z)$.  Plugging \eqref{eq:pseudo-monomial} and \eqref{eq:coef-basis} into \eqref{eq:obj-penalized} we obtain  
\begin{multline}
(\ref{eq:obj-penalized}) = \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\ \text{s.t }\zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle\\ 
+ \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 \\
+\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}
Taking the derivative with respect to any $v_w \in \mathbf{v}$ we obtain 

\begin{multline}
\frac{\partial \mathcal{L}_\rho(\mathbf{v})}{\partial v_w}  = \frac{1}{|\mathcal{P}|}\Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t } w \subseteq z}} \sum_{\substack{s \subseteq z\\\text{s.t } w \subseteq s}} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{w' \subseteq s\\ \text{s.t } \zeta(w,w') = s}} v_{w'}\\ 
+ 2\rho \Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t } w \subseteq z}} \sum_{\substack{w',h,h' \subseteq s\\ \text{s.t } \zeta(w,w') = \zeta(h,h')}} \big(\langle v_w,v_{w'}\rangle - \langle v_h, v_{h'}\rangle\big) v_w' \\
+(\| v_w\|^2 - 1)v_w\Bigg]\Bigg]
\end{multline} 
The gradient update is then what is detailed in \Algref{alg:message-passing}
\begin{align}
    v^{t+1}_w = v^t_w - \eta \frac{\partial \mathcal{L}_\rho(\mathbf{v})}{\partial v_w}
\end{align}
Thus far we have established the form of the gradient.  To prove the gradient iteration converges we reference the literature on convergence of perturbed gradient descent \citep{jin2017escape} which we rewrite in \thmref{thm:perturbed-gd}.  First we note that the \sdpref{alg:sdp-vector} has $\ell$ smooth gradient for $\ell \leq poly(\rho,B)$ and has $\gamma$ lipschitz Hessian for $\gamma = poly(\rho,B)$ which we arrive at in \lemref{lem:csp-lipschitz} and \lemref{lem:csp-hessian}.   
Then by \thmref{thm:perturbed-gd} the iteration converges to an $(\epsilon',\gamma^2)$-SOSP \defref{def:sosp} in no more than $\Tilde{O}(\frac{1}{\epsilon'^2})$ iterations with probability $1-\delta$. 
Now that we've established that the basic gradient iteration converges to approximate SOSP, we need to then prove that the approximate SOSP are approximate global optimum. We achieve this by using the result of \cite{bhojanapalli2018smoothed} lemma 3 which we restate here for convenience.      

To show that $(\epsilon',\gamma^2)$-SOSP are approximately global optimum, we have to work with the original SDP loss as opposed to the nonconvex vector loss.  

For subsequent analysis we need to define the penalized loss which we denote $\mathcal{H}_\rho(\pE[\mathbf{x}])$ in terms of the SDP moment matrix $\pE[\mathbf{x}]$.  
\begin{multline} \label{eq:obj-sdp-penalized}
\mathcal{H}_\rho(\pE[\mathbf{x}]) \defeq \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \pE_{\hat{\mu}}[P_z(X_z)]\\ + \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\pE_{\hat{\mu}}[X_{\zeta(g,g')}] - \pE_{\hat{\mu}}[X_{\zeta(h,h')}]\big)^2 +
\sum_{\substack{X_s \text{ s.t } s \subset \mathcal{S}(P)\\ |s| \leq k, \forall P \in \mathcal{P}}} (\pE_{\hat{\mu}}[X_s^2] - 1)^2\Bigg]\Bigg]
\end{multline}
Here we use the notation $\pE_{\hat{\mu}}[X_{\zeta(g,g')}]$ and $\pE_{\hat{\mu}}[X_{\zeta(h,h')}]$ to denote $\langle v_g,v_g'\rangle$ and $\langle v_h,v_h'\rangle$ respectively.    
Note that although by definition $\mathcal{H}_\rho(\pE[\mathbf{x}]) = \mathcal{L}_\rho(\mathbf{v})$ , their gradients and hessians are distinct because $\mathcal{L}_\rho(\mathbf{v})$ is overparameterized.  This is the key point.  It is straightforward to argue that SOSP of a convex optimization are approximately global, but we are trying to make this argument for SOSP of the overparameterized loss $\mathcal{L}_\rho(\mathbf{v})$. For this we defer to the analysis of \cite{bhojanapalli2018smoothed} \lemref{lem:smoothed} where we add our own discussion of some technical differences for adapting to the Max-CSP setting.         

Let the global optimum of \sdpref{alg:sdp-vector} be denoted $\pE_{\Tilde{\mu}}[\Tilde{\mathbf{x}}]$ with a cholesky decomposition $\Tilde{\mathbf{v}}$.  Let $\hat{\mathbf{v}}$ be the set of vectors outputted by \Algref{alg:message-passing} with associated pseudoexpectation $\pE_{\hat{\mu}}[\hat{\mathbf{x}}]$.  Then, we can bound
\begin{align} \label{eq:convex-bound}
\mathcal{L}_\rho(\hat{\mathbf{v}}) - \mathcal{L}_\rho(\Tilde{\mathbf{v}}) = \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]) - \mathcal{H
}_\rho(\pE[\Tilde{\mathbf{x}}])  \leq
\big\langle \nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]), \pE[\hat{\mathbf{x}}] - \pE[\Tilde{\mathbf{x}}]\big\rangle
\end{align}
Here the first equality is by definition, and the inequality is by the convexity of $\mathcal{H}_\rho$.  Moving on, we use the fact that $\nabla^2 \mathcal{L}_\rho(\hat{\mathbf{v}}) \succeq -\gamma\sqrt{\epsilon'}$ implies $\lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \geq -\gamma\sqrt{\epsilon'}$.  This fact is proven in \cite{bhojanapalli2018smoothed} lemma 3 \lemref{lem:smoothed}.  Subsequently, we adapt the lines of their argument in lemma 3 most relevant to our analysis which we detail here for the sake of completeness.
\begin{multline}
\text{\eqref{eq:convex-bound}} \leq  - \lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \Tr(\pE[\hat{\mathbf{x}}]) - \big\langle \nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]), \pE[\Tilde{\mathbf{x}}] \big\rangle\\
 \leq - \lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \Tr(\pE[\hat{\mathbf{x}}]) + \| \nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])\|_F \|\pE[\Tilde{\mathbf{x}}]\|_F\\
\leq \gamma \sqrt{\epsilon'} \Tr(\pE[\mathbf{x}]) +  \epsilon' \|\Tilde{\mathbf{v}}\|_F \leq \gamma \sqrt{\epsilon'}|\mathcal{P}|2^k + \epsilon' |\mathcal{P}|2^k \leq \epsilon\\
\end{multline}
Here the first inequality follows by a standard inequality of frobenius inner product, the second inequality follows by Cauchy-Schwarz, the third inequality follows by the $(\epsilon',\gamma^2)$-SOSP conditions on both the min eigenvalue of the hessian and the norm of the gradient, the final two inequalities follow from knowing the main diagonal of $\pE[\hat{\mathbf{x}}]$ is the identity and that every vector in $\tilde{\mathbf{v}}$ is a unit vector up to inverse polynomial error $poly(\rho^{-1},2^k)$.  For this last point see the proof in \lemref{lem:precision}.  Therefore if we set $\epsilon' = poly(\epsilon,2^{-k})$ we arrive at any $\epsilon$ error.  
Therefore we have established our estimate $\hat{v}$ is approximates the global optimum of the quadratically penalized objective i.e 
$\mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]) - \mathcal{H
}_\rho(\pE[\Tilde{\mathbf{x}}]) \leq \epsilon$.  
To finish our proof, we have to bound the distance between the global optimum of the quadratically penalized objective $\mathcal{H}_\rho(\pE[\Tilde{\mathbf{x}}])$ and OPTSDP$(\Lambda)$ the optimum of \sdpref{alg:sdp-vector}.  This is established for $\rho$ a sufficiently large $poly(\epsilon^{-1},2^k)$ in \lemref{lem:precision}. This concludes our proof that the iterates of \Algref{alg:message-passing} converge to the solution of \sdpref{alg:sdp-vector}.    
\end{proof}

\begin{lemma}\label{lem:smoothed} [\cite{bhojanapalli2018smoothed} lemma 3 rephrased]
Let $\mathcal{L}_\rho(\cdot)$ be defined as in \eqref{eq:obj-penalized} and let $\mathcal{H}_\rho(\cdot)$ be defined as in \eqref{eq:obj-sdp-penalized}.  Let $U \in \R^{N2^k \times N2^k}$ be an $(\epsilon,\gamma)$-SOSP of $\mathcal{L}_\rho(\cdot)$, then 
\[\lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \geq - \gamma\sqrt{\epsilon}\]
Furthermore, the  global optimum $\mathbf{\Tilde{X}}$ obeys the optimality gap 

\[\mathcal{H}_\rho(UU^T) - \mathcal{H}_\rho(\mathbf{\Tilde{X}}) \leq \gamma\sqrt{\epsilon} \Tr(\mathbf{\Tilde{X}}) + \frac{1}{2}\epsilon \|U\|_F\]

\end{lemma}


The following \lemref{lem:precision} establishes that for a sufficiently large penalty parameter $\rho = poly(\epsilon^{-1},2^k)$ the optimum of the penalized problem and the exact solution to \sdpref{alg:sdp-vector} are close.  

\begin{lemma} \label{lem:precision}
Let $\Lambda$ be a Max-k-CSP instance, and let OPTSDP$(\Lambda)$ be the optimum of \sdpref{alg:sdp-vector}.  Let $\mathcal{L}_\rho(\mathbf{v})$ be the quadratically penalized objective 
\begin{multline} \label{eq:loss-normalize}
\mathcal{L}_\rho(\mathbf{v}) \defeq \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\ \text{s.t } \zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle\\ 
+ \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 \\
+\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}
Let $\Tilde{v}$ be the argmin of the unconstrained minimization 
\[\Tilde{v} \defeq \argmin_{\mathbf{v} \in \R^{|\mathcal{P}|^2 (2^{2k})}} \mathcal{L}_\rho(\mathbf{v}) \]
Then we have   
\[\mathcal{L}_\rho(\Tilde{\mathbf{v}}) - \text{OPTSDP}(\Lambda) \leq \epsilon\]
for $\rho = poly(\epsilon^{-1},2^k)$ 
\end{lemma}

\begin{proof}
We begin the analysis with the generic equality constrained semidefinite program of the form 
\begin{align} \label{eq:sdp-generic} 
\text{Minimize:} \quad &  \langle C,X\rangle\\
\text{Subject to:} \quad & \langle A_{i},X\rangle = b_i & \forall i \in \mathcal{F}\\
\quad & X \succeq 0\\
\quad & X \in \R^{d \times d}
\end{align}

For an objective matrix $C$ and constraint matrices $\{A_i\}_{i \in \mathcal{F}}$ in some constraint set $\mathcal{F}$.  We will invoke specific properties of \sdpref{alg:sdp-vector} to enable our analysis.  First we define the penalized objective in this generic form
\[\mathcal{H}_\rho(X) \defeq \langle C,X\rangle + \rho\sum_{i \in \mathcal{F}}(\langle A_i,X\rangle - b_i)^2 \]
Let $\Tilde{X}$ be the minimizer of the penalized problem.  
\[\Tilde{X} \defeq \argmin_{X \in \R^{d \times d}}\mathcal{L}_\rho(X)\]
Let  $X^*$ be the minimizer of the constrained problem \eqref{eq:sdp-generic}.  
Let $\tau_i$ be the error $\Tilde{X}$ has in satisfying constraint $\langle A_i, \Tilde{X}\rangle = b_i$. 
\[\tau_i \defeq |\langle A_i,\Tilde{X}\rangle - b_i|\]
We will show that $\tau_i$ scales inversely with $\rho$.  That is, $\tau_i \leq poly(k,\rho^{-1})$.  Notice that the quadratic penalty on the violated constraints must be smaller than the decrease in the objective for having violated the constraints.  So long as the objective is not too sensitive 'robust' to perturbations in the constraint violations the quadratic penalty should overwhelm the decrease in the objective.  To carry out this intuition, we begin with the fact that the constrained minimum is larger than the penalized minimum.  
\begin{align}
\mathcal{H}_\rho(X^*) - \mathcal{H}_\rho(\Tilde{X}) \leq 0
\end{align}
Applying the definitions of $\mathcal{H}_\rho(X^*)$ and $\mathcal{H}_\rho(\Tilde{X})$ we obtain
\begin{align}
\langle C,X^* \rangle - (\langle C,\Tilde{X} \rangle + \rho\sum_{i \in \mathcal{F}} \tau_i^2) \leq 0
\end{align}
Rearranging LHS and RHS and dividing by $|\mathcal{F}|$ we obtain 
\begin{align} \label{eq:51}
\rho \frac{1}{|\mathcal{F}|}\sum_{i \in \mathcal{F}} \tau_i^2 \leq \frac{1}{|\mathcal{F}|} \langle C,\Tilde{X} - X^*\rangle
\end{align}
We upper bound the RHS using the robustness theorem of \cite{RSanycsp09} restated in the appendix \thmref{thm:robustness} which states that an SDP solution that violates the constraints by a small perturbation changes the objective by a small amount.  Thus we obtain,  
\begin{align} \label{eq:52}
RHS \leq \Big(\frac{1}{|\mathcal{F}|}\sum_{i \in \mathcal{F}} \tau_i \Big)^{1/2} poly(k)
\end{align}
Therefore combining \eqref{eq:51} with \eqref{eq:52} we obtain 
\[\rho \frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \leq \Big(\frac{1}{|\mathcal{F}|}\sum_i \tau_i \Big)^{1/2} poly(k)\]
Taking Cauchy-Schwarz on the RHS we obtain 
\[\rho \frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \leq \Big(\frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \Big)^{1/4}poly(k)\]
Noticing that $\frac{1}{|\mathcal{F}|}\sum_i \tau_i^2$ appears in both LHS and RHS we rearrange to obtain 
\[\frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \leq  \frac{poly(k)}{\rho^{4/3}} \leq \epsilon\]

Where for $\rho = \frac{poly(k)}{\epsilon^{3/4}}$ we have the average squared error of the constraints is upper bounded by $\epsilon$.  Then via markov's no more than $\sqrt{\epsilon}$ fraction of the constraints can be violated by more than squared error $\sqrt{\epsilon}$.  We label these 'grossly' violated constraints. The clauses involved in these grossly violated constraints contributes no more than $\sqrt{\epsilon} poly(k)$ to the objective.  On the other hand, the  constraints that are violated by no more than squared error $\sqrt{\epsilon}$ contributed no more than $\epsilon^{1/8} poly(k,q)$ to the objective which follows from the robustness theorem \thmref{thm:robustness}.  Taken together we conclude that   
\[\mathcal{L}_\rho(\Tilde{\mathbf{v}}) - \text{OPTSDP}(\Lambda) \leq \epsilon\]
For $\rho = poly(k,\epsilon^{-1})$ as desired.  
\end{proof}

Finally we show it's not hard to generalize our algorithm to alphabets of size $[q]$.  

\paragraph{Notation for General Alphabet.}
For any predicate $P \in \mathcal{P}$, let $\mathcal{D}(P)$ be the set of all variable assignment tuples indexed by a set of variables $s \subseteq \mathcal{S}(P)$ and an assignment $\tau \in [q]^{|s|}$.  Let $x_{(i,a)}$ denote an assignment of value $a \in [q]$ to variable $x_i$.   

\begin{SDPOPT}
\setcounter{algorithm}{1}
\caption{SDP Vector Formulation for Max-k-CSP General Alphabet (Equivalent to UGC optimal)}
\label{alg:sdp-vector-q}
\begin{algorithmic}
\State {SDP Vector Formulation General Alphabet $\Lambda = (\mathcal{V},\mathcal{P},q)$.\\  {Pseudoexpectation formulation of the objective.}} 
\begin{align} \label{eq:sdp-vector-q}
\min_{x_1,x_2,\dots,x_N}  & \sum_{P_z \subset \mathcal{P}} \pE_{\mu}[-P_z(X_z)]  \\ \nonumber
 \\ \text{subject to:} \quad & \pE_\mu[(x_{(i,a)}^2 - x_{(i,a)})\prod_{(j,b) \in \phi} x_{(j,b)}] = 0 \quad \forall i \in \mathcal{V}\text{, } \forall a \in [q]\text{, }\forall \phi \subseteq \mathcal{D}(P) \text{, } \forall P \in \mathcal{P}\\
\quad & \pE_\mu[(\sum_{a \in [q]} x_{ia} - 1)\prod_{(j,b) \in \phi} x_{(j,b)}] = 0\quad \forall i \in \mathcal{V}\text{, } \forall \phi \subseteq \mathcal{D}(P) \text{, }\forall P \in \mathcal{P}, \\
\quad & \pE_\mu[x_{(i,a)}x_{(i,a')} \prod_{(j,b) \in \phi} x_{(j,b)}] = 0 \quad \forall i \in \mathcal{V} \text{, } \forall a \neq a' \in [q]\text{, } \forall \phi \subseteq \mathcal{D}(P) \text{, }\forall P \in \mathcal{P}, \\
\quad & \pE[SoS_{2kq}(X_\phi)] \geq 0 \quad \forall \phi \subseteq \mathcal{D}(P) \text{, }\forall P \in \mathcal{P}, \\ 
\quad & \pE[SoS_2(\mathbf{x})] \geq 0.
  \end{align}
\State {First constraint corresponds to booleanity of each value in the alphabet. \\
Second constraint corresponds to a variable taking on only one value in the alphabet.\\
Third constraint corresponds to a variable taking on only one value in the alphabet.\\
Fourth constraint corresponds to local distribution on the variables in each predicate.
\\
Fifth constraint correpsonds to the positivity of every degree two sum of squares of polynomials.}


\end{algorithmic}
\end{SDPOPT} 



\begin{lemma} \label{lem:alphabet}
There exists a message passing algorithm that computes in $poly(\epsilon^{-1},|\mathcal{P}|,2^k,\log(\delta^{-1}))$ iterations a set of vectors $\mathbf{v} \defeq\{\hat{v}_{(i,a)}\}$ for all $(i,a) \in \phi$, for all $\phi \subseteq \mathcal{D}(P)$, for all $P \in \mathcal{P}$ that satisfy the constraints of \Algref{alg:sdp-vector-q} to error $\epsilon$ and approximates the optimum of \Algref{alg:sdp-vector-q} to error $\epsilon$ with probability $1-\delta$ 
\[\big|\sum_{P_z \in \mathcal{P}} \pE_{\hat{\mu}}[P_z(X_z)] - \text{OPTSDP}(\Lambda)\big| \leq \epsilon\]
where $\text{OPTSDP}(\Lambda)$ is the optimum of \Algref{alg:sdp-vector-q}. 

\end{lemma}

\begin{proof}
The proof is entirely parallel to the proof of \thmref{thm:main-theorem}.  We can write \Algref{alg:sdp-vector-q} entirely in terms of the vector of its cholesky decomposition where once again we take advantage of the fact that SoS degree $2kq$ distributions are actual distributions over subsets of $kq$ variables over each predicate.  Given the overparameterized vector formulation, we observe that once again we are faced with equality constraints that can be added to the objective with a quadratic penalty.  Perturbed gradient descent induces a message passing algorithm over the constraint graph $G_\Lambda$, and in no more than $poly(\epsilon^{-1},|P|,q^k)$ iterations reaches an $(\epsilon,\gamma)$-SOSP.  The analysis of optimality goes along the same lines as \lemref{lem:precision}.  For sufficiently large penalty $\rho = poly(\epsilon^{-1},|P|,q^k)$ the error in satisfying the constraints is $\epsilon$ and the objective is robust to small perturbations in satisfying the constraint.  That concludes our discussion of generalizing to general alphabets.       
\end{proof}
\subsection{Definitions}

\begin{definition}[Message passing algorithm] \label{def:message-passing}
 Given a graph $G = (V,E)$ with a set of vectors $\mathbf{v} = \{v_i\}_{i \in V}$ a message passing algorithm for $T$ iterations is an update of the form; for vector $v_i$ in $\mathbf{v}$ and for iteration $t \in [T]$, 
\[v_i^{t+1} = \text{UPDATE}(\{v_j^t\}_{j \in N(i)},v_i^t)\]
For an arbitrary polynomial time computable function $\text{UPDATE}: \R^{r|N(i)|} \times \R^r \rightarrow \R^r$
\end{definition}

\subsection{Neural Certification Scheme}
\label{sec:certificate}
An intriguing aspect of OptGNN is that the embeddings can be interpreted as the solution to a low rank SDP which leaves open the possibility that the embeddings can be used to generate a dual certificate i.e a lower bound on a convex relaxation.  First, we define the primal problem 
\begin{align} \label{eq:sdp-generic}
\text{Minimize:} \quad &  \langle C,X\rangle \\
\text{Subject to:} \quad & \langle A_i, X\rangle = b_i & \forall i \in [\mathcal{F}]\\
\quad & X \succeq 0
\end{align}
\begin{lemma}
\label{lem:certificate}
Let OPT be the minimizer of the SDP \eqref{eq:sdp-generic}.  Then for any $\Tilde{X} \in \R^{N \times N} \succeq 0$ and any $\lambda^* \in \R^{|\mathcal{F}|}$, we define $F_{\lambda^*}(X)$ to be
\[F_{\lambda^*}(\Tilde{X}) \defeq  \langle C,\Tilde{X}\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i (\langle A_i,\Tilde{X}\rangle - b_i) \]
We require SDP to satisfy a bound on its trace $Tr(X) \leq \mathcal{Y}$ for some $\mathcal{Y} \in \R^+$. Then the following is a lower bound on OPT.  
\[OPT \geq F_{\lambda^*}(\Tilde{X})  - \langle \nabla F_{\lambda^*}(\Tilde{X}), \Tilde{X}\rangle + \lambda_{min}(\nabla F_{\lambda^*}(\Tilde{X}) )\mathcal{Y}\]
\end{lemma}

\begin{proof}
Next we introduce lagrange multipliers $\lambda \in \mathbb{R}^k$ and $Q \succeq 0$ to form the lagrangian 
\begin{align*}
\mathcal{L}(\lambda,Q,X) = \langle C,X\rangle + \sum_{i \in \mathcal{F}} \lambda_i (\langle A_i,X\rangle - b_i) - \langle Q,X\rangle
\end{align*}

We lower bound the optimum of OPT defined to be the minimizer of \eqref{eq:sdp-generic}
\begin{align}
OPT \defeq \min_{X \succeq 0}\max_{\lambda \in \R,Q \succeq 0}\mathcal{L}(\lambda,Q,X) 
\geq & \min_{V \in \mathbb{R}^{N \times N}}\max_{\lambda}\langle C,VV^T\rangle + \sum_{i \in \mathcal{F}} \lambda_i (\langle A_i,VV^T\rangle - b_i)\\
=& \max_{\lambda}\min_{V \in \mathbb{R}^{N \times N}}\langle C,VV^T\rangle + \sum_{i \in \mathcal{F}} \lambda_i (\langle A_i,VV^T\rangle - b_i) \\
 \label{eq:sdp-overparam}  
=& \min_{V \in \mathbb{R}^{N \times N}}\langle C,VV^T\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i (\langle A_i,VV^T\rangle - b_i).
\end{align}
Where in the first inequality we replaced $X \succeq 0$ with $VV^T$ which is a lower bound as every psd matrix admits a cholesky decomposition.  In the second inequality we flipped the order of min and max, and in the final inequality we chose a specific set of dual variables $\lambda^* \in \R^{|\mathcal{F}|}$ which lower bounds the maximization over dual variables.  The key is to find a good setting for $\lambda^*$. 

Next we establish that for any choice of $\lambda^*$ we can compute a lower bound on inequality \ref{eq:sdp-overparam} as follows. 
Let $F_{\lambda^*}(VV^T)$ be defined as the funciton in the RHS of \ref{eq:sdp-overparam}. 
\begin{align*}
F_{\lambda^*}(VV^T) \defeq  \langle C,X\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i (\langle A_i,X\rangle - b_i) 
\end{align*}
Then \eqref{eq:sdp-overparam} can be rewritten as 
\begin{align*}
OPT \geq \min_{V \in \mathbb{R}^{N \times N}}F_{\lambda^*}(VV^T) \defeq  \langle C,X\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i (\langle A_i,X\rangle - b_i) 
\end{align*}
Now let $V^*$ be the minimizer of \eqref{eq:sdp-overparam}  and let $X^* = V^* (V^*)^T$.  We have by convexity that 
\begin{align}
F_{\lambda^*}(X) -  F_{\lambda^*}(X^*) \leq \langle \nabla F_{\lambda^*}(X), X - X^* \rangle = \langle \nabla F_{\lambda^*}(X), X\rangle + \langle - \nabla F_{\lambda^*}(X) ,X^* \rangle \\
\leq \langle \nabla F_{\lambda^*}(X), X\rangle - \lambda_{min}(\nabla F_{\lambda^*}(X) )\mathrm{Tr}(X^*)\\
\leq \langle \nabla F_{\lambda^*}(X), X\rangle - \lambda_{min}(\nabla F_{\lambda^*}(X) )N
\end{align}
In the first inequality we apply the convexity of $F_{\lambda^*}$.  In the second inequality we apply a standard inequality of frobenius inner product.  In the last inequality we use the fact that $\mathrm{Tr}(X^*) = N$.  
Rearranging we obtain for any $X$
\begin{align}
OPT \geq F_\lambda(X^*)
\geq F_{\lambda^*}(X)  - \langle \nabla F_{\lambda^*}(X), X\rangle + \lambda_{min}(\nabla F_{\lambda^*}(X) )N
\end{align}
Therefore it suffices to upper bound the two terms above $\langle \nabla F_{\lambda^*}(X), X\rangle$ and $\lambda_{min}(\nabla F_{\lambda^*}(X))$ which is an expression that holds for any $X$.  Given the output embeddings $\Tilde{V}$ of OptGNN (or indeed any set of vectors $\Tilde{V}$) let $\Tilde{X} = \Tilde{V}\Tilde{V}^T$. Then we have concluded   
\begin{align}
OPT \geq F_\lambda(X^*)
\geq F_{\lambda^*}(\Tilde{X})  - \langle \nabla F_{\lambda^*}(\Tilde{X}), \Tilde{X}\rangle + \lambda_{min}(\nabla F_{\lambda^*}(\Tilde{X}) )N
\end{align}
as desired.  
\end{proof}
Up to this point, every manipulation is formal proof.  Subsequently we detail how to make an educated 'guess' of the dual variables $\lambda^*$.  Although any guess will produce a bound, it won't produce a tight bound.  To be clear, solving for the optimal $\lambda^*$ would be the same as building an SDP solver which would bring us back into the expensive primal dual procedures that are involved in solving SDP's.  We are designing quick and cheap ways to output a dual certificate that may be somewhat looser.  Our scheme is simply to set $\lambda^*$ such that $\|\nabla F_{\lambda^*}(\Tilde{X})\|$ is minimized, ideally equal to zero.  The intuition is that if $(\Tilde{X}, \lambda^*)$ were a primal dual pair, then the lagrangian would have a derivative with respect to $X$ evaluated at $\Tilde{X}$ would be equal to zero.   
Let $H_\lambda(V)$ be defined as follows 
\begin{align*}
H_{\lambda^*}(\Tilde{V}) \defeq  \langle C,\Tilde{V}\Tilde{V}^T\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i) 
\end{align*}
We know the gradient of $H_{\lambda}(\Tilde{V})$
\begin{align*}
\nabla H_\lambda(\Tilde{V}) =  2(C + \sum_{i \in \mathcal{F}} \lambda^*_i A_i)\Tilde{V} = 2 \nabla F_\lambda(\Tilde{V}\Tilde{V}^T) \Tilde{V}
\end{align*}
Therefore it suffices to find a setting of $\lambda^*$ such that  $\|\nabla F_\lambda(\Tilde{X}) \Tilde{V}\|$ is small, ideally zero.  This would be a simple task, indeed a regression, if not for the unfortunate fact that OptGNN explicitly projects the vectors in $\Tilde{V}$ to be unit vectors.  This creates numerical problems such that minimizing the norm of $\|\nabla F_\lambda(\Tilde{X}) \Tilde{V}\|$ does not produce a $\nabla F_\lambda(\Tilde{X})$ with a large minimum eigenvalue.  

To fix this issue, let $R_{\eta,\rho} (V)$ denote the penalized lagrangian with quadratic penalties for constraints of the form $\langle A_i,X \rangle = b_i$ and linear penalty $\eta_i$ for constraints along the main diagonal of $X$ of the form $\langle e_ie_i^T, X\rangle = 1$.
\begin{align*}
    R_{\eta,\rho} (V) \defeq  \langle C,VV^T\rangle + \sum_{i \in \mathcal{J}} \rho (\langle A_i,VV^T\rangle - b_i)^2 + \sum_{i=1}^N \eta_i(\langle e_ie_i^T, VV^T\rangle - 1)
\end{align*}
Taking the gradient of $R_{\eta,\rho} (V)$ we obtain 
\begin{align*}
    \nabla R_{\eta,\rho} (V) \defeq  2CV + \sum_{i \in \mathcal{J}} 2\rho (\langle A_i,VV^T\rangle - b_i)A_i V + \sum_{i=1}^N 2\eta_i e_ie_i^TV
\end{align*}

Our rule for setting dual variables $\delta_i$ for $i \in \mathcal{J}$ is 
\[\delta_i \defeq  2\rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i)\] 

our rule for setting dual variables $\eta_j$ for $j \in [N]$ is 
\[\eta_j \defeq \frac{1}{2}\|e_j^T(C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i,VV^T\rangle - b_i)A_i) V \| \]

Then our full set of dual variables $\lambda^*$ is simply the concatenation $(\delta,\eta)$. Writing out everything explicitly we obtain the following matrix for $\nabla F_{\lambda^*}(\Tilde{V}\Tilde{V}^T)$

\begin{align*}
\nabla F_\lambda(\Tilde{V}\Tilde{V}^T) =  C + \sum_{i \in \mathcal{F}}  \rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2}\|e_j^T(C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i)A_i) \Tilde{V} \| e_ie_i^T  
\end{align*}
Plugging this expression into \lemref{lem:certificate} the final bound we evaluate in our code is 
\begin{multline}
OPT \geq \langle C,\Tilde{V}\Tilde{V}^T\rangle + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i)^2\\   - \Big\langle  C + \sum_{i \in \mathcal{F}}  \rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2}\|e_j^T(C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i)A_i) \Tilde{V} \| e_ie_i^T  , \Tilde{V}\Tilde{V}^T\Big\rangle\\
+ \lambda_{min}\Big( C + \sum_{i \in \mathcal{F}}  \rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2}\|e_j^T(C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i)A_i) \Tilde{V} \| e_ie_i^T  \Big)N
\end{multline}

Which is entirely computed in terms of $\Tilde{V}$ the output embeddings of OptGNN.  The resulting plot is as follows.     

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{cert50.png}
    \caption{N=50 p=0.1 SDP vs Opt-GNN Dual Certificate}
    \label{fig:cert50}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\linewidth]{cert100.png}
%     \caption{N=100 p=0.1 SDP vs Opt-GNN Dual Certificate}
%     \label{fig:cert100}
% \end{figure}
\textbf{Note:} The reason for splitting the set of dual variables is because the projection operator onto the unit ball is hard coded into the architecture of the lift network. Satisfying the constraint set via projection is different from the soft quadratic penalties on the remaining constraints and require separate handling.
\paragraph{Max Cut Certificate}
For Max Cut our dual variables are particularly simple as there are no constraints $\langle A_i,X\rangle = b_i$ for $b_i \neq 0$.  The dual variables for Max Cut take on the form for all $i \in [N]$
\begin{align*}
    \lambda^*_i = \frac{1}{2}\| \sum_{j \in N(i)} w_{ij}v_j\|    
\end{align*}

It's certainly possible to come up with tighter certification schemes which we leave to future work.    

\textbf{Intuition: } Near global optimality one step of the augmented method of lagrange multipliers ought to closely approximate the dual variables.  After obtaining a guess for the penalized lagrange multipliers we estimate the lagrange multipliers for the norm constraint by approximating $\nabla R_{\lambda}(V) = 0$.  The alternative would have been to solve the linear system for all the lagrange multipliers at once but this runs into numerical issues and degeneracies.   

\paragraph{Certificate Experiment: } We run our certification procedure which we name Opt-GNN-cert and compare it to the SDP certificate.  Note, that mathematically we will always produce a larger (i.e inferior) dual certificate in comparison to the SDP because we are bounding the distance to the SDP optimum with error in the gradients and hessians of the output embeddings of OptGNN.  Our advantage is in the speed of the procedure.  Without having to go through a primal dual solver, the entire time of producing Opt-GNN-cert is in the time required to feedforward through Opt-GNN. 
In this case we train an Opt-GNN-Max Cut with $10$ layers, on $1000$ Erdos-Renyi graphs, with $N=100$ nodes and edge density $p=0.1$.  We plot the Opt-GNN Max Cut value (an actual integer cut) on the x-axis and in the y-axis we plot the dual certificate value on the same graph where we compare the SDP certificate with the Opt-GNN-cert. See \ref{fig:cert50} for the $N=50$ graphs and \ref{fig:cert100} for the $N=100$ graphs.   

Note of course the dual certificate for any technique must be larger than the cut value outputted by Opt-GNN so the scatter plot must be above the $x=y$ axis of the plot.  We see as is mathematically necessary, the Opt-GNN-cert is not as tight as the SDP certificate but certainly competitive and more importantly it is arrived at dramatically faster. Without any attempt at optimizing the runtime, the Opt-GNN feedforward and certification takes no more than $0.02$ seconds whereas the SDP takes $0.5$ seconds on $N=100$ node graphs.       




\subsection{Miscellaneous Lemmas}
\label{sec:misc}
\begin{theorem}[perturbed-gd \cite{jin2017escape}] \label{thm:perturbed-gd} 
 Let $f$ be $\ell$-smooth (that is, it's gradient is $\ell$-Lipschitz) and have a $\gamma$-Lipschitz Hessian.  There exists an absolute constant $c_{max}$ such that for any $\delta \in (0,1), \epsilon \leq \frac{\ell^2}{\gamma}, \Delta_f \geq f(X_0) - f^*$, and constant $c \leq c_{max}$, $PGD(X_0, \ell, \gamma, \epsilon, c, \delta, \Delta_f)$ applied to the cost fucntion $f$ outputs a $(\gamma^2,\epsilon)$ SOSP with probability at least $1-\delta$ in 
\[
O\left( \frac{(f(X_0) - f^*)\ell}{\epsilon^2} \log^4\left(\frac{d\ell\Delta_f}{\epsilon^2\delta}\right) \right)
\]

iterations.  
\end{theorem}

\begin{definition} \label{def:sosp}[$(\gamma,\epsilon)$-second order stationary point] A $(\gamma,\epsilon)$ second order stationary point of a function $f$ is a point $x$ satisfying 
\[\|\nabla f(x)\| \leq \epsilon\]
\[\lambda_{min}(\nabla^2 f(x)) \geq -\sqrt{\gamma\epsilon}\]
\end{definition}

\begin{theorem}\label{thm:robustness}(Robustness Theorem 4.6 \citep{RSanycsp09} rephrased) Let $\mathbf{v}$ be a set of vectors satisfying the constraints of \sdpref{alg:sdp-vector} to additive error $\epsilon$ with objective $OBJ(\mathbf{v})$, then    
\[\text{SDPOBJ}(\Lambda) \geq OBJ(\mathbf{v}) - \sqrt{\epsilon} poly(kq)\]
\end{theorem}

\begin{corollary} \label{cor:optgnn}
Given a Max-k-CSP instance $\Lambda$, there is an OptGNN$_{(T,r,G_\Lambda)}(\mathbf{v})$  with $T = poly(\delta^{-1},\epsilon^{-1},|\mathcal{P}|q^k)$ layers, $r = |\mathcal{P}|q^k$ dimensional embeddings, with learnable parameters $\{M_{1,t}\}_{t \in [T]}$ and $\{M_{2,t}\}_{t \in [T]}$ that outputs a set of vectors $\bold{v}$ satisfying the constraints of \sdpref{alg:sdp-vector} and approximating its objective, $\text{SDPOBJ}(\Lambda)$, to error $\epsilon$ with probability $1-\delta$. 
\end{corollary}

\begin{proof}
The proof is by inspecting the definition of OptGNN in the context of \thmref{thm:main}.  
\end{proof}

\begin{corollary} The OptGNN of \corref{cor:optgnn} , which by construction is equivalent to \Algref{alg:message-passing}, outputs a set of embeddings $\mathbf{v}$ such that the rounding of \cite{RSanycsp09} outputs an integral assignment $\mathcal{V}$ with a Max-k-CSP objective OBJ($\mathcal{V}$) satisfying 
$OBJ(\mathcal{V}) \geq S_{\Lambda}(\text{SDPOBJ}(\Lambda)-\epsilon)-\epsilon$ in time $\text{exp}(\text{exp}(\text{poly}(\frac{kq}{\epsilon})))$ which approximately dominates the Unique Games optimal approximation ratio.    
\end{corollary}

\begin{proof}
The proof follows from the robustness theorem of \cite{RSanycsp09} which states that any solution to the SDP that satisfies the constraints approximately does not change the objective substantially \thmref{thm:robustness}.      
\end{proof}

\section{Experiment details} \label{app:experimental_setup}
In this section we give further details on our experimental setup.


\paragraph{Datasets.}
Our experiments span a variety of randomly generated and real-world datasets. Our randomly generated datasets contain graphs from several random graph models, in particular Erd\H{o}s-R\'enyi (with $p=0.15$), Barab\'asi–Albert (with $m=4$), Holme-Kim (with $m=4$ and $p=0.25$), and Watts-Strogatz (with $k=4$ and $p=0.25$). Our real-world datasets are ENZYMES, PROTEINS, MUTAG, IMDB-BINARY, COLLAB (which we will together call \textbf{TU-small}), and REDDIT-BINARY, REDDIT-MULTI-5K, and REDDIT-MULTI-12K (which we will call \textbf{TU-REDDIT}).

We abbreviate the generated datasets using their initials and the range of vertex counts. For example, by ER (50,100) we denote Erd\H{o}s-R\'enyi random graphs with a vertex count drawn uniformly at random from [50, 100]. In tables, we mark generated datasets with superscript \textsuperscript{a}, \textbf{TU-small} with \textsuperscript{b}, and \textbf{TU-REDDIT} with \textsuperscript{c}.

\paragraph{Baselines.}
We compare the performance of our approach against knwon classical algorithms. In terms of classical baselines, we run Gurobi with varying timeouts and include SDP results on smaller datasets. 
% % SDP scales extremely poorly with graph size so we omit the results for datasets with larger graphs. 
% For minimum Vertex Cover, we include the classical baseline KaMIS, a maximum independent set solver. 

We also include a greedy baseline, which is the function \texttt{one\_exchange} (for Maximum Cut) or \texttt{min\_weighted\_vertex\_cover} (for minimum Vertex Cover) from \texttt{networkx}~\citep{networkx}.

% Our neural baselines include LwD~\citep{ahn2020learning} and \textsc{Dgl-TreeSearch}~\citep{li2018combinatorial,bother2022s}.

\paragraph{Validation and test splits.}
For each dataset we hold out a validation and test slice for evaluation.
In our generated graph experiments we set aside 1000 graphs each for validation and testing. Each step of training ran on randomly generated graphs. For \textbf{TU-small}, we used a train/validation/test split of 0.8/0.1/0.1. For \textbf{TU-REDDIT}, we set aside 100 graphs each for validation and testing.

\paragraph{Scoring.}
To measure a model's score on a graph, we first run the model on the graph to generate an SDP output, and then round this output to an integral solution using 1,000 random hyperplanes. We ran validation periodically during each training run and retained the model that achieved the highest validation score. Then for each model and dataset, we selected the hyperparameter setting that achieved the highest validation score, and we report the average score measured on the test slice. Please see \autoref{sec:hyperparams} for further details on the hyperparameter ranges used.




\paragraph{Hardware.}
Our training runs used 20 cores of an Intel Xeon Gold 6248 (for data loading and random graph generation) and a NVIDIA Tesla V100 GPU.
Our Gurobi runs use 8 threads on a Intel Xeon Platinum 8260.
Our KaMIS runs use an Intel Core i9-13900H.
Our LwD and \textsc{Dgl-TreeSearch} runs use an Intel Core i9-13900H and an RTX 4060.

\begin{SCtable}[][!htbp]
\begin{tabular}{llll}
\toprule
    Parameter & Generated & \textbf{TU-small} & \textbf{TU-REDDIT} \\
\midrule
    Gradient steps & 20,000 & 100,000 & 100,000 \\
    Validation freq & 1,000 & 1,000 & 2,000 \\
    Batch size & 16 & 16 & 16 \\
    Ranks & 4, 8, 16, 32 & 4, 8, 16, 32 & 4, 8, 16, 32 \\
    Layer counts & 8, 16 & 8, 16 & 8, 16 \\
    Positional encodings & RW & LE, RW & RW \\
\midrule
    \textbf{Run count} & 8 & 16 & 8 \\
\bottomrule
\end{tabular}
\caption{Hyperparameter range explored for each group of datasets. For each NN architecture, when training on a dataset, we explored every listed hyperparameter combination in the corresponding column.}
\label{tab:hyperparams}
\end{SCtable}

\paragraph{Hyperparameters.}\label{sec:hyperparams}
We ran each experiment on a range of hyperparameters. See \autoref{tab:hyperparams} for the hyperparameter listing. For all training runs, we used the Adam optimizer~\cite{kingma2014adam} with a learning rate of 0.001. We used Laplacian eigenvector~\cite{dwivedi2020benchmarking} (LE) or random walk~\cite{dwivedi2021graph} (RW) positional encoding with dimensionality of half the rank, except for rank 32 where we used 8 dimensions.

\begin{SCtable}[][!htbp]
\small
\input{maxcut_ratio_baseline.tex}
\caption{Performance of OptGNN compared to Gurobi running under an 8 second time limit, expressed as a ratio. For each dataset, we take the ratio of the integral values achieved by OptGNN and Gurobi 8s on each of the graphs in the test slice. We present the average and standard deviation of these ratios. Here, higher is better. This table demonstrates that OptGNN achieves nearly the same performance, missing on average 1.1\% of the cut value in the worst measured case.}
\label{tab:cut_ratios}
\end{SCtable}

\begin{SCtable}[][!htbp]
\small
\input{VC_ratio_baseline.tex}
\caption{Performance of OptGNN compared to Gurobi running under an 8 second time limit, expressed as a ratio. For each dataset, we take the ratio of the integral values achieved by OptGNN and Gurobi 8s on each of the graphs in the test slice. We present the average and standard deviation of these ratios. Here, lower is better. This table demonstrates that OptGNN achieves nearly the same performance, producing a cover on average 3.1\% larger than Gurobi 8s in the worst measured case.}
\label{tab:VC_ratios}
\end{SCtable}

%\begin{table}[!htbp]
%\small
%\input{maxcut_ratio_model.tex}
%\caption{Performance of various model architectures for selected datasets on Maximum Cut. Here, higher is better.}
%\label{tab:cut_ratio_models}
%\end{table}

%\begin{table}[!htbp]
%\small
%\input{VC_ratio_model.tex}
%\caption{Performance of various model architectures for selected datasets on minimum Vertex Cover. Here, lower is better.}
%\label{tab:VC_ratio_models}
%\end{table}

\subsection{Ratio tables}
In \autoref{tab:cut_ratios} and \autoref{tab:VC_ratios} we supply the performance of OptGNN as a ratio against the integral value achieved by Gurobi running with a time limit of 8 seconds. These tables include the standard deviation in the ratio. We note that for Maximum Cut, OptGNN comes within 1.1\% of the Gurobi 8s value, and for minimum Vertex Cover, OptGNN comes within 3.1\%.

\begin{table}[!htbp]
\small
\centering
\input{VC_model_table.tex}
\caption{Performance of various model architectures compared to OptGNN for selected datasets on Minimum Vertex Cover. Here, lower is better.}
\label{tab:VC_models}
\end{table}

\subsection{Vertex cover alternative architectures}\label{sec:VC_ablation}
\autoref{tab:VC_models} presents the performance of alternative neural network architectures on minimum vertex cover.

\subsection{Effects of hyperparameters on performance}
\autoref{fig:hparam_vc_tusmall}, \autoref{fig:hparam_vc_generated}, \autoref{fig:hparam_mc_tusmall}, and \autoref{fig:hparam_mc_generated} present overall trends in model performance across hyperparameters.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{hparam_vc_tusmall.png}
    \caption{Trends in model performance with respect to the number of layers, hidden size, and positional encoding of the models.}
    \label{fig:hparam_vc_tusmall}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{hparam_vc_generated.png}
    \caption{Trends in model performance with respect to the number of layers, hidden size, and positional encoding of the models.}
    \label{fig:hparam_vc_generated}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{hparam_mc_tusmall.png}
    \caption{Trends in model performance with respect to the number of layers, hidden size, and positional encoding of the models.}
    \label{fig:hparam_mc_tusmall}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{hparam_mc_generated.png}
    \caption{Trends in model performance with respect to the number of layers, hidden size, and positional encoding of the models.}
    \label{fig:hparam_mc_generated}
\end{figure}



\subsection{Generalizability}
Models trained on one dataset work quite well on other datasets, suggesting that models have good ability to generalize to examples outside their training distribution. Please see \autoref{tab:generalization}.

\include{sat.tex}
\include{alignment.tex}
\include{hessian.tex}

% \begin{tabular}{llrrrr}
% \toprule
%             Dataset &         OptGNN &  Greedy & {Gurobi}& Gurobi & Gurobi \\
%               &             &      &     0.1s &     1.0s &     8.0s \\
% \midrule
% BA\textsuperscript{a} (400,500) &   2197.99 (66) & 1255.22 &  2208.11 &  2208.11 &  2212.49 \\
% ER\textsuperscript{a} (400,500) & 16387.46 (225) & 8622.34 & 16476.72 & 16491.60 & 16495.31 \\
% HK\textsuperscript{a} (400,500) &   2159.90 (61) & 1230.98 &  2169.46 &  2169.46 &  2173.88 \\
% WC\textsuperscript{a} (400,500) &   1166.47 (78) &  690.19 &  1173.45 &  1175.97 &  1179.86 \\
%       COLLAB\textsuperscript{b} &   2622.41 (22) & 1345.70 &  2624.32 &  2624.57 &  2624.62 \\
%  REDDIT-M-5K\textsuperscript{c} &   786.09 (133) &  495.02 &   785.44 &   787.48 &   787.92 \\
% \bottomrule
% \end{tabular}



% \begin{tabular}{llrrrr}
% \toprule
%             Dataset &      OptGNN & Greedy &  {Gurobi}& Gurobi & Gurobi \\
%               &          &     &   0.1s &   1.0s &   8.0s \\
% \midrule
% BA\textsuperscript{a} (400,500) & 248.74 (27) & 302.53 & 256.33 & 246.49 & 246.46 \\
% ER\textsuperscript{a} (400,500) & 420.70 (41) & 442.84 & 423.07 & 423.07 & 415.52 \\
% HK\textsuperscript{a} (400,500) & 249.26 (27) & 298.98 & 247.90 & 247.57 & 247.57 \\
% WC\textsuperscript{a} (400,500) & 274.21 (31) & 434.52 & 269.58 & 269.39 & 269.39 \\
% COLLAB\textsuperscript{b} &  67.50 (23) &  71.74 &  67.47 &  67.46 &  67.46 \\ REDDIT-M-5K\textsuperscript{c} & 107.36 (33) & 153.24 & 108.73 & 107.32 & 107.32 \\
% \bottomrule
% \end{tabular}

==> icml.tex <==
\textbf{Min-Vertex-Cover experiments.}
We evaluated OptGNN on forced RB instances, which are hard vertex cover instances from the RB random CSP model that contain hidden optimal solutions \citep{xu2007random}. We considered two forced RB distributions, RB200 and RB500, as specified in prior work \citep{wang2023unsupervised}. The results are in \autoref{tab:forced_rb}, which also includes the performance of several neural and classical baselines as reported in \citep{wang2023unsupervised,brusca2023maximum}. OptGNN consistently outperforms state-of-the-art unsupervised baselines on this task and is even able to match the performance of Gurobi with a 0.5s time limit.

\textbf{Max-3-SAT experiment and ablation.}
The purpose of this experiment is twofold: to demonstrate the viability of OptGNN on the Max-3-SAT problem and to examine the role of overparameterization in OptGNN.
We generate 3-SAT formulae on the fly with 100 variables and a random number of clauses in the $[400, 430]$ interval, and train OptGNN for 100,000 iterations. We then test on instances with 100 variables and $\{400,415,430\}$ clauses. The results are in \autoref{tab:sat_baselines}. 
We compare with WalkSAT, a classic local search algorithm for SAT, and ErdosGNN \cite{karalias2020erdos}, a neural baseline trained in the same way. Furthermore, we compare with a simple baseline reported as \enquote{Autograd} that implements gradient descent directly on the Lagrangian. For details see \ref{sec:autograd}. OptGNN is able to outperform Erd\H{o}sGNN consistently and improves significantly over Autograd, which supports the overparameterized message passing of OptGNN.

\textbf{Max-Cut experiments.} \autoref{tab:cut_baselines} presents a comparison between OptGNN, a greedy algorithm, and Gurobi for Max-Cut. OptGNN is competitive with Gurobi when run on a similar time budget and clearly outperforms greedy on all datasets. For results on more datasets see \ref{sec:complete-results}.
We generated Erd\H{o}s-Renyi graphs $\mathcal{G}_{n,p}$ for $n\in [400,500]$ and $p=0.15$ on the fly and trained an OptGNN for 20k iterations. \autoref{tab:cut_neural} shows test results on GSET benchmark instances \citep{benlic2013breakout}.
Furthermore, we report the performance for several other baselines, including a greedy algorithm, the Goemans-Williamson SDP, and neural baselines. We can see that OptGNN consistently outperforms the SDP and the greedy algorithm, while also being competitive with the neural baselines. However, OptGNN is not able to outperform ANYCSP, which to the best of our knowledge achieves the current state-of-the-art results.

\begin{table}%[!htbp]
\centering
\scriptsize
\input{maxcut_neural}
\caption{Comparison on GSET instances for Max-Cut against state of the art neural baselines. Numbers reported are the mean deviations from the best known Max-Cut values, reported as $f_\text{best}$ in table 2 of \cite{benlic2013breakout}. Lower is better.}
\label{tab:cut_neural}
\end{table}

\iffalse
% XXX DO NOT INCLUDE THIS FOR NOW; IT CONTRADICTS APPENDIX D
% \begin{table*}[!htbp]
% \centering
% \begin{tabular}{llll}
% \toprule
% Dataset       & KaMIS          & LwD           & OptGNN (trained on (400, 500)) \\
% \midrule
% ER (500, 500) & 459.39 (10.39) & 466.98 (0.23) & 470.52 (0.049) \\\midrule

% BA (500, 500) & 292.83 (2.07)  & 293.27 (0.23) & 297.67 (0.026) \\\midrule

% HK (500, 500) & 391.71 (9.68)  & 394.28 (0.27) & 455.82 (0.046) \\ \midrule

% WS (500, 500) & 432.5 (4.57)   & 443.78 (0.27) & 479.11 (0.037) \\ \midrule
% \end{tabular}
% \caption{PROLLY NOT GONNA HAVE THIS IN unless we get fresh numbers on optgnn. Comparison against KaMIS and LwD on various randomly generated instances.
% Numbers reported are the Vertex-Cover set sizes found by each method.
% We report the best test score achieved by any of our models trained on the (400, 500) version of the corresponding dataset.
% So the scores we report are not exactly an apples to apples comparison; especially for HK and WS the gap is clear.}
% \end{table*}
\fi

\textbf{Out of distribution generalization.}
We tested OptGNN's ability to perform well on data distributions (for the same optimization problem) that it was not trained on. We test this using a collection of different datasets. The results can be seen in table \ref{tab:generalization} and \autoref{sec:oodtest}. Overall, the results show that the model is capable of performing well even on datasets it has not been trained on.

\textbf{Model ablation.}
We train modern GNN architectures from the literature with the same loss function and compare them against OptGNN. Please see \ref{sec:VC_ablation} for more details and results on multiple datasets for two different problems. Overall, OptGNN is the best performing model on both problems across all datasets.

\begin{figure}%[!htbp]
    \centering
    \includegraphics[width=0.6\linewidth]{cert100.png}
    \caption{Experimental comparison of SDP versus OptGNN Dual Certificates on random graphs of 100 nodes for the Max-Cut problem. Our OptGNN certificates track closely with the SDP certificates while taking considerably less time to generate.}
    \label{fig:cert100}
\end{figure}

\subsection{Experimental demonstration of neural certificates.} \label{sec:certificates-experiment}
In this section, we provide a simple experimental example of our neural certificate scheme on small synthetic instances.
Deploying this scheme on Max-Cut on random graphs, we find this dual certificate to be remarkably tight. An example can be seen in  \figref{fig:cert100}. For $100$ node graphs with $1000$ edges our certificates deviate from the SDP certificate by about $20$ nodes but are dramatically faster to produce.  The runtime is dominated by the feedforward of OptGNN which is $0.02$ seconds vs. the SDP solve time which is $0.5$ seconds on cvxpy.  See \ref{sec:certificate} for extensive discussion and additional results.

\section{Conclusion}
We have presented OptGNN, a GNN that can capture provably optimal message passing algorithms for a large class of combinatorial optimization problems. OptGNN achieves the appealing combination of obtaining approximation guarantees while also being able to adapt to the data to achieve improved results. Empirically, we observed that the OptGNN architecture achieves strong performance on a wide range of datasets and on multiple problems. OptGNN opens up several directions for future exploration, such as the design of more powerful and sound (neural) rounding procedures that can secure approximation guarantees, the construction of neural certificates that improve upon the ones we described in Appendix \ref{sec:certificate}, and the design of neural SDP-based branch and bound solvers. 

\section{Impact Statement}
This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here.
 % \section{Acknowledgment} 

 % The authors would like to thank Ankur Moitra, Sirui Li, and Zhongxia Yan for insightful discussions in the preparation of this work.  Nikolaos Karalias is funded by the SNSF, in the context of the project "General neural solvers for combinatorial optimization and algorithmic reasoning" (SNSF grant number: P500PT\_217999). Stefanie Jegelka acknowledges support from NSF award 1900933 and NSF AI Institute TILOS (NSF CCF-2112665).


% Striving for simplicity, we opted for a rudimentary approach to rounding that was able to yield efficient high quality solutions. This can certainly be improved by considering more sophisticated rounding algorithms from the literature or perhaps by adding learnable components to that part of the pipeline.



% We leave the generalization and extension of this technique as an avenue for future work. 


% \clearpage
% \bibliography{iclr2024_conference}
% \bibliographystyle{iclr2024_conference}


\nocite{langley00}

\bibliography{iclr2024_conference}
%\bibliographystyle{icml2024}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% APPENDIX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\appendix
\onecolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Min-Vertex-Cover OptGNN}
\label{sec:vertex-cover}
Min-Vertex-Cover can be written as the following integer program 
\begin{align} 
\text{Minimize:} \quad & \sum_{i \in [N]} \frac{1+x_i}{2} \\
\text{Subject to:} \quad & (1-x_i)(1-x_j) = 0 \quad \forall (i,j) \in E \\
& x_i^2 = 1 \quad \forall i \in [N]
\end{align}
To deal with the constraint on the edges $(1-x_i)(1-x_j) = 0$, we add a quadratic penalty to the objective with a penalty parameter $\rho > 0$ yielding
\begin{align} 
\text{Minimize:} \quad & \sum_{i \in [N]} \frac{1+x_i}{2} + \rho \sum_{(i,j) \in E} (1 - x_i - x_j + x_ix_j)^2 \\
\text{Subject to:} \quad & x_i^2 = 1 \quad \forall i \in [N]
\end{align}

Analogously to Max-Cut, we adopt a natural low rank vector formulation for vectors $\mathbf{v} = \{v_i\}_{i \in [N]}$ in $r$ dimensions. 
\begin{align} 
\text{Minimize:} \quad &  \sum_{i \in [N]} \frac{1+\langle v_i,v_{\emptyset}\rangle}{2} + \rho\sum_{(i,j) \in E} (1 - \langle v_i,v_{\emptyset}\rangle - \langle v_j,v_{\emptyset}\rangle + \langle v_i,v_j \rangle)^2\\
\text{Subject to:} \quad & \|v_i\| = 1 \quad v_i \in \R^r \quad \forall i \in [N]
\end{align}

Now we can design a simple projected gradient descent scheme as follows.  For iteration $t $ in max iterations $T$, and for vector $v_i$ in $\mathbf{v}$ we perform the following update.   

\begin{equation}
\hat{v}_i^{t+1} \defeq v_i^t - \eta \big( v_{\emptyset} + 2\rho \sum_{j \in N(i)}(1 - \langle v_i^t,v_{\emptyset}\rangle - \langle v_j^t,v_{\emptyset}\rangle + \langle v_i^t,v_j^t \rangle)(-v_{\emptyset} + v_j^t)  \big)
\end{equation}
\begin{equation}
v_i^{t+1} \defeq \frac{\hat{v}_i^{t+1}}{ \|\hat{v}_i^{t+1}\|}
\end{equation}

We can then define a $\text{OptGNN}_{(M,G)}$ analogously with learnable matrices $M = \{M_{t}\}_{t \in [T]} \in \R^{r \times 2r}$ which are each sets of $T$ learnable matrices corresponding to $T$ layers of neural network. 
Let the message from node $v_j$ to node $v_i$ be
\[\text{MESSAGE}[v_j \rightarrow v_i] \defeq 2\rho (1 - \langle v_i^t,v_{\emptyset}\rangle - \langle v_j^t,v_{\emptyset}\rangle + \langle v_i^t,v_j^t \rangle)(-v_{\emptyset} + v_j^t)  \big)\]
Let the aggregation function $\text{AGG}$ be defined as 
\[
\text{AGG}(\{v_j^t\}_{j \in N(i)}) \defeq \begin{bmatrix}
v_i^t \\
\sum_{j \in N(i)} \text{MESSAGE}[v_j \rightarrow v_i]
\end{bmatrix}
\]
Then for layer $t$ in max iterations $T$, for $v_i$ in $\mathbf{v}$, we have   
\begin{equation} \label{eq:vc-pgd}
\hat{v}_i^{t+1} \defeq M\left( \text{AGG}(v_i^t)\right) 
\end{equation}
\begin{equation}
v_i^{t+1} \defeq \frac{\hat{v}_i^{t+1}}{ \|\hat{v}_i^{t+1}\|}
\end{equation}
This approach can be straightforwardly adopted to compute the maximum clique and the maximum independent set.


\include{sat.tex}
%\include{optimality}

\section{Optimality of Message Passing for Max-CSP} \label{sec:message-passing}

Our primary theoretical result is that a polynomial time message passing algorithm  on an appropriately defined constraint graph computes the approximate optimum of \sdpref{alg:sdp-vector} which is notable for being an SDP that achieves the Unique Games optimal integrality gap.  

Our proof roadmap is simple. First, we design an SDP relaxation \sdpref{alg:sdp-vector} for Max-k-CSP that is provably equivalent to the SDP of \cite{raghavendra2008optimal} and therefore inherits its complexity theoretic optimality.  Finally, we design a message passing algorithm to approximately solve \sdpref{alg:sdp-vector} in polynomial time to polynomial precision. Our message passing algorithm has the advantage of being formulated on an appropriately defined constraint graph.  For a Max-k-CSP instance $\Lambda$ with $N$ variables, $|\mathcal{P}|$ predicates, over an alphabet of size $q$, it takes $|\mathcal{P}|q^k$ space to represent the Max-CSP.  To declutter notation, we let $\Phi$ be the size of the Max-CSP which is equal to $|\mathcal{P}|q^k$ .  Our message passing algorithm achieves an additive $\epsilon$ approximation in time $poly(\epsilon^{-1},\Phi,\log(\delta^{-1}))$ which is then polynomial in the size of the CSP and inverse polynomial in the precision.      

Here we briefly reiterate the definition of Max-k-CSP.  A Max-k-CSP instance $\Lambda = (\mathcal{V}, \mathcal{P}, q)$ consists of a set of $N$ variables $\mathcal{V} \defeq \{x_i\}_{i \in [N]}$ each taking values in an alphabet $[q]$ and a set of predicates $\mathcal{P} \defeq \{P_z\}_{z \subset \mathcal{V}}$ where each predicate is a payoff function over $k$ variables denoted $z = \{x_{i_1}, x_{i_2}, ..., x_{i_k}\}$.  Here we refer to $k$ as the arity of the Max-k-CSP, and we adopt the normalization that each predicate $P_z$ returns outputs in $[0,1]$.  We index each predicate $P_z$ by its domain $z$ and we will use the notation $\mathcal{S}(P)$ to denote the domain of a predicate $P$.  The goal of Max-k-CSP is to maximize the payoff of the predicates.   

\begin{equation} \label{eq:csp-obj}
\max_{(x_1,...,x_N) \in [q]^N} \frac{1}{|\mathcal{P}|}\sum_{P_z \in \mathcal{P}} P_z(X_z) 
\end{equation}

Where $X_z$ denotes the assignment of variables $\{x_i\}_{i \in z}$.  

There is an SDP relaxation of \eqref{eq:csp-obj} that is the "qualitatively most powerful assuming the Unique Games conjecture" \cite{raghavendra2008optimal}. More specifically, the integrality gap of the SDP achieves the Unique Games optimal approximation ratio.  Furthermore, there exists a rounding that achieves its integrality gap.

\paragraph{SDP Reformulation: } Next we will introduce the SDP formulation we adopt in this paper.  For the sake of exposition and notational simplicity, we will work with binary Max-k-CSP's where $q = \{0,1\}$.  The extension to general $q$ is straightforward and detailed in the appendix.

We will adopt the standard pseudoexpectation and pseudodistribution formalism in describing our SDP.  
Let $\pE_\mu[\mathbf{x}]$ be a matrix in dimension $\R^{(N+1)^{d/2} \times (N+1)^{d/2}}$ of optimization variables defined as follows

\begin{align}
\pE_\mu[\mathbf{x}] \defeq \pE_\mu[(1,x_1,x_2,...,x_N)^{\otimes d/2} \big((1,x_1,x_2,...,x_N)^{\otimes d/2}\big)^T]
\end{align}
Where we use $\otimes$ to denote tensor product.  It is convenient to think of  $\pE_\mu[\mathbf{x}]$ as a matrix of variables denoting the up to $d$ multilinear moments of a distribution $\mu$ over the variables $\mathcal{V}$.  A multilinear  polynomial is a polynomial of the form $X_\phi \defeq \prod_{i \in \phi} x_i$ for some subset of the variables $\phi \subseteq \mathcal{V}$.  We index the variables of the matrix $\pE_\mu[\mathbf{x}]$ by the multilinear moment that it represents.  Notice that this creates repeat copies as their are multiple entries representing the same monomial.  This is dealt with by constraining the repeated copies to be equal with linear equality constraints.    

Specifically, let $z$ be a subset of the CSP variables $z \subset \{x_i\}_{i \in [N]}$ of size $k$.  Let $X_z$ denote the multilinear moment $X_z \defeq \prod_{i \in z} x_i$.  Then $\pE_\mu[X_z]$ denotes the SDP variable corresponding to the multilinear moment $\E_{\mu}[X_{z}]$.  Of course optimizing over the space of distributions $\mu$ over $\mathcal{V}$ is intractable, and so we opt for optimizing over the space of low degree pseudodistributions and their associated pseudoexpecation functionals.  See \cite{barak2014sum} for references therein.       

In particular, for any subset of variables $X_{z} \defeq \{x_{i_1},...,x_{i_k}\} \in \mathcal{V}$ we let $\pE_\mu[\mathbf{x}]\big|_{z,d}$ denote the matrix of the up to degree up to $d$ multilinear moments of the variables in $z$.

\begin{align}
\pE_\mu[\mathbf{x}]\big|_{z,d} \defeq \pE_\mu[(1,x_{i_1},x_{i_2},...,x_{i_k})^{\otimes d/2} \big((1,x_{i_1},x_{i_2},...,x_{i_k})^{\otimes d/2}\big)^T]
\end{align}   
We refer to the above matrix as a degree $d$ pseudoexpectation funcitonal over $X_z$.  Subsequently, we describe a pseudoexpectation formulation of our SDP followed by a vector formulation.
\paragraph{Multilinear Formulation:}A predicate for a boolean Max-k-CSP $P_z(X_z)$ can be written as a multilinear polynomial

\begin{align} \label{eq:defpz}
P_z(X_z) \defeq \sum_{\tau = (\tau_1,...,\tau_k) \in \{-1,1\}^k} w_{z,\tau}\prod_{x_i \in z} \frac{1+\tau_i x_i}{2} \defeq \sum_{s \subseteq z} y_sX_s
\end{align}
For some real valued weights $w_{z,\tau}$ and $y_s$ which are simply the fourier coefficients of the function $P_z$.  Then the pseudoexpectation formulation of our SDP is as follows
\begin{equation} \label{eq:sdp-obj}
\max_{\pE_{\mu}[\mathbf{x}]} \frac{1}{|\mathcal{P}|}\sum_{P_z \in \mathcal{P}} \pE_{\mu}[P_z(X_z)] 
\end{equation}

subject to the following constraints 
\begin{enumerate}
    \item \textbf{Unit: } $\pE_\mu[1] = 1$,  $\pE_\mu[x_i^2] = 1$ for all $x_i \in \mathcal{V}$, and $\pE_\mu[\prod_{i \in s} x_i^2 \prod_{j \in s'} x_j] = \pE_\mu[\prod_{j \in s'} x_j]$ for all $s,s' \subseteq \mathcal{S}(P)$ for every predicate $P \in \mathcal{P}$ such that $2s + s' \leq k$.  In expectation, the squares of all multilinear polynomials are equal to $1$.     
    \item \textbf{Positive Semidefinite: } $\pE_\mu[\mathbf{x}]|_{\mathcal{V},2} \succeq 0$ i.e the degree two pseudoexpectation is positive semidefinite. 
 $\pE_\mu[\mathbf{x}]\big|_{z,2k} \succeq 0$ for all $z = \mathcal{S}(P)$ for all $P \in \mathcal{P}$. The moment matrix for the multilinear polynomials corresponding to every predicate is positive semidefinite.     
\end{enumerate}

Equivalently we can view the SDP in terms of the vectors in the cholesky decomposition of $\pE_\mu[\mathbf{x}]$.  We rewrite the above SDP accordingly.  For this purpose it is useful to introduce the notation $\zeta(A,B) \defeq A \cup B / A \cap B$.  It is also useful to introduce the notation $\mathcal{C}(s)$ for the size of the set $\{g,g' \subseteq s: \zeta(g,g') = s\}$.    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM BLOCK
% \makeatletter
% \renewcommand{\ALG@name}{CSP-SDP}
% \makeatother
%\begin{SDPOPT}[tb]
\begin{SDPOPT}
\label{alg:sdp-vector}
\setcounter{algorithm}{0}
\caption{SDP for Max-k-CSP (Equivalent to UGC-optimal)}
\begin{algorithmic} \label{alg:sdp-vector}
\STATE{SDP Vector Formulation} {$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}. Multilinear formulation of objective.
\begin{align}  
\min_{x_1,x_2,\dots,x_N}  & \frac{1}{|\mathcal{P}|}\sum_{P_z \subset \mathcal{P}} \pE_{\mu}[-P_z(X_z)]  \defeq \sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} w_s\frac{1}{|\mathcal{C}(s)|}\sum_{g,g' \subseteq s: \zeta(g,g') = s} \langle v_{g}, v_{g'}\rangle \\
\text{subject to:} 
& \; \|v_{s}\|^2 = 1 \quad \forall s \subseteq \mathcal{S}(P) \text{, } \forall P \in \mathcal{P} \\
& \; \pE_\mu[X_{\zeta(g,g')}] \defeq \langle v_g,v_{g'} \rangle & \nonumber \\
& \quad \quad \quad \quad \quad \; \; = \langle v_{h}, v_{h'}\rangle \quad \forall \zeta(g,g') = \zeta(h,h') \; \text{ s.t } \; g \cup g' \subseteq \mathcal{S}(P), \;\forall P \in \mathcal{P} %\\
\end{align}
\STATE{First constraint is the square of multilinear polynomials are unit.\\
Second constraint are degree $2k$ SoS constraints for products of multilinear polynomials.}
\end{algorithmic}
\end{SDPOPT} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM BLOCK

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM BLOCK
% \begin{algorithm}[tb]
%    \caption{Bubble Sort}
%    \label{alg:example}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} data $x_i$, size $m$
%    \REPEAT
%    \STATE Initialize $noChange = true$.   
%    \FOR{$i=1$ {\bfseries to} $m-1$}
%    \IF{$x_i > x_{i+1}$}
%    \STATE Swap $x_i$ and $x_{i+1}$
%    \STATE $noChange = false$
%    \ENDIF
%    \ENDFOR
%    \UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

\begin{lemma}
For Max-k-CSP instance $\Lambda$, The SDP of \sdpref{alg:sdp-vector} (top of pg.19) is at least as tight as the SDP of \cite{raghavendra2008optimal}.  
\end{lemma}
\begin{proof}
The SDP of \cite{raghavendra2008optimal} is a degree $2$ SoS SDP augmented with $k$-local distributions for every predicate $P \in \mathcal{P}$.  By using the vectors of the cholesky decomposition and constraining them to be unit vectors  we automatically capture degree $2$ SoS.  To capture $k$ local distributions we simply enforce degree $2k$ SoS on the boolean hypercube for the domain of every predicate.  This can be done with the standard vector formulation written in \sdpref{alg:sdp-vector} (top of pg.18).  See \cite{barak2014sum} for background and references.       
\end{proof}
Moving forward, the goal of \Algref{alg:message-passing} is to minimize the loss $\mathcal{L}_\rho(\mathbf{v})$ which is a function of the Max-CSP instance $\Lambda$.  
\begin{multline} \label{eq:main-loss}
\mathcal{L}_\rho(\mathbf{v}) = \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\ \text{s.t }\zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle\\ 
+ \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 \\
+\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}
The loss $\mathcal{L}_\rho$ has gradient of the form 
\begin{multline} \label{eq:loss-grad}
\frac{\partial \mathcal{L}_\rho(\mathbf{v})}{\partial v_w}  = \frac{1}{|\mathcal{P}|}\Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t } w \subseteq z}} \sum_{\substack{s \subseteq z\\\text{s.t } w \subseteq s}} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{w' \subseteq s\\ \text{s.t } \zeta(w,w') = s}} v_{w'}\\ 
+ 2\rho \Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t } w \subseteq z}} \sum_{\substack{w',h,h' \subseteq s\\ \text{s.t } \zeta(w,w') = \zeta(h,h')}} \big(\langle v_w,v_{w'}\rangle - \langle v_h, v_{h'}\rangle\big) v_w' \\
+(\| v_w\|^2 - 1)v_w\Bigg]\Bigg]
\end{multline} 
Noticing that the form of the gradient depends only on the vectors in the neighborhood of the constraint graph $G_\Lambda$ we arrive at our message passing algorithm.  The key to our proof is bounding the number of iterations required to optimize \eqref{eq:main-loss} to sufficient accuracy to be an approximate global optimum of \sdpref{alg:sdp-vector}.  
% % \makeatletter
% % \renewcommand{\ALG@name}{Algorithm}
% % \makeatother
\begin{algorithm}[!h] 
%\setcounter{algorithm}{1}
\caption{Message Passing for Max-CSP}
\label{alg:message-passing} %\setcounter{algorithm}{0}
\begin{algorithmic}[1]
%\Procedure{Message Passing}{$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}
\STATE \textbf{Inputs: Max-CSP instance $\Lambda$}\\
\STATE $n \gets \Phi \log(\delta^{-1})$
\STATE $\eta, \psi, \sigma \gets n^{-100}$ \quad \quad \quad \quad \quad \quad  \quad \quad \quad\quad \quad \quad \COMMENT{Initialize step size, noise threshold, and noise variance}
\STATE $\mathbf{v}^0 = \{v_s\}_{s \subseteq z: P_z \in \mathcal{P}} \gets Uniform(\mathcal{S}^{n-1})$ \quad \quad \quad \COMMENT{Initialize vectors to uniform on the unit sphere}
\FOR{$t \in [poly(\epsilon^{-1},\Phi,\log(\delta^{-1}))]$} 
\FOR{$v_w^t \in \mathbf{v}^t$  \COMMENT{Iterate over vectors and update each vector with neighboring vectors in constraint graph}} 
%
\STATE  
\begin{align} 
\label{eq:key-iteration}
v_w^{t+1} &\gets v_w^{t} - \eta \frac{1}{|\mathcal{P}|}\Biggr[\sum_{\substack{P_z \in \mathcal{P}\\\text{s.t } w \subseteq z}} \sum_{\substack{s \subseteq z\\\text{s.t } w \subseteq s}} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{w' \subseteq s\\ \text{s.t }\zeta(w,w') = s}} v_{w'}^t   \\ 
&+ 2\rho \Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t }w \subseteq z}} \sum_{\substack{w',h,h' \subseteq s\\ \text{s.t } \zeta(w,w') = \zeta(h,h')}} \big(\langle v_w^t,v_{w'}^t\rangle - \langle v_h^t, v_{h'}^t\rangle\big) v_w'^t 
+(\| v_w^t\|^2 - 1)v_w^t\Bigg]\Biggr]  \nonumber
\end{align}
%\COMMENT{Update each vector with neighboring vectors in constraint graph}
\IF {$\| v_w^{t+1} - v_w^t\| \leq \psi$} 
    \STATE $\zeta \gets N(0,\sigma I)$
\ELSE 
    \STATE $\zeta \gets 0$
\ENDIF
\STATE $v_w^{t+1} \gets v_w^{t+1} + \zeta$ %\COMMENT{Add perturbed noise if gradient smaller than threshold}
\ENDFOR
\ENDFOR
\STATE \textbf{return}{ $\mathbf{v}^t$}
\STATE \textbf{Output: vectors corresponding to solution to }\sdpref{alg:sdp-vector} (top of pg.18)
%\COMMENT{Returns the vectors corresponding to solution to \sdpref{alg:sdp-vector}}
%\EndProcedure
\end{algorithmic}
\end{algorithm}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SIMPLIFIED MSG ALGO 1 
% \begin{algorithm} 
% \setcounter{algorithm}{0}
% \caption{Message Passing for Max-CSP (informal-simplified)}
% \label{alg:message-passing} \setcounter{algorithm}{0}
% \begin{algorithmic}[1]
% %\Procedure{Message Passing}{$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}
% \STATE $\mathbf{v}^0 \gets Uniform(\mathcal{S}^{n-1})$ \quad \quad \quad \COMMENT{Initialize vectors to uniform on the unit sphere}
% \FOR{$t=1,2, \dots,  T$}
% \FOR{$v_w^t \in \mathbf{v}^t$ \COMMENT{message passing on the constraint graph}} 
% \STATE 
% \begin{align} 
% \label{eq:key-iteration}
% {v}_w^{t+1} &\gets v_w^{t} - \eta \frac{1}{|\mathcal{P}|}\left[\sum_{v_{w'} \in N(v_w)} \left( \frac{\partial \mathcal{L}_{\text{objective}}(v_{w},v_{w'})}{\partial v_w}
% +  2\rho \frac{\partial \mathcal{L}_{\text{constraint}}(v_{w},v_{w'})}{\partial v_w} \right)\right]
% \end{align}
% %\COMMENT{Update each vector with neighboring vectors in constraint graph}
% \IF {$\| v_w^{t+1} - v_w^t\| \leq \psi $} 
%     \STATE $v_w^{t+1} \gets v_w^{t+1} + \mathcal{N}(0,\sigma I)$ 
% \ENDIF
% \ENDFOR
% \ENDFOR
% \STATE \textbf{return}{ $\mathbf{v}^t$} %\COMMENT{Returns the vectors corresponding to solution to \sdpref{alg:sdp-vector}}
% %\EndProcedure
% \end{algorithmic}
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SIMPLIFIED MSG ALGO 1 


\begin{theorem} \label{thm:main-theorem}
\Algref{alg:message-passing} computes in $poly(\epsilon^{-1},\Phi,\log(\delta^{-1}))$ iterations a set of vectors $\mathbf{v} \defeq\{\hat{v}_s\}$ for all $s \subseteq \mathcal{S}(P)$ for all $P \in \mathcal{P}$ that satisfy the constraints of \sdpref{alg:sdp-vector} to error $\epsilon$ and approximates the optimum of \sdpref{alg:sdp-vector} to error $\epsilon$ with probability $1-\delta$ 
\[\big|\sum_{P_z \in \mathcal{P}} \pE_{\hat{\mu}}[P_z(X_z)] - \text{SDP}(\Lambda)\big| \leq \epsilon\]
where $\text{SDP}(\Lambda)$ is the optimum of \sdpref{alg:sdp-vector}.  
\end{theorem}

\begin{proof}
We begin by writing down the objective penalized by a quadratic on the constraints.    
\begin{multline} \label{eq:obj-penalized}
\mathcal{L}_\rho(\mathbf{v}) \defeq \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \pE_\mu[P_z(X_z)]\\ + \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 +
\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}

For any monomial $X_s = \prod_{i \in s} x_i$ in $P_z(X_z)$ we write     
\begin{align} \label{eq:pseudo-monomial}
\pE_\mu[X_s] \defeq \frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\\text{s.t } \zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle
\end{align}
Where $\mathcal{C}(s)$ is the size of the set $\{g,g' \subseteq s: \zeta(g,g') = s\}$.  In a small abuse of notation, we regard this as the definition of $\pE_\mu[X_s]$ but realize that we're referring to the iterates of the algorithm before they've converged to a pseudoexpectation.  Now recall \eqref{eq:defpz}, we can expand the polynomial $P_z(X_z)$ along its standard monomial basis 
 
\begin{align} \label{eq:coef-basis}
P_z(X_z) = \sum_{s \subseteq z} y_s X_s 
\end{align}

where we have defined coefficients $y_s$ for every monomial in $P_z(X_z)$.  Plugging \eqref{eq:pseudo-monomial} and \eqref{eq:coef-basis} into \eqref{eq:obj-penalized} we obtain  
\begin{multline}
\mathcal{L}_\rho(\mathbf{v}) = \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\ \text{s.t }\zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle\\ 
+ \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 \\
+\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}
Taking the derivative with respect to any $v_w \in \mathbf{v}$ we obtain 

\begin{multline} \label{eq:sdp-penalized-grad}
\frac{\partial \mathcal{L}_\rho(\mathbf{v})}{\partial v_w}  = \frac{1}{|\mathcal{P}|}\Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t } w \subseteq z}} \sum_{\substack{s \subseteq z\\\text{s.t } w \subseteq s}} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{w' \subseteq s\\ \text{s.t } \zeta(w,w') = s}} v_{w'}\\ 
+ 2\rho \Bigg[\sum_{\substack{P_z \in \mathcal{P}\\ \text{s.t } w \subseteq z}} \sum_{\substack{w',h,h' \subseteq s\\ \text{s.t } \zeta(w,w') = \zeta(h,h')}} \big(\langle v_w,v_{w'}\rangle - \langle v_h, v_{h'}\rangle\big) v_w' \\
+(\| v_w\|^2 - 1)v_w\Bigg]\Bigg]
\end{multline} 
The gradient update is then what is detailed in \Algref{alg:message-passing}
\begin{align}
    v^{t+1}_w = v^t_w - \eta \frac{\partial \mathcal{L}_\rho(\mathbf{v})}{\partial v_w}
\end{align}
Thus far we have established the form of the gradient.  To prove the gradient iteration converges we reference the literature on convergence of perturbed gradient descent \citep{jin2017escape} which we rewrite in \thmref{thm:perturbed-gd}.  First we note that the \sdpref{alg:sdp-vector} has $\ell$ smooth gradient for $\ell \leq poly(\rho,B)$ and has $\gamma$ lipschitz Hessian for $\gamma = poly(\rho,B)$ which we arrive at in \lemref{lem:csp-lipschitz} and \lemref{lem:csp-hessian}.  The proofs of \lemref{lem:csp-lipschitz} and \lemref{lem:csp-hessian} are technically involved and form the core hurdle in arriving at our proof.  

Then by \thmref{thm:perturbed-gd} the iteration converges to an $(\epsilon',\gamma^2)$-SOSP \defref{def:sosp} in no more than $\Tilde{O}(\frac{1}{\epsilon'^2})$ iterations with probability $1-\delta$. 
Now that we've established that the basic gradient iteration converges to approximate SOSP, we need to then prove that the approximate SOSP are approximate global optimum. We achieve this by using the result of \cite{bhojanapalli2018smoothed} lemma 3 which we restate in \lemref{lem:smoothed} for convenience.      

The subsequent presentation adapts the proof of \lemref{lem:smoothed} to our setting.   
To show that $(\epsilon',\gamma^2)$-SOSP are approximately global optimum, we have to work with the original SDP loss as opposed to the nonconvex vector loss.  For subsequent analysis we need to define the penalized loss which we denote $\mathcal{H}_\rho(\pE[\mathbf{x}])$ in terms of the SDP moment matrix $\pE[\mathbf{x}]$.  
\begin{multline} \label{eq:obj-sdp-penalized}
\mathcal{H}_\rho(\pE[\mathbf{x}]) \defeq \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \pE_{\hat{\mu}}[P_z(X_z)]\\ + \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \text{s.t } \zeta(g,g') = \zeta(h,h')}} \big(\pE_{\hat{\mu}}[X_{\zeta(g,g')}] - \pE_{\hat{\mu}}[X_{\zeta(h,h')}]\big)^2 +
\sum_{\substack{X_s \text{ s.t } s \subset \mathcal{S}(P)\\ |s| \leq k, \forall P \in \mathcal{P}}} (\pE_{\hat{\mu}}[X_s^2] - 1)^2\Bigg]\Bigg]
\end{multline}
Here we use the notation $\pE_{\hat{\mu}}[X_{\zeta(g,g')}]$ and $\pE_{\hat{\mu}}[X_{\zeta(h,h')}]$ to denote $\langle v_g,v_g'\rangle$ and $\langle v_h,v_h'\rangle$ respectively.    
Note that although by definition $\mathcal{H}_\rho(\pE[\mathbf{x}]) = \mathcal{L}_\rho(\mathbf{v})$ , their gradients and hessians are distinct because $\mathcal{L}_\rho(\mathbf{v})$ is overparameterized.  This is the key point.  It is straightforward to argue that SOSP of a convex optimization are approximately global, but we are trying to make this argument for SOSP of the overparameterized loss $\mathcal{L}_\rho(\mathbf{v})$.     

Let the global optimum of \sdpref{alg:sdp-vector} be denoted $\pE_{\Tilde{\mu}}[\Tilde{\mathbf{x}}]$ with a cholesky decomposition $\Tilde{\mathbf{v}}$.  Let $\hat{\mathbf{v}}$ be the set of vectors outputted by \Algref{alg:message-passing} with associated pseudoexpectation $\pE_{\hat{\mu}}[\hat{\mathbf{x}}]$.  Then, we can bound
\begin{align} \label{eq:convex-bound}
\mathcal{L}_\rho(\hat{\mathbf{v}}) - \mathcal{L}_\rho(\Tilde{\mathbf{v}}) = \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]) - \mathcal{H
}_\rho(\pE[\Tilde{\mathbf{x}}])  \leq
\big\langle \nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]), \pE[\hat{\mathbf{x}}] - \pE[\Tilde{\mathbf{x}}]\big\rangle
\end{align}
Here the first equality is by definition, and the inequality is by the convexity of $\mathcal{H}_\rho$.  Moving on, we use the fact that the min eigenvalue of the hessian of overparameterized loss $\nabla^2 \mathcal{L}_\rho(\hat{\mathbf{v}}) \succeq -\gamma\sqrt{\epsilon'}$ implies the min eigenvalue of the gradient of the convex loss $\lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \geq -\gamma\sqrt{\epsilon'}$.  This fact is invoked in \cite{bhojanapalli2018smoothed} lemma 3 which we adapt to our setting in \lemref{lem:smoothed}.  Subsequently, we adapt the lines of their argument in \lemref{lem:smoothed} most relevant to our analysis which we detail here for the sake of completeness.
\begin{multline}
\text{\ref{eq:convex-bound}} \leq  - \lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \Tr(\pE[\hat{\mathbf{x}}]) - \big\langle \nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]), \pE[\Tilde{\mathbf{x}}] \big\rangle\\
 \leq - \lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \Tr(\pE[\hat{\mathbf{x}}]) + \| \nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])\|_F \|\pE[\Tilde{\mathbf{x}}]\|_F\\
\leq \gamma \sqrt{\epsilon'} \Tr(\pE[\mathbf{x}]) +  \epsilon' \|\Tilde{\mathbf{v}}\|_F \leq \gamma \sqrt{\epsilon'}\Phi + \epsilon' \Phi \leq \epsilon\\
\end{multline}
Here the first inequality follows by a standard inequality of frobenius inner product, the second inequality follows by Cauchy-Schwarz, the third inequality follows by the $(\epsilon',\gamma^2)$-SOSP conditions on both the min eigenvalue of the hessian and the norm of the gradient, the final two inequalities follow from knowing the main diagonal of $\pE[\hat{\mathbf{x}}]$ is the identity and that every vector in $\tilde{\mathbf{v}}$ is a unit vector up to inverse polynomial error $poly(\rho^{-1},2^k)$.  For this last point see the proof in \lemref{lem:precision}.  Therefore if we set $\epsilon' = poly(\epsilon,2^{-k})$ we arrive at any $\epsilon$ error.  
Therefore we have established our estimate $\hat{v}$ is approximates the global optimum of the quadratically penalized objective i.e 
$\mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}]) - \mathcal{H
}_\rho(\pE[\Tilde{\mathbf{x}}]) \leq \epsilon$.  
To finish our proof, we have to bound the distance between the global optimum of the quadratically penalized objective $\mathcal{H}_\rho(\pE[\Tilde{\mathbf{x}}])$ and SDP$(\Lambda)$ the optimum of \sdpref{alg:sdp-vector}.  This is established for $\rho$ a sufficiently large $poly(\epsilon^{-1},2^k)$ in \lemref{lem:precision}. This concludes our proof that the iterates of \Algref{alg:message-passing} converge to the solution of \sdpref{alg:sdp-vector}.    
\end{proof}

In our proof above, the bound on approximate SOSP being approximate global optimum is built on the result of \cite{bhojanapalli2018smoothed} which we rephrase for our setting below.  
\begin{lemma}\label{lem:smoothed} [\cite{bhojanapalli2018smoothed} lemma 3 rephrased]
Let $\mathcal{L}_\rho(\cdot)$ be defined as in \eqref{eq:obj-penalized} and let $\mathcal{H}_\rho(\cdot)$ be defined as in \eqref{eq:obj-sdp-penalized}.  Let $U \in \R^{\Phi \times \Phi}$ be an $(\epsilon,\gamma)$-SOSP of $\mathcal{L}_\rho(\cdot)$, then 
\[\lambda_{\text{min}}(\nabla \mathcal{H
}_\rho(\pE[\hat{\mathbf{x}}])) \geq - \gamma\sqrt{\epsilon}\]
Furthermore, the  global optimum $\mathbf{\Tilde{X}}$ obeys the optimality gap 

\[\mathcal{H}_\rho(UU^T) - \mathcal{H}_\rho(\mathbf{\Tilde{X}}) \leq \gamma\sqrt{\epsilon} \Tr(\mathbf{\Tilde{X}}) + \frac{1}{2}\epsilon \|U\|_F\]

\end{lemma}


The following \lemref{lem:precision} establishes that for a sufficiently large penalty parameter $\rho = poly(\epsilon^{-1},2^k)$ the optimum of the penalized problem and the exact solution to \sdpref{alg:sdp-vector} are close.  

\begin{lemma} \label{lem:precision}
Let $\Lambda$ be a Max-k-CSP instance, and let SDP$(\Lambda)$ be the optimum of \sdpref{alg:sdp-vector}.  Let $\mathcal{L}_\rho(\mathbf{v})$ be the quadratically penalized objective 
\begin{multline} \label{eq:loss-normalize}
\mathcal{L}_\rho(\mathbf{v}) \defeq \frac{1}{|\mathcal{P}|}\Bigg[\sum_{P_z \in \mathcal{P}} \sum_{s \subseteq z} y_s\frac{1}{|\mathcal{C}(s)|}\sum_{\substack{g,g' \subseteq s\\ \text{s.t } \zeta(g,g') = s}} \langle v_{g}, v_{g'}\rangle 
+ \rho \Bigg[\sum_{P_z \in \mathcal{P}} \sum_{\substack{g,g',h,h' \subseteq z\\ \zeta(g,g') = \zeta(h,h')}} \big(\langle v_g,v_{g'}\rangle - \langle v_h, v_{h'}\rangle\big)^2 \\
+\sum_{v_s \in \mathbf{v}} (\| v_s\|^2 - 1)^2\Bigg]\Bigg]
\end{multline}
Let $\Tilde{v}$ be the argmin of the unconstrained minimization 
\[\Tilde{v} \defeq \argmin_{\mathbf{v} \in \R^{|\mathcal{P}|^2 (2^{2k})}} \mathcal{L}_\rho(\mathbf{v}) \]
Then we have   
\[\mathcal{L}_\rho(\Tilde{\mathbf{v}}) - \text{SDP}(\Lambda) \leq \epsilon\]
for $\rho = poly(\epsilon^{-1},2^k)$ 
\end{lemma}

\begin{proof}
We begin the analysis with the generic equality constrained semidefinite program of the form 
\begin{align} 
\label{eq:sdp-generic} 
\text{Minimize:} \quad & \langle C, X\rangle \\
\text{Subject to:} \quad & \langle A_{i}, X\rangle = b_i \quad \forall i \in \mathcal{F} \\
& X \succeq 0 \\
& X \in \mathbb{R}^{d \times d}
\end{align}

For an objective matrix $C$ and constraint matrices $\{A_i\}_{i \in \mathcal{F}}$ in some constraint set $\mathcal{F}$.  We will invoke specific properties of \sdpref{alg:sdp-vector} to enable our analysis.  First we define the penalized objective in this generic form
\[\mathcal{H}_\rho(X) \defeq \langle C,X\rangle + \rho\sum_{i \in \mathcal{F}}(\langle A_i,X\rangle - b_i)^2 \]
Let $\Tilde{X}$ be the minimizer of the penalized problem.  
\[\Tilde{X} \defeq \argmin_{X \in \R^{d \times d}}\mathcal{L}_\rho(X)\]
Let  $X^*$ be the minimizer of the constrained problem \eqref{eq:sdp-generic}.  
Let $\tau_i$ be the error $\Tilde{X}$ has in satisfying constraint $\langle A_i, \Tilde{X}\rangle = b_i$. 
\[\tau_i \defeq |\langle A_i,\Tilde{X}\rangle - b_i|\]
We will show that $\tau_i$ scales inversely with $\rho$.  That is, $\tau_i \leq poly(k,\rho^{-1})$.  Notice that the quadratic penalty on the violated constraints must be smaller than the decrease in the objective for having violated the constraints.  So long as the objective is not too sensitive i.e 'robust' to perturbations in the constraint violations the quadratic penalty should overwhelm the decrease in the objective.  To carry out this intuition, we begin with the fact that the constrained minimum is larger than the penalized minimum.  
\begin{align}
\mathcal{H}_\rho(X^*) - \mathcal{H}_\rho(\Tilde{X}) \leq 0
\end{align}
Applying the definitions of $\mathcal{H}_\rho(X^*)$ and $\mathcal{H}_\rho(\Tilde{X})$ we obtain
\begin{align}
\langle C,X^* \rangle - (\langle C,\Tilde{X} \rangle + \rho\sum_{i \in \mathcal{F}} \tau_i^2) \leq 0
\end{align}
Rearranging LHS and RHS and dividing by $|\mathcal{F}|$ we obtain 
\begin{align} \label{eq:51}
\rho \frac{1}{|\mathcal{F}|}\sum_{i \in \mathcal{F}} \tau_i^2 \leq \frac{1}{|\mathcal{F}|} \langle C,\Tilde{X} - X^*\rangle
\end{align}
We upper bound the RHS using the robustness theorem of \cite{RSanycsp09} restated in the appendix \thmref{thm:robustness} which states that an SDP solution that violates the constraints by a small perturbation changes the objective by a small amount.  Thus we obtain,  
\begin{align} \label{eq:52}
RHS \leq \Big(\frac{1}{|\mathcal{F}|}\sum_{i \in \mathcal{F}} \tau_i \Big)^{1/2} poly(k)
\end{align}
Therefore combining \eqref{eq:51} with \eqref{eq:52} we obtain 
\[\rho \frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \leq \Big(\frac{1}{|\mathcal{F}|}\sum_i \tau_i \Big)^{1/2} poly(k)\]
Taking Cauchy-Schwarz on the RHS we obtain 
\[\rho \frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \leq \Big(\frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \Big)^{1/4}poly(k)\]
Noticing that $\frac{1}{|\mathcal{F}|}\sum_i \tau_i^2$ appears in both LHS and RHS we rearrange to obtain 
\[\frac{1}{|\mathcal{F}|}\sum_i \tau_i^2 \leq  \frac{poly(k)}{\rho^{4/3}} \leq \epsilon\]

Where for $\rho = \frac{poly(k)}{\epsilon^{3/4}}$ we have the average squared error of the constraints is upper bounded by $\epsilon$.  Then via Markov's no more than $\sqrt{\epsilon}$ fraction of the constraints can be violated by more than squared error $\sqrt{\epsilon}$.  We label these 'grossly' violated constraints. The clauses involved in these grossly violated constraints contributes no more than $poly(k)\sqrt{\epsilon} $ to the objective.  On the other hand, the  constraints that are violated by no more than squared error $\sqrt{\epsilon}$ contributed no more than $poly(k)\epsilon^{1/8} $ to the objective which follows from the robustness theorem \thmref{thm:robustness}.  Taken together we conclude that   
\[\mathcal{L}_\rho(\Tilde{\mathbf{v}}) - \text{SDP}(\Lambda) \leq \epsilon\]
For $\rho = poly(k,\epsilon^{-1})$ as desired.  
\end{proof}

Finally we show it's not hard to generalize our algorithm to alphabets of size $[q]$.  

\paragraph{Notation for General Alphabet.}
For any predicate $P \in \mathcal{P}$, let $\mathcal{D}(P)$ be the set of all variable assignment tuples indexed by a set of variables $s \subseteq \mathcal{S}(P)$ and an assignment $\tau \in [q]^{|s|}$.  Let $x_{(i,a)}$ denote an assignment of value $a \in [q]$ to variable $x_i$.   

\begin{SDPOPT}
\setcounter{algorithm}{1}
\caption{SDP Vector Formulation for Max-k-CSP General Alphabet (Equivalent to UGC optimal)}
\label{alg:sdp-vector-q}
\begin{algorithmic}
\STATE {SDP Vector Formulation General Alphabet $\Lambda = (\mathcal{V},\mathcal{P},q)$.\\  {Pseudoexpectation formulation of the objective.}} 
\begin{align} \label{eq:sdp-vector-q}
\min_{x_1,x_2,\dots,x_N}  & \sum_{P_z \subset \mathcal{P}} \pE_{\mu}[-P_z(X_z)]  \\ \nonumber
 \\ \text{subject to:} \quad & \pE_\mu[(x_{(i,a)}^2 - x_{(i,a)})\prod_{(j,b) \in \phi} x_{(j,b)}] = 0 \quad \forall i \in \mathcal{V}\text{, } \forall a \in [q]\text{, }\forall \phi \subseteq \mathcal{D}(P) \text{, } \forall P \in \mathcal{P}\\
\quad & \pE_\mu[(\sum_{a \in [q]} x_{ia} - 1)\prod_{(j,b) \in \phi} x_{(j,b)}] = 0\quad \forall i \in \mathcal{V}\text{, } \forall \phi \subseteq \mathcal{D}(P) \text{, }\forall P \in \mathcal{P}, \\
\quad & \pE_\mu[x_{(i,a)}x_{(i,a')} \prod_{(j,b) \in \phi} x_{(j,b)}] = 0 \quad \forall i \in \mathcal{V} \text{, } \forall a \neq a' \in [q]\text{, } \forall \phi \subseteq \mathcal{D}(P) \text{, }\forall P \in \mathcal{P}, \\
\quad & \pE[SoS_{2kq}(X_\phi)] \geq 0 \quad \forall \phi \subseteq \mathcal{D}(P) \text{, }\forall P \in \mathcal{P}, \\ 
\quad & \pE[SoS_2(\mathbf{x})] \geq 0.
  \end{align}
\STATE {First constraint corresponds to booleanity of each value in the alphabet. \\
Second constraint corresponds to a variable taking on only one value in the alphabet.\\
Third constraint corresponds to a variable taking on only one value in the alphabet.\\
Fourth constraint corresponds to local distribution on the variables in each predicate.
\\
Fifth constraint corresponds to the positivity of every degree two sum of squares of polynomials.}


\end{algorithmic}
\end{SDPOPT} 



\begin{lemma} \label{lem:alphabet}
There exists a message passing algorithm that computes in $poly(\epsilon^{-1},\Phi,\log(\delta^{-1}))$ iterations a set of vectors $\mathbf{v} \defeq\{\hat{v}_{(i,a)}\}$ for all $(i,a) \in \phi$, for all $\phi \subseteq \mathcal{D}(P)$, for all $P \in \mathcal{P}$ that satisfy the constraints of \Algref{alg:sdp-vector-q} to error $\epsilon$ and approximates the optimum of \Algref{alg:sdp-vector-q} to error $\epsilon$ with probability $1-\delta$ 
\[\big|\sum_{P_z \in \mathcal{P}} \pE_{\hat{\mu}}[P_z(X_z)] - \text{SDP}(\Lambda)\big| \leq \epsilon\]
where $\text{SDP}(\Lambda)$ is the optimum of \Algref{alg:sdp-vector-q}. 

\end{lemma}

\begin{proof}
The proof is entirely parallel to the proof of \thmref{thm:main-theorem}.  We can write \Algref{alg:sdp-vector-q} entirely in terms of the vector of its cholesky decomposition where once again we take advantage of the fact that SoS degree $2kq$ distributions are actual distributions over subsets of $kq$ variables over each predicate.  Given the overparameterized vector formulation, we observe that once again we are faced with equality constraints that can be added to the objective with a quadratic penalty.  Perturbed gradient descent induces a message passing algorithm over the constraint graph $G_\Lambda$, and in no more than $poly(\epsilon^{-1}\Phi)$ iterations reaches an $(\epsilon,\gamma)$-SOSP.  The analysis of optimality goes along the same lines as \lemref{lem:precision}.  For sufficiently large penalty $\rho = poly(\epsilon^{-1},q^k)$ the error in satisfying the constraints is $\epsilon$ and the objective is robust to small perturbations in satisfying the constraint.  That concludes our discussion of generalizing to general alphabets.       
\end{proof}
\subsection{Definitions}

\begin{definition}[Message passing algorithm] \label{def:message-passing}
 Given a graph $G = (V,E)$ with a set of vectors $\mathbf{v} = \{v_i\}_{i \in V}$ a message passing algorithm for $T$ iterations is an update of the form; for vector $v_i$ in $\mathbf{v}$ and for iteration $t \in [T]$, 
\[v_i^{t+1} = \text{UPDATE}(\{v_j^t\}_{j \in N(i)},v_i^t)\]
For an arbitrary polynomial time computable function $\text{UPDATE}: \R^{r|N(i)|} \times \R^r \rightarrow \R^r$
\end{definition}

\subsection{Neural Certification Scheme}
\label{sec:certificate}
An intriguing aspect of OptGNN is that the embeddings can be interpreted as the solution to a low rank SDP which leaves open the possibility that the embeddings can be used to generate a dual certificate i.e a lower bound on a convex relaxation.  First, we define the primal problem 
\begin{align} 
\label{eq:sdp-generic}
\text{Minimize:} \quad &  \langle C, X\rangle \\
\text{Subject to:} \quad & \langle A_i, X\rangle = b_i \quad \forall i \in [\mathcal{F}] \\
& X \succeq 0
\end{align}

\begin{lemma}
\label{lem:certificate}
Let OPT be the minimizer of the SDP \eqref{eq:sdp-generic}.  Then for any $\Tilde{X} \in \R^{N \times N} \succeq 0$ and any $\lambda^* \in \R^{|\mathcal{F}|}$, we define $F_{\lambda^*}(X)$ to be
\[F_{\lambda^*}(\Tilde{X}) \defeq  \langle C,\Tilde{X}\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i \left(\langle A_i,\Tilde{X}\rangle - b_i \right) \]
We require SDP to satisfy a bound on its trace $Tr(X) \leq \mathcal{Y}$ for some $\mathcal{Y} \in \R^+$. Then the following is a lower bound on OPT.  
\[
OPT \geq F_{\lambda^*}(\Tilde{X}) - \langle \nabla F_{\lambda^*}(\Tilde{X}), \Tilde{X} \rangle + \lambda_{\min}\left(\nabla F_{\lambda^*}(\Tilde{X}) \right)\mathcal{Y}
\]

\end{lemma}

\begin{proof}
Next we introduce lagrange multipliers $\lambda \in \mathbb{R}^k$ and $Q \succeq 0$ to form the lagrangian 
\begin{align*}
\mathcal{L}(\lambda,Q,X) = \langle C,X\rangle + \sum_{i \in \mathcal{F}} \lambda_i \left(\langle A_i,X\rangle - b_i \right) - \langle Q,X\rangle
\end{align*}

We lower bound the optimum of OPT defined to be the minimizer of \eqref{eq:sdp-generic}
\begin{align}
OPT \defeq \min_{X \succeq 0}\max_{\lambda \in \R,Q \succeq 0}\mathcal{L}(\lambda,Q,X) 
\geq & \min_{V \in \mathbb{R}^{N \times N}}\max_{\lambda}\langle C,VV^T\rangle + \sum_{i \in \mathcal{F}} \lambda_i \left(\langle A_i,VV^T\rangle - b_i\right)\\
=& \max_{\lambda}\min_{V \in \mathbb{R}^{N \times N}}\langle C,VV^T\rangle + \sum_{i \in \mathcal{F}} \lambda_i \left(\langle A_i,VV^T\rangle - b_i\right) \\
 \label{eq:sdp-overparam}  
=& \min_{V \in \mathbb{R}^{N \times N}}\langle C,VV^T\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i \left(\langle A_i,VV^T\rangle - b_i\right).
\end{align}
Where in the first inequality we replaced $X \succeq 0$ with $VV^T$ which is a lower bound as every psd matrix admits a cholesky decomposition.  In the second inequality we flipped the order of min and max, and in the final inequality we chose a specific set of dual variables $\lambda^* \in \R^{|\mathcal{F}|}$ which lower bounds the maximization over dual variables.  The key is to find a good setting for $\lambda^*$. 

Next we establish that for any choice of $\lambda^*$ we can compute a lower bound on inequality \ref{eq:sdp-overparam} as follows. 
Let $F_{\lambda^*}(VV^T)$ be defined as the funciton in the RHS of \ref{eq:sdp-overparam}. 
\begin{align*}
F_{\lambda^*}(VV^T) \defeq  \langle C,X\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i \left(\langle A_i,X\rangle - b_i\right) 
\end{align*}
Then \eqref{eq:sdp-overparam} can be rewritten as 
\begin{align*}
OPT \geq \min_{V \in \mathbb{R}^{N \times N}}F_{\lambda^*}(VV^T) \defeq  \langle C,X\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i \left(\langle A_i,X\rangle - b_i\right) 
\end{align*}
Now let $V^*$ be the minimizer of \eqref{eq:sdp-overparam}  and let $X^* = V^* (V^*)^T$.  We have by convexity that 
\begin{align}
F_{\lambda^*}(X) -  F_{\lambda^*}(X^*) \leq \langle \nabla F_{\lambda^*}(X), X - X^* \rangle = \langle \nabla F_{\lambda^*}(X), X\rangle + \langle - \nabla F_{\lambda^*}(X) ,X^* \rangle \\
\leq \langle \nabla F_{\lambda^*}(X), X\rangle - \lambda_{min}\left(\nabla F_{\lambda^*}(X) \right)\mathrm{Tr}(X^*)\\
\leq \langle \nabla F_{\lambda^*}(X), X\rangle - \lambda_{min}(\nabla F_{\lambda^*}(X) )N
\end{align}
In the first inequality we apply the convexity of $F_{\lambda^*}$.  In the second inequality we apply a standard inequality of frobenius inner product.  In the last inequality we use the fact that $\mathrm{Tr}(X^*) = N$.  
Rearranging we obtain for any $X$
\begin{align}
OPT \geq F_\lambda(X^*)
\geq F_{\lambda^*}(X)  - \langle \nabla F_{\lambda^*}(X), X\rangle + \lambda_{min}\left(\nabla F_{\lambda^*}(X) \right)N
\end{align}
Therefore it suffices to upper bound the two terms above $\langle \nabla F_{\lambda^*}(X), X\rangle$ and $\lambda_{min}(\nabla F_{\lambda^*}(X))$ which is an expression that holds for any $X$.  Given the output embeddings $\Tilde{V}$ of OptGNN (or indeed any set of vectors $\Tilde{V}$) let $\Tilde{X} = \Tilde{V}\Tilde{V}^T$. Then we have concluded   
\begin{align}
OPT \geq F_\lambda(X^*) \geq F_{\lambda^*}(\Tilde{X}) - \langle \nabla F_{\lambda^*}(\Tilde{X}), \Tilde{X} \rangle + \lambda_{\min}(\nabla F_{\lambda^*}(\Tilde{X})) N
\end{align}

as desired.  
\end{proof}
Up to this point, every manipulation is formal proof.  Subsequently we detail how to estimate the dual variables $\lambda^*$.  Although any estimate will produce a bound, it won't produce a tight bound.  To be clear, solving for the optimal $\lambda^*$ would be the same as building an SDP solver which would bring us back into the expensive primal dual procedures that are involved in solving SDP's.  We are designing quick and cheap ways to output a dual certificate that may be somewhat looser.  Our scheme is simply to set $\lambda^*$ such that $\|\nabla F_{\lambda^*}(\Tilde{X})\|$ is minimized, ideally equal to zero.  The intuition is that if $(\Tilde{X}, \lambda^*)$ were a primal dual pair, then the lagrangian would have a derivative with respect to $X$ evaluated at $\Tilde{X}$ would be equal to zero.   
Let $H_\lambda(V)$ be defined as follows 
\begin{align*}
H_{\lambda^*}(\Tilde{V}) \defeq  \langle C,\Tilde{V}\Tilde{V}^T\rangle + \sum_{i \in \mathcal{F}} \lambda^*_i \left(\langle A_i,\Tilde{V}\Tilde{V}^T\rangle - b_i\right) 
\end{align*}
We know the gradient of $H_{\lambda}(\Tilde{V})$
\begin{align*}
\nabla H_\lambda(\Tilde{V}) = 2\left(C + \sum_{i \in \mathcal{F}} \lambda^*_i A_i\right)\Tilde{V} = 2 \nabla F_\lambda(\Tilde{V}\Tilde{V}^T) \Tilde{V}
\end{align*}

Therefore it suffices to find a setting of $\lambda^*$ such that  $\|\nabla F_\lambda(\Tilde{X}) \Tilde{V}\|$ is small, ideally zero.  This would be a simple task, indeed a regression, if not for the unfortunate fact that OptGNN explicitly projects the vectors in $\Tilde{V}$ to be unit vectors.  This creates numerical problems such that minimizing the norm of $\|\nabla F_\lambda(\Tilde{X}) \Tilde{V}\|$ does not produce a $\nabla F_\lambda(\Tilde{X})$ with a large minimum eigenvalue.  

To fix this issue, let $R_{\eta,\rho} (V)$ denote the penalized lagrangian with quadratic penalties for constraints of the form $\langle A_i,X \rangle = b_i$ and linear penalty $\eta_i$ for constraints along the main diagonal of $X$ of the form $\langle e_ie_i^T, X\rangle = 1$.
\begin{align*}
    R_{\eta,\rho} (V) \defeq  \langle C, VV^T\rangle + \sum_{i \in \mathcal{J}} \rho (\langle A_i, VV^T\rangle - b_i)^2 + \sum_{i=1}^N \eta_i(\langle e_ie_i^T, VV^T\rangle - 1)
\end{align*}

Taking the gradient of $R_{\eta,\rho} (V)$ we obtain 
\begin{align*}
    \nabla R_{\eta,\rho} (V) \defeq  2CV + \sum_{i \in \mathcal{J}} 2\rho (\langle A_i, VV^T\rangle - b_i)A_i V + \sum_{i=1}^N 2\eta_i e_ie_i^TV
\end{align*}


Our rule for setting dual variables $\delta_i$ for $i \in \mathcal{J}$ is 
\[
\delta_i \defeq  2\rho \left( \langle A_i, \Tilde{V}\Tilde{V}^T \rangle - b_i \right)
\]


our rule for setting dual variables $\eta_j$ for $j \in [N]$ is 
\[
\eta_j \defeq \frac{1}{2} \left\| e_j^T \left( C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i, VV^T\rangle - b_i)A_i \right) V \right\|
\]


Then our full set of dual variables $\lambda^*$ is simply the concatenation $(\delta,\eta)$. Writing out everything explicitly we obtain the following matrix for $\nabla F_{\lambda^*}(\Tilde{V}\Tilde{V}^T)$

\begin{align*}
\nabla F_\lambda(\Tilde{V}\Tilde{V}^T) = C + \sum_{i \in \mathcal{F}} \rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2} \left\| e_j^T\left( C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i)A_i \right) \Tilde{V} \right\| e_ie_i^T
\end{align*}

Plugging this expression into \lemref{lem:certificate} the final bound we evaluate in our code is 
\begin{multline}
OPT \geq \langle C, \Tilde{V}\Tilde{V}^T\rangle + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i)^2 \\
- \left\langle  C + \sum_{i \in \mathcal{F}}  \rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2}\left\|e_j^T\left(C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i)A_i\right) \Tilde{V} \right\| e_ie_i^T, \Tilde{V}\Tilde{V}^T\right\rangle \\
+ \lambda_{\min}\left( C + \sum_{i \in \mathcal{F}}  \rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i) A_i + \sum_{j \in [N]} \frac{1}{2}\left\|e_j^T\left(C + \sum_{i \in \mathcal{F}} 2\rho (\langle A_i, \Tilde{V}\Tilde{V}^T\rangle - b_i)A_i\right) \Tilde{V} \right\| e_ie_i^T  \right)N
\end{multline}


Which is entirely computed in terms of $\Tilde{V}$ the output embeddings of OptGNN.  The resulting plot is as follows.     

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\linewidth]{cert50.png}
    \caption{N=50 p=0.1 SDP vs OptGNN Dual Certificate}
    \label{fig:cert50}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\linewidth]{cert100.png}
%     \caption{N=100 p=0.1 SDP vs OptGNN Dual Certificate}
%     \label{fig:cert100}
% \end{figure}
\textbf{Note:} The reason for splitting the set of dual variables is because the projection operator onto the unit ball is hard coded into the architecture of the lift network. Satisfying the constraint set via projection is different from the soft quadratic penalties on the remaining constraints and require separate handling.
\paragraph{Max-Cut Certificate}
For Max-Cut our dual variables are particularly simple as there are no constraints $\langle A_i,X\rangle = b_i$ for $b_i \neq 0$.  The dual variables for Max-Cut take on the form for all $i \in [N]$
\begin{align*}
    \lambda^*_i = \frac{1}{2}\left\| \sum_{j \in N(i)} w_{ij}v_j\right\|    
\end{align*}

It's certainly possible to come up with tighter certification schemes which we leave to future work.    

\textbf{Intuition: } Near global optimality one step of the augmented method of lagrange multipliers ought to closely approximate the dual variables.  After obtaining a estimate for the penalized lagrange multipliers we estimate the lagrange multipliers for the norm constraint by approximating $\nabla R_{\lambda}(V) = 0$.  The alternative would have been to solve the linear system for all the lagrange multipliers at once but this runs into numerical issues and degeneracies.   

\textbf{Certificate Experiment: } We run our certification procedure which we name OptGNN-cert and compare it to the SDP certificate.  Note, that mathematically we will always produce a larger (i.e inferior) dual certificate in comparison to the SDP because we are bounding the distance to the SDP optimum with error in the gradients and hessians of the output embeddings of OptGNN.  Our advantage is in the speed of the procedure.  Without having to go through a primal dual solver, the entire time of producing OptGNN-cert is in the time required to feedforward through OptGNN. 
In this case we train an OptGNN-Max-Cut with $10$ layers, on $1000$ Erdos-Renyi graphs, with $N=100$ nodes and edge density $p=0.1$.  We plot the OptGNN Max-Cut value (an actual integer cut) on the x-axis and in the y-axis we plot the dual certificate value on the same graph where we compare the SDP certificate with the OptGNN-cert. See \ref{fig:cert50} for the $N=50$ graphs and \ref{fig:cert100} for the $N=100$ graphs.   

Note of course the dual certificate for any technique must be larger than the cut value outputted by OptGNN so the scatter plot must be above the $x=y$ axis of the plot.  We see as is mathematically necessary, the OptGNN-cert is not as tight as the SDP certificate but certainly competitive and more importantly it is arrived at dramatically faster. Without any attempt at optimizing the runtime, the OptGNN feedforward and certification takes no more than $0.02$ seconds whereas the SDP takes $0.5$ seconds on $N=100$ node graphs.       

\section{Experiment details} \label{app:experimental_setup}
In this section we give further details on our experimental setup.


\textbf{Datasets.}
Our experiments span a variety of randomly generated and real-world datasets. Our randomly generated datasets contain graphs from several random graph models, in particular Erd\H{o}s-R\'enyi (with $p=0.15$), Barab\'asi–Albert (with $m=4$), Holme-Kim (with $m=4$ and $p=0.25$), Watts-Strogatz (with $k=4$ and $p=0.25$), and forced RB (with two sets of parameters, RB200 and RB500). Our real-world datasets are ENZYMES, PROTEINS, MUTAG, IMDB-BINARY, COLLAB (which we will together call \textbf{TU-small}), and REDDIT-BINARY, REDDIT-MULTI-5K, and REDDIT-MULTI-12K (which we will call \textbf{TU-REDDIT}).

We abbreviate the generated datasets using their initials and the range of vertex counts. For example, by ER (50,100) we denote Erd\H{o}s-R\'enyi random graphs with a vertex count drawn uniformly at random from [50, 100]. In tables, we mark generated datasets with superscript \textsuperscript{a}, \textbf{TU-small} with \textsuperscript{b}, and \textbf{TU-REDDIT} with \textsuperscript{c}.

For \autoref{tab:forced_rb}, we display results for forced RB instances drawn from two different distributions. For RB200, we select $N$ uniformly in $[6, 15]$ and $K$ uniformly in $[12, 21]$. For RB500, we select $N$ uniformly in $[20, 34]$ and $K$ uniformly in $[10, 29]$.

In \autoref{tab:sat_baselines}, random 3-SAT instances are generated by drawing three random variables for each clause and negating each variable with $p = 0.5$. We trained on instances with 100 variables and clause count drawn uniformly from the interval $[400, 430]$, and tested on instances with 100 variables and 400, 415, and 430 clauses respectively.

\textbf{Baselines.}
We compare the performance of our approach against known classical algorithms. In terms of classical baselines, we run Gurobi with varying timeouts and include SDP results on smaller datasets.
% % SDP scales extremely poorly with graph size so we omit the results for datasets with larger graphs. 
% For Min-Vertex-Cover, we include the classical baseline KaMIS, a maximum independent set solver. 

We also include a greedy baseline, which is the function \texttt{one\_exchange} (for Max-Cut) or \texttt{min\_weighted\_vertex\_cover} (for Min-Vertex-Cover) from \texttt{networkx}~\citep{networkx}.

% Our neural baselines include LwD~\citep{ahn2020learning} and \textsc{Dgl-TreeSearch}~\citep{li2018combinatorial,bother2022s}.

\textbf{Validation and test splits.}
For each dataset we hold out a validation and test slice for evaluation.
In our generated graph experiments we set aside 1000 graphs each for validation and testing. Each step of training ran on randomly generated graphs. For \textbf{TU-small}, we used a train/validation/test split of 0.8/0.1/0.1. For \textbf{TU-REDDIT}, we set aside 100 graphs each for validation and testing.

\textbf{Scoring.}
To measure a model's score on a graph, we first run the model on the graph with a random initial vector assignment to generate an SDP output, and then round this output to an integral solution using 1,000 random hyperplanes. For the graph, we retain the best score achieved by any hyperplane.

We ran validation periodically during each training run and retained the model that achieved the highest validation score. Then for each model and dataset, we selected the hyperparameter setting that achieved the highest validation score, and we report the average score measured on the test slice. Please see \ref{sec:hyperparams} for further details on the hyperparameter ranges used.

In \autoref{tab:forced_rb} and \autoref{tab:cut_neural}, at test time, we use 100 random initial vector assignments instead of just 1, and retain the best score achieved by any hyperplane on any random initial vector assignment. We use 1 random initial vector assignment for validation as in other cases.

\textbf{Hardware.}
Our training runs used 20 cores of an Intel Xeon Gold 6248 (for data loading and random graph generation) and a NVIDIA Tesla V100 GPU.
Our Gurobi runs use 8 threads on a Intel Xeon Platinum 8260.
Our KaMIS runs use an Intel Core i9-13900H.
Our LwD and \textsc{Dgl-TreeSearch} runs use an Intel Core i9-13900H and an RTX 4060.

\begin{figure}[]
\centering
\small
\begin{tabular}{lllllll}
\toprule
    Parameter & ER, BA, WS, HK & RB200 & RB500 & 3-SAT & \textbf{TU-small} & \textbf{TU-REDDIT} \\
\midrule
    Gradient steps & 20,000 & 200,000 & 100,000 & 100,000 & 100,000 & 100,000 \\
    Validation freq & 1,000 & 2,000 & 2,000 & 2,000 & 1,000 & 2,000 \\
    Batch size & 16 & 32 & 32 & 32 & 16 & 16 \\
    Ranks & 4, 8, 16, 32 & 32, 64 & 32, 64 & 32, 64 & 4, 8, 16, 32 & 4, 8, 16, 32 \\
    Layer counts & 8, 16 & 16 & 16 & 16 & 8, 16 & 8, 16 \\
    Positional encodings & RW & none & none & none & LE, RW & RW \\
\midrule
    \textbf{Run count} & 8 & 2 & 2 & 2 & 16 & 8 \\
\bottomrule
\end{tabular}
\caption{Hyperparameter range explored for each group of datasets. For each NN architecture, when training on a dataset, we explored every listed hyperparameter combination in the corresponding column.}
\label{tab:hyperparams}
\end{figure}

\textbf{Hyperparameters.}\label{sec:hyperparams}
We ran each experiment on a range of hyperparameters. See \autoref{tab:hyperparams} for the hyperparameter listing. For all training runs, we used the Adam optimizer~\cite{kingma2014adam} with a learning rate of 0.001. We used Laplacian eigenvector~\cite{dwivedi2020benchmarking} (LE) or random walk~\cite{dwivedi2021graph} (RW) positional encoding with dimensionality of half the rank, except for rank 32 where we used 8 dimensions. For Max-3-SAT, we set the penalty term $\rho = 0.003$.

\subsection{Max-3-SAT} \label{sec:max3sat-extra-info}
\textbf{Erd\H{o}sGNN}. The Erd\H{o}sGNN baseline accepts as input a clause-variable bipartite graph of the SAT formula and the node degrees as input attributes. Each variable $x_i$ is set to TRUE with probability $p_i$. A graph neural network (GatedGCNN) is trained until convergence ($\sim$50k iterations) with randomly generated formulae with clause to variable ratiot in the range $[4,4.3]$. The neural network is trained to produce output probabilities $p_i$ by minimizing the expected number of unsatisfied clauses. The exact closed form of the expectation can be found in \citep{karalias2023probabilistic}. At inference time, the probabilities are rounded to binary assignments using the method of conditional expectation.

\textbf{WalkSAT.} We use a publicly available python implementation of WalkSAT and we set the max number of variable flips to $4 \times$number of variables, for a total of 400 flips on the instances we tested.

\textbf{Autograd.}\label{sec:autograd}
The autograd comparison measures the performance of autograd on the same loss as OptGNN.
Starting with some initial node embeddings for the instance, the Lagrangian is computed for the problem and the node embeddings are updated by minimizing the Lagrangian using Adam. This process is run for several iterations. After it is concluded, the vectors are rounded with hyperplane rounding, yielding a binary assignment for the variables of the formula.

\textbf{Autograd parameters.} We use the Adam optimizer with learning rate 0.1 for 1000 epochs with penalty 0.01 and round with 10,000 hyperplanes, which is 10 times as many as that used by OptGNN.  
% \begin{table}[!htbp]
% \small
% \input{maxcut_ratio_model.tex}
% \caption{Performance of various model architectures for selected datasets on Maximum Cut. Here, higher is better.}
% \label{tab:cut_ratio_models}
% \end{table}

% \begin{table}[!htbp]
% \small
% \input{VC_ratio_model.tex}
% \caption{Performance of various model architectures for selected datasets on Min-Vertex-Cover. Here, lower is better.}
% \label{tab:VC_ratio_models}
% \end{table}

\subsection{Additional Results}
\label{sec:complete-results}

\subsubsection{Comparisons with Gurobi and Greedy}
\autoref{tab:cut_baselines} and \autoref{tab:VC_baselines} contain comparisons on additional datasets with Gurobi and Greedy.

\begin{table}[!htbp]
\centering
\small
\input{VC_baseline_table}
\caption{Performance of OptGNN, Greedy, and Gurobi 0.1s, 1s, and 8s on Min-Vertex-Cover. For each approach and dataset, we report the average Vertex-Cover size measured on the test slice. Here, lower score is better. In parentheses, we include the average runtime in \textit{milliseconds} for OptGNN.}
\label{tab:VC_baselines}
\end{table}

% \autoref{tab:VC_baselines} presents the average size of the Vertex-Cover achieved by OptGNN and classical baselines on our datasets. For this problem OptGNN also performs nearly as well as Gurobi 8s, remaining within 1\% on the TU datasets and 3.1\% on the worst case, ER (100, 200). OptGNN in certain cases outperforms Gurobi when considering execution time. Indeed, OptGNN requires only a few milliseconds to execute and is able to frequently outperform Gurobi when the latter is given a comparable time budget (0.1s). However, Gurobi with a 1s time budget is able to solve many of the datasets to optimality. While more computationally expensive than OptGNN, this constitutes only a small increase in total execution time for the entire dataset so Gurobi remains an extremely strong baseline.

\begin{table}[!htbp]
\centering
\small
\input{maxcut_baseline_table}
\caption{Performance of OptGNN, Greedy, and Gurobi 0.1s, 1s, and 8s on Maximum Cut. For each approach and dataset, we report the average cut size measured on the test slice. Here, higher score is better. In parentheses, we include the average runtime in \textit{milliseconds} for OptGNN.}
\label{tab:cut_baselines}
\end{table}

% Overall, we can see that OptGNN can consistently outperform a greedy algorithm and is competitive with Gurobi when execution time is taken into account. 
% \autoref{tab:cut_baselines} presents results for the maximum cut problem. Specifically, we report the average integral cut value achieved by OptGNN and classical baselines on a variety of datasets. We note that Greedy achieves poor performance compared to OptGNN and Gurobi on every dataset, indicating that for these datasets, finding Maximum Cut is not trivial. On the worst case, WS (400, 500), OptGNN achieves a cut value within 1.1\% on average of Gurobi with an 8s time limit. On other datasets, OptGNN is typically within a fraction of a percent. Notably, OptGNN is within 0.1\% of Gurobi 8s on all the TU datasets.

\subsubsection{Ratio tables}
In \autoref{tab:cut_ratios} and \autoref{tab:VC_ratios} we supply the performance of OptGNN as a ratio against the integral value achieved by Gurobi running with a time limit of 8 seconds. These tables include the standard deviation in the ratio. We note that for Maximum Cut, OptGNN comes within 1.1\% of the Gurobi 8s value, and for Min-Vertex-Cover, OptGNN comes within 3.1\%.


\begin{figure}[!htbp]
\centering
\small
\input{maxcut_ratio_baseline.tex}
\caption{Performance of OptGNN on Max-Cut compared to Gurobi running under an 8 second time limit, expressed as a ratio. For each dataset, we take the ratio of the integral values achieved by OptGNN and Gurobi 8s on each of the graphs in the test slice. We present the average and standard deviation of these ratios. Here, higher is better. This table demonstrates that OptGNN achieves nearly the same performance, missing on average 1.1\% of the cut value in the worst measured case.}
\label{tab:cut_ratios}
\end{figure}

\begin{figure}[!htbp]
\centering
\small
\input{VC_ratio_baseline.tex}
\caption{Performance of OptGNN on Min-Vertex-Cover compared to Gurobi running under an 8 second time limit, expressed as a ratio. For each dataset, we take the ratio of the integral values achieved by OptGNN and Gurobi 8s on each of the graphs in the test slice. We present the average and standard deviation of these ratios. Here, lower is better. This table demonstrates that OptGNN achieves nearly the same performance, producing a cover on average 3.1\% larger than Gurobi 8s in the worst measured case.}
\label{tab:VC_ratios}
\end{figure}


\subsection{Model ablation study}\label{sec:VC_ablation}Here we provide the evaluations of several models that were trained on the same loss as OptGNN. We see that OptGNN consistently achieves the best performance among different neural architectures.
Note that while OptGNN was consistently the best model, other models were able to perform relatively well; for instance, GatedGCNN achieves average cut values within a few percent of OptGNN on nearly all the datasets (excluding COLLAB). This points to the overall viability of training using an SDP relaxation for the loss function.

\begin{table*}[!htbp]
\scriptsize
\centering
\input{maxcut_model_table.tex}
\caption{Performance of various model architectures for selected datasets on Maximum Cut. Here, higher is better. GAT is the Graph Attention network \citep{velivckovic2018graph}, GIN is the Graph Isomorphism Network \citep{xu2018how}, GCNN is the Graph Convolutional Neural Network \citep{morris2019weisfeiler}, and GatedGCNN is the gated version \citep{li2015gated}.}
\label{tab:cut_models}
\end{table*}
\autoref{tab:VC_models} presents the performance of alternative neural network architectures on Min-Vertex-Cover.
\begin{table}[!htbp]
\scriptsize
\centering
\input{VC_model_table.tex}
\caption{Performance of various model architectures compared to OptGNN for selected datasets on Min-Vertex-Cover. Here, lower is better.}
\label{tab:VC_models}
\end{table}

\subsection{Effects of hyperparameters on performance}
\autoref{fig:hparam_vc} and \autoref{fig:hparam_mc} present overall trends in model performance across hyperparameters.
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{hparam_vc_tusmall.png}
        \caption{On \textbf{TU-small} datasets.}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{hparam_vc_generated.png}
        \caption{On generated datasets.}
    \end{subfigure}
    \caption{Trends in model performance on Min-Vertex-Cover with respect to the number of layers, hidden size, and positional encoding of the models.}
    \label{fig:hparam_vc}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{hparam_mc_tusmall.png}
        \caption{On \textbf{TU-small} datasets.}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{hparam_mc_generated.png}
        \caption{On generated datasets.}
    \end{subfigure}
    \caption{Trends in model performance on Max-Cut with respect to the number of layers, hidden size, and positional encoding of the models.}
    \label{fig:hparam_mc}
\end{figure}

\subsection{Out of distribution testing} \label{sec:oodtest}
% \begin{table*}[!htbp]
% \small
% \centering
% \input{maxcut_model_table.tex}
% \caption{Performance of various model architectures for selected datasets on Maximum Cut. Here, higher is better. GAT is the Graph Attention network \citep{velivckovic2018graph}, GIN is the Graph Isomorphism Network \citep{xu2018how}, GCNN is the Graph Convolutional Neural Network \citep{morris2019weisfeiler}, and GatedGCNN is the gated version \citep{li2015gated}.}
% \label{tab:cut_models}
% \end{table*}

\begin{table}[!h] 
\centering
\scriptsize
\input{generalizability_table.tex}
\caption{Models for Min-Vertex-Cover trained on "dataset" were tested on a selection of the TU datasets ({ENZYMES, PROTEINS, MUTAG, IMDB-BINARY, and COLLAB}). We observe that the performance of the models generalizes well even when they are taken out of their training context.}
\label{tab:generalization}
\end{table}

OptGNN trained on one dataset performed quite well on other datasets without any finetuning, suggesting that the model can generalize to examples outside its training distribution.
For each dataset in our collection, we train a model and then test the trained model on a subset of datasets in the collection. The results are shown in \autoref{tab:generalization}.
It is apparent from the results that the model performance generalizes well to different datasets. Interestingly, we frequently observe that the model reaches its peak performance on a given test dataset even when trained on a different one. This suggests that the model indeed is capturing elements of a more general process instead of just overfitting the training data.



\subsection{Pseudocode for OptGNN training and inference} \label{sec:pseudocode}
In \algref{alg:OptGNNpseudocodemaxcut}, we present pseudocode for OptGNN in the Max-Cut case and in \algref{alg:OptGNNpseudocodegeneral} pseudocode for the forward pass of a general SDP.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \makeatletter
% % \renewcommand{\ALG@name}{Algorithm}
% % \makeatother
\begin{algorithm} 
%\setcounter{algorithm}{3}
\caption{OptGNN pseudocode for Max-Cut forward pass}
\label{alg:OptGNNpseudocodemaxcut} %\setcounter{algorithm}{3}
\begin{algorithmic}[1]
%\Procedure{Message Passing}{$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}
\REQUIRE graph $G$
\STATE $\mathbf{v}^0 = \{v_1, v_2, \dots, v_N\}$ (random initial feature vectors and/or positional encodings)
\FOR{$t=1,2,3,\dots, T$} 
\FOR{$v_i^t \in \mathbf{v}^t$} 
\STATE ${v}_i^{t+1} \gets {v}_i^{t} + \sum_{j \in N(i)}v_j^t$
\STATE $\hat{v}_i^{t+1} \gets \text{Linear}(\frac{{v}_i^{t+1}}{|{v}_i^{t+1}|}) $
\ENDFOR 
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
%\setcounter{algorithm}{4}
\caption{OptGNN pseudocode for implementing a general SDP forward pass}
\label{alg:OptGNNpseudocodegeneral} %\setcounter{algorithm}{4}
\begin{algorithmic}[1]
%\Procedure{Message Passing}{$\Lambda = (\mathcal{V},\mathcal{P},\{0,1\})$}
\REQUIRE graph $G$
\STATE $\mathbf{v}^0 = \{v_1, v_2, \dots, v_N\}$  (random initial feature vectors and/or positional encodings)
\FOR{$t=1,2,3,\dots, T$} 
\FOR{$v_i^t \in \mathbf{v}^t$} 
\STATE ${v}_i^{t+1} \gets {v}_i^{t} + \text{Autograd}(\mathcal{L}( \mathbf{v}_i^{t};G))$
\STATE $\hat{v}_i^{t+1} \gets \text{Linear}(\frac{{v}_i^{t+1}}{|{v}_i^{t+1}|}) $
\ENDFOR 
\ENDFOR
\end{algorithmic}
\end{algorithm}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\include{alignment.tex}
\include{hessian.tex}
% \begin{tabular}{llrrrr}
% \toprule
%             Dataset &         OptGNN &  Greedy & {Gurobi}& Gurobi & Gurobi \\
%               &             &      &     0.1s &     1.0s &     8.0s \\
% \midrule
% BA\textsuperscript{a} (400,500) &   2197.99 (66) & 1255.22 &  2208.11 &  2208.11 &  2212.49 \\
% ER\textsuperscript{a} (400,500) & 16387.46 (225) & 8622.34 & 16476.72 & 16491.60 & 16495.31 \\
% HK\textsuperscript{a} (400,500) &   2159.90 (61) & 1230.98 &  2169.46 &  2169.46 &  2173.88 \\
% WC\textsuperscript{a} (400,500) &   1166.47 (78) &  690.19 &  1173.45 &  1175.97 &  1179.86 \\
%       COLLAB\textsuperscript{b} &   2622.41 (22) & 1345.70 &  2624.32 &  2624.57 &  2624.62 \\
%  REDDIT-M-5K\textsuperscript{c} &   786.09 (133) &  495.02 &   785.44 &   787.48 &   787.92 \\
% \bottomrule
% \end{tabular}



% \begin{tabular}{llrrrr}
% \toprule
%             Dataset &      OptGNN & Greedy &  {Gurobi}& Gurobi & Gurobi \\
%               &          &     &   0.1s &   1.0s &   8.0s \\
% \midrule
% BA\textsuperscript{a} (400,500) & 248.74 (27) & 302.53 & 256.33 & 246.49 & 246.46 \\
% ER\textsuperscript{a} (400,500) & 420.70 (41) & 442.84 & 423.07 & 423.07 & 415.52 \\
% HK\textsuperscript{a} (400,500) & 249.26 (27) & 298.98 & 247.90 & 247.57 & 247.57 \\
% WC\textsuperscript{a} (400,500) & 274.21 (31) & 434.52 & 269.58 & 269.39 & 269.39 \\
% COLLAB\textsuperscript{b} &  67.50 (23) &  71.74 &  67.47 &  67.46 &  67.46 \\ REDDIT-M-5K\textsuperscript{c} & 107.36 (33) & 153.24 & 108.73 & 107.32 & 107.32 \\
% \bottomrule
% \end{tabular}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%COPY PASTE
% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite

==> maxcut.tex <==
\begin{lemma}[Lipschitz Gradient Lemma Max Cut]\label{lem:maxcut-gradient} Let $\mathcal{L}_\rho(\cdot)$ be the penalized loss of any Max Cut instance.  
\[
\mathcal{L}_\rho(V) = -\frac{1}{|E|}\left[\left(\frac{|E|}{2} - \frac{1}{4}\langle A, VV^T\rangle \right) + \rho \sum_{i \in [N]}(\|v_i\|^2 - 1)^2\right]
\]
Where we negate the objective so that we're working with minimization.  Then we have that the gradient of $\mathcal{L}_\rho(\cdot)$ satisfies 
\[\left\|\nabla\mathcal{L}_\rho(V) - \nabla\mathcal{L}_\rho(\hat{V})\right\|_F \leq O(\rho B^2)\left\| V - \hat{V}\right\|_F \]
\end{lemma}
\begin{proof} First we prove the lipschitzness of the gradient. 
Consider the form of the max cut gradient 
\[
\nabla \mathcal{L}_\rho(V) = 
\begin{cases}
\frac{\partial \mathcal{L}_\rho}{\partial v_i} =  \frac{1}{|E|}\left[\sum_{j \in N(i)} v_j + 2\rho(\|v_i\|^2 - 1)v_i\right], & \text{for } i \in [N] \\
\end{cases}
\]
We bound the lipschitz constant as follows.  First by definition,  

\begin{align*}
\left\|\nabla \mathcal{L}_\rho(V) - \nabla \mathcal{L}_\rho(\hat{V})\right\|_F 
&= \frac{1}{|E|}\sqrt{\sum_{i \in [N]} \left\| \sum_{j \in N(i)} (v_j - \hat{v}_j) + 2\rho \left((\|v_i\|^2 - 1)v_i - (\|\hat{v}_i\|^2-1)\hat{v_i}\right) \right\|^2}
\end{align*}

By triangle inequality we upper bound by
\begin{align}
\leq \frac{1}{|E|}\sqrt{\sum_{i \in [N]}\left(\sum_{j \in N(i)} (v_j - \hat{v}_j) \right)^2} + \frac{1}{|E|}\sqrt{\sum_{i \in [N]}4\rho^2\left\| (\left\|v_i\right\|^2 - 1)v_i - (\left\|\hat{v}_i\right\|^2-1)\hat{v}_i\right\|^2}
\end{align}


It suffices to independently bound the two terms above which we denote 

\[\mathcal{T}_1 \defeq \frac{1}{|E|}\sqrt{\sum_{i \in [N]}\left\|\sum_{j \in N(i)} (v_j - \hat{v}_j) \right\| ^2}\] 
and 
\[\mathcal{T}_2 \defeq \frac{1}{|E|}\sqrt{\sum_{i \in [N]}4\rho^2 \left\| \left(\left(\left\|v_i\right\|^2 - 1\right)v_i - \left(\left\|\hat{v}_i\right\|^2 - 1\right)\hat{v}_i\right)\right\|^2}\]
To bound the first term $\mathcal{T}_1$ , note that 
\begin{align}
\mathcal{T}_1 \defeq \frac{1}{|E|}\| A (V- \hat{V})\|_F &\leq \frac{1}{|E|}\| A \|_F \|V- \hat{V}\|_F \\
&\leq \frac{1}{\sqrt{|E|}} \|V- \hat{V}\|_F
\end{align}


Where in the last inequality we used the fact that any adjacency matrix $A$ has a frobenius norm upper bounded by  $\|A\|_F \leq \sqrt{|E|}$.  
It remains to bound $\mathcal{T}_2$.  
\[\mathcal{T}_2 \defeq \frac{1}{|E|}\sqrt{\sum_{i \in [N]}4\rho^2 \left\| \left(\left(\left\|v_i\right\|^2 - 1\right)v_i - \left(\left\|\hat{v}_i\right\|^2 - 1\right)\hat{v}_i\right)\right\|^2}\]

Let $\omega_i \defeq \|v_i\|^2 - 1 \in \R$ and $\hat{\omega}_i \defeq \|\hat{v}_i\|^2 - 1 \in \R$. Let $\delta_{w_i} = \omega_i - \hat{\omega}_i \in \R$ and $\delta_{v_i} \defeq v_i - \hat{v_i} \in \R^{|\mathcal{P}|2^k}$.  Then we have   

\[\mathcal{T}_2 = \sqrt{\sum_{i \in [N]}4\rho^2\left\| \omega_i v_i - \hat{\omega}_i\hat{v}_i\right\|^2} =  \sqrt{\sum_{i \in [N]}4\rho^2\left\| \omega_i v_i - (\omega_i + \delta_{\omega})(v_i + \delta_{v_i})\right\|^2}\]

\begin{align}
=  \sqrt{\sum_{i \in [N]}4\rho^2\left\| -\delta_{\omega_i}v_i - \omega_i \delta_{v_i} + \delta_{\omega_i}\delta_{v_i}\right\|^2}
\end{align}
Upper bounding via triangle inequality we obtain 
\begin{align}
 \leq O(\rho^2) \sqrt{\sum_{i \in [N]}\big(\|\delta_{\omega_i}v_i\|^2 + \|\omega_i \delta_{v_i}\|^2 + \|\delta_{\omega_i}\delta_{v_i}\|^2\big)}
\end{align}

Upper bounding the norm of vectors $\|v_i\| \leq B$ we obtain 

\[\leq O(\rho^2) \sqrt{\sum_{i \in [N]}\big(\delta_{\omega_i}^2 B^2 + B^2\|\delta_{v_i}\|^2 + \delta_{\omega_i}^2\|\delta_{v_i}\|^2\big)}\]
For the second term in the square root, rewriting in terms of matrices $\|V-\hat{V}\|_F^2 = \sum_{i \in [N]} \|\delta_{v_i}\|^2$ we obtain 
\begin{align} \label{eq:77}
\leq O(\rho) \sqrt{ \sum_{i \in [N]} \delta_{w_i}^2 B^2 + B^2\|V - \hat{V}\|_F^2 + \sum_{i \in [N]}\delta_{\omega_i}^2\|\delta_{v_i}\|^2}
\end{align}
Note that the first term in the square root can be upper bounded as follows   
\begin{align}
B^2\sum_{i \in [N]} \delta_{w_i}^2 &= B^2\sum_{i \in [N]} (\| v_i\|^2 - \|\hat{v_i}\|^2)^2 \\
&= B^2\sum_{i \in [N]} (\| v_i\| - \|\hat{v_i}\|)^2(\| v_i\| + \|\hat{v_i}\|)^2 \\
&\leq B^4\sum_{i \in [N]} (\| v_i\| - \|\hat{v_i}\|)^2 \\
&\leq B^4\sum_{i \in [N]} \| v_i - \hat{v_i}\|^2 \\
&= B^4\|V - \hat{V}\|_F^2
\end{align}
Plugging this bound into \eqref{eq:77} we obtain 
\begin{align}
\ref{eq:77} \leq  O(\rho) \sqrt{ B^4 \| V - \hat{V}\|_F^2 + B^2\|V - \hat{V}\|_F^2 + \sum_{i \in [N]}\delta_{\omega_i}^2\|\delta_{v_i}\|^2}
\end{align}
Moving on to the third term in the square root, we upper bound $|\delta_{w_i}| \leq B$ we obtain 
\[\leq O(\rho) \sqrt{\|V - \hat{V}\|_F^2 B^4 + B^2\sum_{i \in [N]}\|\delta_{v_i}\|^2}\]
Again using the fact that $\|V-\hat{V}\|_F^2 = \sum_{i \in [N]} \|\delta_{v_i}\|^2$ we obtain
\[\mathcal{T}_2 \leq O(\rho B^2)\|V - \hat{V}\|_F\]
as desired.  Putting together our bound for $\mathcal{T}_1$ and $\mathcal{T}_2$ we obtain
\begin{align*}
\left\|\nabla \mathcal{L}_\rho(V) - \nabla \mathcal{L}_\rho(\hat{V})\right\|_F 
& \leq \frac{1}{\sqrt{|E|}} \|V- \hat{V}\|_F + O(\rho B^2)\|V - \hat{V}\|_F\\ &
\leq O(\rho B^2)\|V - \hat{V}\|_F
\end{align*}
Where in the last inequality we assume the number of edges is greater than 1.  This concludes the proof.  
\end{proof}

\begin{lemma} [Smooth Hessian Lemma Max Cut]  For a MaxCut instance $\Lambda$, Let $\mathcal{L}_\rho(\mathbf{v})$ be the normalized loss defined in \eqref{eq:loss-normalize}.  Then the hessian satisfies
\[\big\|\nabla^2 \mathcal{L}_\rho(\mathbf{v}) - \nabla^2 \mathcal{L}_\rho(\mathbf{\hat{v}}) \| \leq 8\rho\|V - \hat{V}\|_F \]
In particular for $\rho = poly(\epsilon^{-1})$ we have that the hessian is $poly(\epsilon^{-1})$ smooth.   
\end{lemma}   
\begin{proof}
Definition of smoothness of Hessian.  

\[\|\nabla^2 \mathcal{L}(\mathbf{v}) - \nabla^2 \mathcal{L}(\mathbf{\hat{v}})\| \leq \rho \|V - \hat{V}\|_F\]
Here the norm on the left is operator norm.  Consider the form of the max cut hessian $\nabla^2 \mathcal{L}_\rho(V)$.   


\[
\nabla^2 \mathcal{L}(V) \defeq 
\begin{cases} 
  \frac{\partial \mathcal{L}(V)}{\partial v_{ia}\partial v_{jb} } = \frac{1}{|E|}, & \text{for } j \in N(i) \text{ } a,b \in [r] \\
  \frac{\mathcal{L}(V)}{\partial v_{ia}\partial v_{ib} } = \frac{8\rho v_{ib}v_{ia}}{|E|}, & \text{for } i \in [N] \text{ } a,b \in [r] 
\end{cases}
\]
Now we compute the smoothness.  The key is that the hessian has the sparsity structure of the adjacency matrix of the constraint graph encoded.  
\[\|\nabla^2 \mathcal{L}(V) - \nabla^2 \mathcal{L}(\hat{V})\| \leq \| \mathcal{L}(V) - \mathcal{L}(\hat{V}) \|_F\]
Where we upper bounded the operator norm by frobenius norm 
Let $\nabla^2 \mathcal{L}(V) = \frac{1}{|E|}\big(\mathcal{H}_{\emptyset}(V) + \mathcal{H}_{\upsilon}(V)\big)$, where $\mathcal{H}_{\emptyset}(V)$ is the set of entries in the hessian that are constant and $\mathcal{H}_{\upsilon}(V)$ is the set of entries that are not constant.  Then we have     
\[\|\nabla^2 \mathcal{L}(V_1) - \nabla^2 \mathcal{L}(\hat{V})\| \leq \frac{1}{|E|} \| \mathcal{H}_{\emptyset}(V) - \mathcal{H}_{\emptyset}(\hat{V}) + \mathcal{H}_{\upsilon}(V) - \mathcal{H}_{\upsilon}(\hat{V}) \|_F \]
We have $\mathcal{H}_{\emptyset}(V) - \mathcal{H}_{\emptyset}(\hat{V}) = 0$ because they're both constants by definition.  Then we have 
\[ = \frac{1}{|E|} \| \mathcal{H}_{\upsilon}(V) - \mathcal{H}_{\upsilon}(\hat{V}) \|_F \]
Then using the fact that each nonzero entry of 
\[\frac{8\rho}{|E|}\sqrt{\sum_{i \in [N]}\sum_{a,b \in [r]}(v_{ia}v_{ib} - \hat{v}_{ia}\hat{v}_{ib})^2} \leq \frac{1}{|E|}\sqrt{\sum_{i \in [N]}\sum_{a,b \in [r]}\big(v_{ia}^2v_{ib}^2 + \hat{v}_{ia}^2\hat{v}_{ib}^2 - 2v_{ia}v_{ib}\hat{v}_{ia}\hat{v}_{ib}\big)}\]

\[= \frac{8\rho}{|E|}\sqrt{\sum_{i \in [N]}\big(\sum_{a,b \in [r]}v_{ia}^2v_{ib}^2 + \sum_{a,b \in [r]}\hat{v}_{ia}^2\hat{v}_{ib}^2 - \sum_{a,b \in [r]}2v_{ia}v_{ib}\hat{v}_{ia}\hat{v}_{ib}\big)}\]

\[= \frac{8\rho}{|E|}\sqrt{\sum_{i \in [N]}\big((\sum_{a \in [r]}v_{ia}^2)^2 + (\sum_{a \in [r]}\hat{v}_{ia}^2)^2 - 2\langle v_{i},\hat{v}_{i}\rangle^2\big)}\]

\[= \frac{8\rho}{|E|}\sqrt{\sum_{i \in [N]} \|v_i - \hat{v}_i \|^2} = \frac{8\rho}{|E|}\|V - \hat{V} \|_F \leq O(\rho)\|V - \hat{V} \|_F\]
as desired.  
\end{proof}

==> maxcut_neural.tex <==
\begin{tabular}{lllll}
\toprule
Method  & $N=800$ & $N=1000$ & $N=2000$ & $N\geq 3000$ \\ \midrule 
Greedy  & 411.44  & 359.11   & 737.00   & 774.25       \\ 
SDP     & 245.44  & 229.22   & -        & -            \\ 
Low-Rank SDP (\citep{wang2019low}) & 153.88 & 149.00 & 335.00 & 331.37
     \\ \midrule
RUNCSP  & 185.89  & 156.56   & 357.33   & 401.00       \\ 
ECO-DQN & 65.11   & 54.67    & 157.00   & 428.25       \\ 
ECORD   & 8.67    & 8.78     & 39.22    & 187.75       \\ 
ANYCSP  & 1.22    & 2.44     & 13.11    & 51.63        \\ \midrule 
OptGNN   & 109.22  & 125.00   & 284.67   & 549.38       \\ \bottomrule
\end{tabular}

==> maxcut_ratio_models.tex <==
\begin{tabular}{llllll}
\toprule
         Dataset &             GAT &            GCNN &             GIN &       GatedGCNN &          OptGNN \\
\midrule
 \midrule 
ER\textsuperscript{a} (50,100) & 0.992 $\pm$ 0.005 & 0.944 $\pm$ 0.021 & \textbf{0.940} $\pm$ 0.015 & 0.994 $\pm$ 0.005 & 0.998 $\pm$ 0.002 \\
ER\textsuperscript{a} (100,200) & 0.988 $\pm$ 0.004 & \textbf{0.943} $\pm$ 0.019 & 0.944 $\pm$ 0.010 & 0.988 $\pm$ 0.004 & 0.996 $\pm$ 0.002 \\
ER\textsuperscript{a} (400,500) & 0.989 $\pm$ 0.002 & \textbf{0.951} $\pm$ 0.006 & 0.959 $\pm$ 0.003 & 0.982 $\pm$ 0.002 & 0.993 $\pm$ 0.001 \\
       \midrule 
MUTAG\textsuperscript{b} & 0.994 $\pm$ 0.016 & \textbf{0.972} $\pm$ 0.033 & 0.974 $\pm$ 0.053 & \textbf{1.000} $\pm$ 0.000 & \textbf{1.000} $\pm$ 0.000 \\
     ENZYMES\textsuperscript{b} & 0.992 $\pm$ 0.010 & 0.903 $\pm$ 0.091 & \textbf{0.896} $\pm$ 0.088 & \textbf{0.999} $\pm$ 0.003 & \textbf{0.999} $\pm$ 0.003 \\
    PROTEINS\textsuperscript{b} & 0.993 $\pm$ 0.010 & \textbf{0.888} $\pm$ 0.088 & 0.927 $\pm$ 0.046 & 0.997 $\pm$ 0.005 & \textbf{1.000} $\pm$ 0.002 \\
    IMDB-BIN\textsuperscript{b} & 0.834 $\pm$ 0.111 & \textbf{0.764} $\pm$ 0.145 & 0.829 $\pm$ 0.115 & 0.997 $\pm$ 0.008 & \textbf{1.000} $\pm$ 0.001 \\
      COLLAB\textsuperscript{b} & 0.990 $\pm$ 0.011 & \textbf{0.814} $\pm$ 0.160 & 0.899 $\pm$ 0.131 & 0.922 $\pm$ 0.090 & \textbf{0.999} $\pm$ 0.002 \\
%   \midrule 
%REDDIT-BIN\textsuperscript{c} &                 &                 &                 &                 & \textbf{1.000} $\pm$ 0.001 \\
%REDDIT-M-12K\textsuperscript{c} &                 &                 &                 &                 & \textbf{0.999} $\pm$ 0.002 \\
% REDDIT-M-5K\textsuperscript{c} &                 &                 &                 &                 & \textbf{0.999} $\pm$ 0.002 \\
\bottomrule
\end{tabular}

==> removed.tex <==
Moving on, consider the dual feasibility condition 
\[C = Q + \sum_{i \in \mathcal{F}} \lambda_i A_i\]
for some $Q \succeq 0$.  Then we have 
\[\langle C,X^* - \Tilde{X}\rangle = \langle Q,X^* \rangle - \langle Q,\Tilde{X}\rangle  + \sum_{i \in \mathcal{F}} \lambda_i \langle A_i, X^* - \Tilde{X} \rangle \]
By complementary slackness $\langle Q,X^*\rangle = 0$ so we obtain
\[ = - \langle Q,\Tilde{X} \rangle + \sum_{i \in \mathcal{F}} \lambda_{i} \langle A_i, X^* - \Tilde{X} \rangle \]
By PSD'ness of both $Q$ and $\Tilde{X}$ we upper bound by 
\[ \leq  \sum_{i \in \mathcal{F}} \lambda_i \langle A_i, X^* - \Tilde{X} \rangle  = 
 \sum_{i \in \mathcal{F}} \lambda_i (b_i - \langle A_i, \Tilde{X}\rangle ) \leq \sqrt{\sum_{i \in \mathcal{F}} \lambda_i^2} \| \tau\|\]
Where in the first equality we used the fact that $\langle A_i,\Tilde{X}\rangle = b_i$, and the second inequality is Cauchy-Schwarz.  Since we've already established that $\|\tau\| \propto \rho^{-1}$ we must simply bound the size of the dual variables $\lambda_i$.  To bound the size of $\lambda_i$, we separate the constraints $A_i$ into the diagonal constraints $\{F_i\}_{i \in \mathcal{W}}$ and equality constraints $\{G_i\}_{i \in \mathcal{R}}$ where 
\[\langle F_i,X\rangle = 1 \quad \forall i \in \mathcal{W} \quad \quad \langle G_i, X\rangle = 0 \quad \forall i \in \mathcal{R}\]   
The dual takes on the following form for $\delta,\eta \in \R$
\begin{align} \label{eq:dual-objective}
\text{Maximize: } \sum_{i \in \mathcal{W}} \delta_i
\end{align}
\begin{align}
\label{eq:dual-feasible}
\text{Subject to: }C - \sum_{i \in \mathcal{W}} \delta_i F_i - \sum_{i \in \mathcal{R}} \eta_i G_i \succeq 0
\end{align}

Where we've split the dual variables $\{\lambda_i \}_{i \in \mathcal{F}}$ into two sets $\{\delta_i\}_{i \in \mathcal{W}}$ and $\{\eta_i\}_{i \in \mathcal{R}}$.  Note that the $\delta_i$ are polynomially bounded i.e $|\delta_i| \leq poly(|\mathcal{P}|,2^k)$.  Assume the contrary, if $\delta_i > poly(|\mathcal{P}|,2^k)$ then the objective is polynomially unbounded which contradicts dual objective being smaller than primal objective.  If $\delta_i < -poly(\mathcal{P},2^k)$ then the $i'th$ diagonal coordinate of \eqref{eq:dual-feasible} is polynomially unbounded and then $e_i$ is a negative eigenvalue of \eqref{eq:dual-feasible} which is a contradiction of PSD'ness.  Therefore, the $\delta_i$ are polynomially bounded.  To demonstrate the $\{\eta_i\}_{i \in \mathcal{R}}$ are polynomially bounded, note that because of linear independence of the constraints plus the minimum singular value being greater than a constant, there exists a setting of the $\eta$ that is polynomially bounded such that the dual feasibility constraint is satisfied. Since the $\eta$ do not appear in the objective, finding a setting that satisfies \eqref{eq:dual-feasible} suffices.  

\paragraph{Constraint matrix is well conditioned.} The smallest singular value of $\{A_i\}_{i \in \mathcal{F}}$ is a constant.  This is a technical observation the $\{A_i\}_{i \in \mathcal{F}}$ matrices which are collections of vectors of the form $\{e_1 + e_j\}_{j \in [2,T]}$ where we let $e_i$ denote the $i'th$ standard basis vector.  Any unit vector $v$ satisfies $\|\sum_j v_j(e_1 + e_j)\| = (\sum_j v_j)^2 + \sum_j v_j^2 \geq 1$.

==> sat.tex <==
\section{Max-3-SAT OptGNN} \label{sec:max3sat}
Our formulation for Max 3-SAT directly translates the $\text{OptGNN}$ architecture from \defref{def:OptGNN-maxcsp}.
Let $\Lambda$ be a 3-SAT instance with a set of clauses $\mathcal{P}$ over a set of binary literals $\mathcal{V} =\{x_1,x_2,...,x_N\} \in \{-1,1\}$.  Here $-1$ corresponds to assigning the literal to False whilst $1$ corresponds to True. Each clause $P_z \in \mathcal{P}$ can be specified by three literals $(x_i,x_j,x_k)$ and a set of three 'tokens'  $(\tau_i,\tau_j,\tau_k) \in \{-1,1\}^3$ which correspond to whether the variable $x_i,x_j,x_k$ are negated in the clause.   For instance the clause $(x_1 \vee \neg x_2 \vee x_3)$ is translated into three literals $(x_1,x_2,x_3)$ and tokens $(1,-1,1)$.    

The 3-SAT problem on instance $\Lambda$ is equivalent to maximizing the following polynomial   
\begin{align}
\sum_{(x_i,x_j,x_k,\tau_i,\tau_j,\tau_k) \in \mathcal{P}} \big(1 - \frac{1}{8}(1+\tau_i x_i)(1+\tau_j x_j)(1+\tau_k x_k)\big)
\end{align}
Subject to the constraint $x_1,x_2,...,x_N \in \{1,-1\}$.  Now we're reading to define the $\text{OptGNN}$ for 3-SAT
\paragraph{Objective:} First we define the set of vector embeddings. For every literal $x_i$ we associate an embedding $v_i \in \R^r$.  For every pair of literals that appear in a clause $(x_i,x_j)$ we associate a variable $v_{ij} \in \R^r$.  Finally we associate a vector $v_\emptyset$ to represent $1$.  Then the unconstrained objective $\text{SAT}$ is defined as   

\begin{multline}
\text{SAT}(\Lambda) \defeq \sum_{(x_i,x_j,x_k,\tau_i,\tau_j,\tau_k) \in \mathcal{P}}\frac{1}{8}\Bigg(-\tau_i \tau_j \tau_k \frac{1}{3}\left[\langle v_i,v_{jk} \rangle + \langle v_j,v_{ik} \rangle + \langle v_k,v_{ij}\rangle\right]\\
- \tau_i\tau_j\frac{1}{2}\left[\langle v_i,v_j \rangle + \langle v_{ij},v_{\emptyset} \rangle\right] - \tau_i\tau_k\frac{1}{2}\left[\langle v_i,v_k \rangle + \langle v_{ik},v_{\emptyset} \rangle\right] - \tau_j\tau_k\frac{1}{2}\left[\langle v_j,v_k \rangle + \langle v_{jk},v_{\emptyset} \rangle\right]\\ - \tau_i\langle v_i,v_{\emptyset}\rangle - \tau_j\langle v_j,v_{\emptyset}\rangle - \tau_k\langle v_k,v_\emptyset\rangle + 7 \Bigg)
\end{multline}

\paragraph{Constraints: } The constraints are then as follows.  For every clause involving variables $(x_i,x_j,x_k)$ we impose the following constraints on $v_i,v_j,v_k,v_{ij},v_{ik},v_{jk}$ and $v_\emptyset$.  Note that these constraints are exactly the ones listed in \algref{alg:sdp-vector} which we organize here for convenience. The naming convention is the degree of the polynomial on the left to the degree of the polynomial on the right.    
\begin{enumerate}
  \item \textbf{pair-to-pair} 
  \begin{align}
      \langle v_i,v_j\rangle = \langle v_{ij}, v_{\emptyset}\rangle\\
      \langle v_i,v_k\rangle = \langle v_{ik}, v_{\emptyset}\rangle\\
      \langle v_j,v_k\rangle = \langle v_{jk}, v_{\emptyset}\rangle
  \end{align}
  \item \textbf{triplets-to-triplet}
  \begin{align}
      \langle v_{ij},v_k \rangle =
      \langle v_{ik},v_j \rangle =
    \langle v_{jk},v_i \rangle
  \end{align}
  \item \textbf{triplet-to-single}
  \begin{align}
  \langle v_i,v_{ij}\rangle = \langle v_j,v_{\emptyset} \rangle\\
  \langle v_j,v_{ij}\rangle = \langle v_i,v_{\emptyset}\rangle\\
  \langle v_j,v_{jk}\rangle = \langle v_k,v_{\emptyset}\rangle\\
  \langle v_k,v_{jk}\rangle = \langle v_j,v_{\emptyset}\rangle\\
  \langle v_i,v_{ik}\rangle = \langle v_k,v_{\emptyset}\rangle\\
  \langle v_k,v_{ik}\rangle = \langle v_i,v_{\emptyset}\rangle\\
  \end{align}
  \item \textbf{quad-to-pair} 
  \begin{align}
      \langle v_{ij},v_{jk}\rangle = \langle v_{i},v_{k}\rangle\\
      \langle v_{ij},v_{ik}\rangle = \langle v_{j},v_{k}\rangle\\
      \langle v_{ik},v_{jk}\rangle = \langle v_{i},v_{j}\rangle\\
  \end{align}
  \item \textbf{unit norm}
  \begin{align}
      \left\| v_i\right\| = \left\| v_j\right\| = \left\| v_k\right\| = \left\| v_{ij}\right\| = \left\| v_{ik}\right\| = \left\| v_{jk}\right\| = \left\| v_{\emptyset}\right\| = 1
  \end{align}
\end{enumerate}

Then for completeness we write out the full penalized objective.  We perform this exercise in such great detail to inform the reader of how this could be set up for other Max-CSP's.  
\begin{definition} [OptGNN for 3-SAT] Let $\Lambda$ be a 3-SAT instance.  Let $\mathcal{L}_\rho$ be defined as 
\begin{multline} \label{eq:83}
    \mathcal{L}_\rho(V) \defeq \sum_{(x_i,x_j,x_k,\tau_i,\tau_j,\tau_k) \in \mathcal{P}} \Biggr[-\frac{1}{8}\Bigg(-\tau_i \tau_j \tau_k \frac{1}{3}\left[\langle v_i,v_{jk} \rangle + \langle v_j,v_{ik} \rangle + \langle v_k,v_{ij}\rangle\right]\\
- \tau_i\tau_j\frac{1}{2}\left[\langle v_i,v_j \rangle + \langle v_{ij},v_{\emptyset} \rangle\right] - \tau_i\tau_k\frac{1}{2}\left[\langle v_i,v_k \rangle + \langle v_{ik},v_{\emptyset} \rangle\right] - \tau_j\tau_k\frac{1}{2}\left[\langle v_j,v_k \rangle + \langle v_{jk},v_{\emptyset} \rangle\right]\\ - \tau_i\langle v_i,v_{\emptyset}\rangle - \tau_j\langle v_j,v_{\emptyset}\rangle - \tau_k\langle v_k,v_\emptyset\rangle + 7 \Bigg) \\
+ \rho \left[ (\langle v_i,v_j\rangle - \langle v_{ij}, v_{\emptyset}\rangle)^2
      + (\langle v_i,v_k\rangle - \langle v_{ik}, v_{\emptyset}\rangle)^2 + 
      (\langle v_j,v_k\rangle -\langle v_{jk}, v_{\emptyset}\rangle)^2\right]\\
      + \rho\left[(\langle v_{ij},v_k \rangle -
      \langle v_{ik},v_j \rangle)^2 + (\langle v_{ik},v_j \rangle -\langle v_{jk},v_i \rangle)^2 + (\langle v_{jk},v_i \rangle - \langle v_{ij},v_k \rangle )^2\right]\\
      + \rho \left[(\langle v_{ij},v_{jk}\rangle - \langle v_{i},v_{k}\rangle)^2 + 
      (\langle v_{ij},v_{ik}\rangle - \langle v_{j},v_{k}\rangle)^2 + 
      (\langle v_{ik},v_{jk}\rangle - \langle v_{i},v_{j}\rangle)^2\right]\\
      \rho\big[(\langle v_i,v_{ij}\rangle - \langle v_j,v_{\emptyset} \rangle)^2 + 
  (\langle v_j,v_{ij}\rangle - \langle v_i,v_{\emptyset}\rangle)^2 + 
  (\langle v_j,v_{jk}\rangle - \langle v_k,v_{\emptyset}\rangle)^2 + 
  (\langle v_k,v_{jk}\rangle - \langle v_j,v_{\emptyset}\rangle)^2\\ + 
  (\langle v_i,v_{ik}\rangle - \langle v_k,v_{\emptyset}\rangle)^2 + 
  (\langle v_k,v_{ik}\rangle - \langle v_i,v_{\emptyset}\rangle)^2 \big]\\
      + \rho\left[ (\left\| v_i\right\| - 1)^2 + (\left\| v_j\right\| - 1)^2 + (\left\| v_k\right\| - 1)^2 + (\left\| v_{ij}\right\| - 1)^2 + (\left\| v_{ik}\right\| - 1)^2 + (\left\| v_{jk}\right\| - 1)^2 + (\left\| v_{\emptyset}\right\| - 1)^2\right]
      \Biggr]
\end{multline}

Then taking the gradient of $\mathcal{L}$ gives us the precise form of the message passing.  We list the forms of the messages from adjacent nodes in the constraint graph $G_\Lambda$.  
\paragraph{Message: Pair to Singles for Single in Pair.} This is the message $\text{MESSAGE}[v_{ij} \rightarrow v_i]$  for each pair node $v_{ij}$ to a single $v_i$ node.  
\begin{align}
\text{MESSAGE}[v_{ij} \rightarrow v_i] =
      |\{c \in \mathcal{P}: x_i,x_j \in c\}|2\rho (\langle v_i,v_{ij}\rangle - \langle v_j,v_\emptyset\rangle) v_{ij}
\end{align}
\paragraph{Message: Pair to Singles for Single not in Pair.} This is the message $\text{MESSAGE}[v_{ij} \rightarrow v_k]$  for each pair node $v_{ij}$ to a single $v_k$ node. 
\begin{multline}
\text{MESSAGE}[v_{ij} \rightarrow v_k] = \sum_{c \in \mathcal{P}: (x_i,x_j,x_k) \in c} \Biggr[-\frac{1}{8}\Bigg(-\tau_i \tau_j \tau_k \frac{1}{3} v_{ij}\Bigg)\\ + 2\rho \left[(\langle v_k,v_{ij}\rangle - \langle v_i,v_{jk}\rangle) v_{ij} + (\langle v_i,v_{jk}\rangle - \langle v_k,v_{ij}\rangle)(-v_{ij})\right] \Biggr]
\end{multline}
\paragraph{Message: Single to Pair for Single in Pair.} This is the message $\text{MESSAGE}[v_{i} \rightarrow v_{ij}]$ for each single node $v_{i}$ to a pair $v_k$
\begin{align}
\text{MESSAGE}[v_{i} \rightarrow v_{ij}] =
      |\{c \in \mathcal{P}: x_i,x_j \in c\}|2\rho (\langle v_i,v_{ij}\rangle - \langle v_j,v_\emptyset\rangle) v_{i}
\end{align}
\paragraph{Message: Single to Pair for Single not in Pair.} This is the message $\text{MESSAGE}[v_{ij} \rightarrow v_k]$  for each pair node $v_{ij}$ to a single $v_k$ node. 
\begin{align}
\text{MESSAGE}[v_{ij} \rightarrow v_k] =\sum_{c \in \mathcal{P}: (x_i,x_j,x_k) \in c} \Biggr[-\frac{1}{8}\Bigg(-\tau_i \tau_j \tau_k \frac{1}{3} v_{k}\Bigg)  + 2\rho \left[(\langle v_k,v_{ij}\rangle - \langle v_i,v_{jk}\rangle) v_{k} + (\langle v_k,v_{ij}\rangle - \langle v_j,v_{ik}\rangle)v_{k}\right] \Biggr]
\end{align}
\paragraph{Message: Single to Single} This is the message $\text{MESSAGE}[v_{i} \rightarrow v_j]$  for each single node $v_{i}$ to a single $v_j$ node. 
\begin{align}
\text{MESSAGE}[v_{i} \rightarrow v_j] = \sum_{c \in \mathcal{P}: (x_i,x_j,x_k) \in c} \Biggr[-\frac{1}{8}\Bigg(-\tau_i \tau_j \frac{1}{2} v_{i}\Bigg) + 2\rho \left[(\langle v_i,v_{j}\rangle - \langle v_{ij},v_{\emptyset}\rangle) v_{i} + (\langle v_{ik},v_{jk}\rangle - \langle v_i,v_j\rangle)(-v_i)\right] \Biggr]
\end{align}
\paragraph{Message: Pair to Pair} This is the message $\text{MESSAGE}[v_{ij} \rightarrow v_{jk}]$  for each pair node $v_{ij}$ to a pair $v_{jk}$ node. 
\begin{align}
\text{MESSAGE}[v_{ij} \rightarrow v_{jk}] =  |\{c \in \mathcal{P}: x_i,x_j,x_k \in c\}|2\rho \left[(\langle v_{ij},v_{jk}\rangle - \langle v_{i},v_{k}\rangle) v_{ij}\right] 
\end{align}
Then the $\text{OptGNN}_{(M,G_\Lambda)}$ is defined with the following functions UPDATE, AGGREGATE, and NONLINEAR.   
For any node $v$, the OptGNN update is 
\begin{align}
\text{AGGREGATE}(\{v_{\zeta}\}_{\zeta \in N(v)}) &\defeq \sum_{v_\zeta \in N(v)}\text{MESSAGE}[v_\zeta \rightarrow v] \\
\text{UPDATE}(v) &= M\left(\begin{bmatrix}
v \\
\text{AGGREGATE}(\{v_{\zeta}\}_{\zeta \in N(v)})
\end{bmatrix}\right) \\ 
\text{NONLINEAR}(v) &= \frac{v}{\|v\|} 
\end{align}
\end{definition}
Finally, we note that many of the signs in the forms of messages could have been chosen differently i.e $\langle v_i,v_j\rangle - \langle v_{ij}, v_\emptyset\rangle$ produces different gradients from $\langle v_{ij}, v_\emptyset\rangle - \langle v_i,v_j\rangle$.  We leave small choices like this to the reader.    


